Averages of $b$-hadron, $c$-hadron, and $\tau$-lepton properties as of 2018

This paper reports world averages of measurements of $b$-hadron, $c$-hadron, and $\tau$-lepton properties obtained by the Heavy Flavor Averaging Group using results available through September 2018. In rare cases, significant results obtained several months later are also used. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, CP violation parameters, parameters of semileptonic decays, and Cabibbo-Kobayashi-Maskawa matrix elements.

==> tau/hflav-2018-elab-vadirect.tex <==
\htquantdef{B_tau_had_fit}{B_tau_had_fit}{}{64.76 \pm 0.10}{64.76}{0.10}%
\htquantdef{B_tau_had_uni}{B_tau_had_uni}{}{64.79 \pm 0.06}{64.79}{0.06}%
\htquantdef{B_tau_had_uni_SM}{B_tau_had_uni_SM}{}{64.86 \pm 0.04}{64.86}{0.04}%
\htquantdef{B_tau_s_fit}{B_tau_s_fit}{}{2.931 \pm 0.041}{2.931}{0.041}%
\htquantdef{B_tau_s_unitarity}{B_tau_s_unitarity}{}{(2.958 \pm 0.098) \cdot 10^{-2}}{2.958\cdot 10^{-2}}{0.098\cdot 10^{-2}}%
\htquantdef{B_tau_VA}{B_tau_VA}{}{0.61833 \pm 0.00099}{0.61833}{0.00099}%
\htquantdef{B_tau_VA_fit}{B_tau_VA_fit}{}{61.83 \pm 0.10}{61.83}{0.10}%
\htquantdef{B_tau_VA_unitarity}{B_tau_VA_unitarity}{}{0.61861 \pm 0.00075}{0.61861}{0.00075}%
\htquantdef{Be_by_tau_tau}{Be_by_tau_tau}{}{(6.1248 \pm 0.0021) \cdot 10^{11}}{6.1248\cdot 10^{11}}{0.0021\cdot 10^{11}}%
\htquantdef{Be_fit}{Be_fit}{}{0.17817 \pm 0.00041}{0.17817}{0.00041}%
\htquantdef{Be_from_Bmu}{Be_from_Bmu}{}{0.17882 \pm 0.00041}{0.17882}{0.00041}%
\htquantdef{Be_from_taulife}{Be_from_taulife}{}{0.17780 \pm 0.00031}{0.17780}{0.00031}%
\htquantdef{Be_lept}{Be_lept}{}{17.850 \pm 0.032}{17.850}{0.032}%
\htquantdef{Be_lept_unc_perc}{Be_lept_unc_perc}{}{0.178}{0.178}{0}%
\htquantdef{Be_unitarity}{Be_unitarity}{}{0.1784 \pm 0.0010}{0.1784}{0.0010}%
\htquantdef{Be_univ}{Be_univ}{}{17.814 \pm 0.022}{17.814}{0.022}%
\htquantdef{Bmu_by_Be_th}{Bmu_by_Be_th}{}{0.9725606 \pm 0.0000036}{0.9725606}{0.0000036}%
\htquantdef{Bmu_fit}{Bmu_fit}{}{0.17392 \pm 0.00039}{0.17392}{0.00039}%
\htquantdef{Bmu_from_taulife}{Bmu_from_taulife}{}{0.17293 \pm 0.00030}{0.17293}{0.00030}%
\htquantdef{Bmu_unitarity}{Bmu_unitarity}{}{0.1742 \pm 0.0010}{0.1742}{0.0010}%
\htquantdef{BR_a1_pigamma}{BR_a1_pigamma}{}{0.2100\cdot 10^{-2}}{0.2100\cdot 10^{-2}}{0}%
\htquantdef{BR_eta_2gam}{BR_eta_2gam}{}{0.3941}{0.3941}{0}%
\htquantdef{BR_eta_3piz}{BR_eta_3piz}{}{0.3268}{0.3268}{0}%
\htquantdef{BR_eta_charged}{BR_eta_charged}{}{0.2810}{0.2810}{0}%
\htquantdef{BR_eta_neutral}{BR_eta_neutral}{}{0.7212}{0.7212}{0}%
\htquantdef{BR_eta_pimpipgamma}{BR_eta_pimpipgamma}{}{4.220\cdot 10^{-2}}{4.220\cdot 10^{-2}}{0}%
\htquantdef{BR_eta_pimpippiz}{BR_eta_pimpippiz}{}{0.2292}{0.2292}{0}%
\htquantdef{BR_f1_2pip2pim}{BR_f1_2pip2pim}{}{0.1120}{0.1120}{0}%
\htquantdef{BR_f1_2pizpippim}{BR_f1_2pizpippim}{}{0.2230}{0.2230}{0}%
\htquantdef{BR_KS_2piz}{BR_KS_2piz}{}{0.3069}{0.3069}{0}%
\htquantdef{BR_KS_pimpip}{BR_KS_pimpip}{}{0.6920}{0.6920}{0}%
\htquantdef{BR_om_pimpip}{BR_om_pimpip}{}{1.530\cdot 10^{-2}}{1.530\cdot 10^{-2}}{0}%
\htquantdef{BR_om_pimpippiz}{BR_om_pimpippiz}{}{0.8920}{0.8920}{0}%
\htquantdef{BR_om_pizgamma}{BR_om_pizgamma}{}{8.400\cdot 10^{-2}}{8.400\cdot 10^{-2}}{0}%
\htquantdef{BR_phi_KmKp}{BR_phi_KmKp}{}{0.4920}{0.4920}{0}%
\htquantdef{BR_phi_KSKL}{BR_phi_KSKL}{}{0.3400}{0.3400}{0}%
\htquantdef{BRA_Kz_KL_KET}{BRA_Kz_KL_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{BRA_Kz_KS_KET}{BRA_Kz_KS_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{BRA_Kzbar_KL_KET}{BRA_Kzbar_KL_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{BRA_Kzbar_KS_KET}{BRA_Kzbar_KS_KET}{}{0.5000}{0.5000}{0}%
\htquantdef{deltaR_su3break}{deltaR_su3break}{}{0.242 \pm 0.033}{0.242}{0.033}%
\htquantdef{deltaR_su3break_d2pert}{deltaR_su3break_d2pert}{}{9.300 \pm 3.400}{9.300}{3.400}%
\htquantdef{deltaR_su3break_pheno}{deltaR_su3break_pheno}{}{0.1544 \pm 0.0037}{0.1544}{0.0037}%
\htquantdef{deltaR_su3break_remain}{deltaR_su3break_remain}{}{(0.3400 \pm 0.2800) \cdot 10^{-2}}{0.3400\cdot 10^{-2}}{0.2800\cdot 10^{-2}}%
\htquantdef{dRrad_K_munu}{dRrad_K_munu}{}{1.07 \pm 0.21}{1.07}{0.21}%
\htquantdef{dRrad_kmunu_by_pimunu}{dRrad_kmunu_by_pimunu}{}{-0.69 \pm 0.17}{-0.69}{0.17}%
\htquantdef{dRrad_pi_munu}{dRrad_pi_munu}{}{1.76 \pm 0.21}{1.76}{0.21}%
\htquantdef{dRrad_tauK_by_Kmu}{dRrad_tauK_by_Kmu}{}{0.90 \pm 0.22}{0.90}{0.22}%
\htquantdef{dRrad_taupi_by_pimu}{dRrad_taupi_by_pimu}{}{0.16 \pm 0.14}{0.16}{0.14}%
\htquantdef{EmNuNumb}{EmNuNumb}{}{0.1782}{0.1782}{0}%
\htquantdef{f_Kpm}{f_Kpm}{}{155.7 \pm 0.3}{155.7}{0.3}%
\htquantdef{f_Kpm_by_f_pipm}{f_Kpm_by_f_pipm}{}{1.1932 \pm 0.0019}{1.1932}{0.0019}%
\htquantdef{f_pipm}{f_pipm}{}{130.2 \pm 0.8}{130.2}{0.8}%
\htquantdef{G_F_by_hcut3_c3}{G_F_by_hcut3_c3}{}{(1.16637870 \pm 0.00000060) \cdot 10^{-11}}{1.16637870\cdot 10^{-11}}{0.00000060\cdot 10^{-11}}%
\htquantdef{Gamma1}{\BR_{1}}{\BRF{\tau^-}{(\text{particles})^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K^0\, \nu_\tau}}{0.8521 \pm 0.0011}{0.8521}{0.0011}%
\htquantdef{Gamma10}{\BR_{10}}{\BRF{\tau^-}{K^- \nu_\tau}}{(0.6986 \pm 0.0085) \cdot 10^{-2}}{0.6986\cdot 10^{-2}}{0.0085\cdot 10^{-2}}%
\htquantdef{Gamma102}{\BR_{102}}{\BRF{\tau^-}{3h^- 2h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.~} K^0)}}{(9.901 \pm 0.368) \cdot 10^{-4}}{9.901\cdot 10^{-4}}{0.368\cdot 10^{-4}}%
\htquantdef{Gamma103}{\BR_{103}}{\BRF{\tau^-}{3h^- 2h^+ \nu_\tau ~(\text{ex.~}K^0)}}{(8.260 \pm 0.314) \cdot 10^{-4}}{8.260\cdot 10^{-4}}{0.314\cdot 10^{-4}}%
\htquantdef{Gamma104}{\BR_{104}}{\BRF{\tau^-}{3h^- 2h^+ \pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(1.641 \pm 0.114) \cdot 10^{-4}}{1.641\cdot 10^{-4}}{0.114\cdot 10^{-4}}%
\htquantdef{Gamma106}{\BR_{106}}{\BRF{\tau^-}{(5\pi)^- \nu_\tau}}{(0.7532 \pm 0.0356) \cdot 10^{-2}}{0.7532\cdot 10^{-2}}{0.0356\cdot 10^{-2}}%
\htquantdef{Gamma10by5}{\frac{\BR_{10}}{\BR_{5}}}{\frac{\BRF{\tau^-}{K^- \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{(3.921 \pm 0.048) \cdot 10^{-2}}{3.921\cdot 10^{-2}}{0.048\cdot 10^{-2}}%
\htquantdef{Gamma10by9}{\frac{\BR_{10}}{\BR_{9}}}{\frac{\BRF{\tau^-}{K^- \nu_\tau}}{\BRF{\tau^-}{\pi^- \nu_\tau}}}{(6.467 \pm 0.084) \cdot 10^{-2}}{6.467\cdot 10^{-2}}{0.084\cdot 10^{-2}}%
\htquantdef{Gamma11}{\BR_{11}}{\BRF{\tau^-}{h^- \ge{} 1\,  \text{neutrals}\, \nu_\tau}}{0.36996 \pm 0.00094}{0.36996}{0.00094}%
\htquantdef{Gamma110}{\BR_{110}}{\BRF{\tau^-}{X_s^- \nu_\tau}}{(2.931 \pm 0.041) \cdot 10^{-2}}{2.931\cdot 10^{-2}}{0.041\cdot 10^{-2}}%
\htquantdef{Gamma110_pdg09}{\BR_{110}_pdg09}{}{(2.863 \pm 0.028) \cdot 10^{-2}}{2.863\cdot 10^{-2}}{0.028\cdot 10^{-2}}%
\htquantdef{Gamma12}{\BR_{12}}{\BRF{\tau^-}{h^- \ge{} 1\, \pi^0\, \nu_\tau\;(\text{ex.~} K^0)}}{0.36495 \pm 0.00094}{0.36495}{0.00094}%
\htquantdef{Gamma126}{\BR_{126}}{\BRF{\tau^-}{\pi^- \pi^0 \eta \nu_\tau}}{(0.1386 \pm 0.0072) \cdot 10^{-2}}{0.1386\cdot 10^{-2}}{0.0072\cdot 10^{-2}}%
\htquantdef{Gamma128}{\BR_{128}}{\BRF{\tau^-}{K^- \eta \nu_\tau}}{(1.543 \pm 0.080) \cdot 10^{-4}}{1.543\cdot 10^{-4}}{0.080\cdot 10^{-4}}%
\htquantdef{Gamma13}{\BR_{13}}{\BRF{\tau^-}{h^- \pi^0 \nu_\tau}}{0.25938 \pm 0.00090}{0.25938}{0.00090}%
\htquantdef{Gamma130}{\BR_{130}}{\BRF{\tau^-}{K^- \pi^0 \eta \nu_\tau}}{(4.825 \pm 1.161) \cdot 10^{-5}}{4.825\cdot 10^{-5}}{1.161\cdot 10^{-5}}%
\htquantdef{Gamma132}{\BR_{132}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \eta \nu_\tau}}{(9.364 \pm 1.491) \cdot 10^{-5}}{9.364\cdot 10^{-5}}{1.491\cdot 10^{-5}}%
\htquantdef{Gamma136}{\BR_{136}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \eta \nu_\tau\;(\text{ex.~} K^0)}}{(2.196 \pm 0.129) \cdot 10^{-4}}{2.196\cdot 10^{-4}}{0.129\cdot 10^{-4}}%
\htquantdef{Gamma14}{\BR_{14}}{\BRF{\tau^-}{\pi^- \pi^0 \nu_\tau}}{0.25447 \pm 0.00091}{0.25447}{0.00091}%
\htquantdef{Gamma149}{\BR_{149}}{\BRF{\tau^-}{h^- \omega \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(2.402 \pm 0.075) \cdot 10^{-2}}{2.402\cdot 10^{-2}}{0.075\cdot 10^{-2}}%
\htquantdef{Gamma150}{\BR_{150}}{\BRF{\tau^-}{h^- \omega \nu_\tau}}{(1.996 \pm 0.064) \cdot 10^{-2}}{1.996\cdot 10^{-2}}{0.064\cdot 10^{-2}}%
\htquantdef{Gamma150by66}{\frac{\BR_{150}}{\BR_{66}}}{\frac{\BRF{\tau^-}{h^- \omega \nu_\tau}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}}{0.4331 \pm 0.0139}{0.4331}{0.0139}%
\htquantdef{Gamma151}{\BR_{151}}{\BRF{\tau^-}{K^- \omega \nu_\tau}}{(4.100 \pm 0.922) \cdot 10^{-4}}{4.100\cdot 10^{-4}}{0.922\cdot 10^{-4}}%
\htquantdef{Gamma152}{\BR_{152}}{\BRF{\tau^-}{h^- \pi^0 \omega \nu_\tau}}{(0.4066 \pm 0.0419) \cdot 10^{-2}}{0.4066\cdot 10^{-2}}{0.0419\cdot 10^{-2}}%
\htquantdef{Gamma152by54}{\frac{\BR_{152}}{\BR_{54}}}{\frac{\BRF{\tau^-}{h^- \omega \pi^0 \nu_\tau}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}}{(2.674 \pm 0.275) \cdot 10^{-2}}{2.674\cdot 10^{-2}}{0.275\cdot 10^{-2}}%
\htquantdef{Gamma152by76}{\frac{\BR_{152}}{\BR_{76}}}{\frac{\BRF{\tau^-}{h^- \omega \pi^0 \nu_\tau}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.~} K^0)}}}{0.8236 \pm 0.0757}{0.8236}{0.0757}%
\htquantdef{Gamma16}{\BR_{16}}{\BRF{\tau^-}{K^- \pi^0 \nu_\tau}}{(0.4904 \pm 0.0092) \cdot 10^{-2}}{0.4904\cdot 10^{-2}}{0.0092\cdot 10^{-2}}%
\htquantdef{Gamma167}{\BR_{167}}{\BRF{\tau^-}{K^- \phi \nu_\tau}}{(4.409 \pm 1.626) \cdot 10^{-5}}{4.409\cdot 10^{-5}}{1.626\cdot 10^{-5}}%
\htquantdef{Gamma168}{\BR_{168}}{\BRF{\tau^-}{K^- \phi \nu_\tau ~(\phi \to K^+ K^-)}}{(2.169 \pm 0.800) \cdot 10^{-5}}{2.169\cdot 10^{-5}}{0.800\cdot 10^{-5}}%
\htquantdef{Gamma169}{\BR_{169}}{\BRF{\tau^-}{K^- \phi \nu_\tau ~(\phi \to K_S^0 K_L^0)}}{(1.499 \pm 0.553) \cdot 10^{-5}}{1.499\cdot 10^{-5}}{0.553\cdot 10^{-5}}%
\htquantdef{Gamma17}{\BR_{17}}{\BRF{\tau^-}{h^- \ge{} 2\,  \pi^0\, \nu_\tau}}{0.10793 \pm 0.00091}{0.10793}{0.00091}%
\htquantdef{Gamma18}{\BR_{18}}{\BRF{\tau^-}{h^- 2\pi^0 \nu_\tau}}{(9.421 \pm 0.092) \cdot 10^{-2}}{9.421\cdot 10^{-2}}{0.092\cdot 10^{-2}}%
\htquantdef{Gamma19}{\BR_{19}}{\BRF{\tau^-}{h^- 2\pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(9.270 \pm 0.092) \cdot 10^{-2}}{9.270\cdot 10^{-2}}{0.092\cdot 10^{-2}}%
\htquantdef{Gamma19by13}{\frac{\BR_{19}}{\BR_{13}}}{\frac{\BRF{\tau^-}{h^- 2\pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{\BRF{\tau^-}{h^- \pi^0 \nu_\tau}}}{0.3574 \pm 0.0042}{0.3574}{0.0042}%
\htquantdef{Gamma2}{\BR_{2}}{\BRF{\tau^-}{(\text{particles})^- \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}{0.8455 \pm 0.0010}{0.8455}{0.0010}%
\htquantdef{Gamma20}{\BR_{20}}{\BRF{\tau^-}{\pi^- 2\pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(9.211 \pm 0.092) \cdot 10^{-2}}{9.211\cdot 10^{-2}}{0.092\cdot 10^{-2}}%
\htquantdef{Gamma23}{\BR_{23}}{\BRF{\tau^-}{K^- 2\pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(5.850 \pm 0.272) \cdot 10^{-4}}{5.850\cdot 10^{-4}}{0.272\cdot 10^{-4}}%
\htquantdef{Gamma24}{\BR_{24}}{\BRF{\tau^-}{h^- \ge{} 3\, \pi^0\, \nu_\tau}}{(1.372 \pm 0.034) \cdot 10^{-2}}{1.372\cdot 10^{-2}}{0.034\cdot 10^{-2}}%
\htquantdef{Gamma25}{\BR_{25}}{\BRF{\tau^-}{h^- \ge{} 3\, \pi^0\, \nu_\tau\;(\text{ex.~} K^0)}}{(1.288 \pm 0.034) \cdot 10^{-2}}{1.288\cdot 10^{-2}}{0.034\cdot 10^{-2}}%
\htquantdef{Gamma26}{\BR_{26}}{\BRF{\tau^-}{h^- 3\pi^0 \nu_\tau}}{(1.236 \pm 0.030) \cdot 10^{-2}}{1.236\cdot 10^{-2}}{0.030\cdot 10^{-2}}%
\htquantdef{Gamma26by13}{\frac{\BR_{26}}{\BR_{13}}}{\frac{\BRF{\tau^-}{h^- 3\pi^0 \nu_\tau}}{\BRF{\tau^-}{h^- \pi^0 \nu_\tau}}}{(4.764 \pm 0.118) \cdot 10^{-2}}{4.764\cdot 10^{-2}}{0.118\cdot 10^{-2}}%
\htquantdef{Gamma27}{\BR_{27}}{\BRF{\tau^-}{\pi^- 3\pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(1.138 \pm 0.029) \cdot 10^{-2}}{1.138\cdot 10^{-2}}{0.029\cdot 10^{-2}}%
\htquantdef{Gamma28}{\BR_{28}}{\BRF{\tau^-}{K^- 3\pi^0 \nu_\tau ~(\text{ex.~}K^0,\eta)}}{(1.127 \pm 0.263) \cdot 10^{-4}}{1.127\cdot 10^{-4}}{0.263\cdot 10^{-4}}%
\htquantdef{Gamma29}{\BR_{29}}{\BRF{\tau^-}{h^- 4\pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(0.1333 \pm 0.0071) \cdot 10^{-2}}{0.1333\cdot 10^{-2}}{0.0071\cdot 10^{-2}}%
\htquantdef{Gamma3}{\BR_{3}}{\BRF{\tau^-}{\mu^- \bar{\nu}_\mu \nu_\tau}}{0.17392 \pm 0.00039}{0.17392}{0.00039}%
\htquantdef{Gamma30}{\BR_{30}}{\BRF{\tau^-}{h^- 4\pi^0 \nu_\tau ~(\text{ex.~}K^0,\eta)}}{(8.640 \pm 0.670) \cdot 10^{-4}}{8.640\cdot 10^{-4}}{0.670\cdot 10^{-4}}%
\htquantdef{Gamma31}{\BR_{31}}{\BRF{\tau^-}{K^- \ge{} 0\, \pi^0 \ge{} 0\, K^0 \ge{} 0\, \gamma \nu_\tau}}{(1.568 \pm 0.018) \cdot 10^{-2}}{1.568\cdot 10^{-2}}{0.018\cdot 10^{-2}}%
\htquantdef{Gamma32}{\BR_{32}}{\BRF{\tau^-}{K^- \ge{} 1\, (\pi^0\,\text{or}\,K^0\,\text{or}\,\gamma) \nu_\tau}}{(0.8729 \pm 0.0141) \cdot 10^{-2}}{0.8729\cdot 10^{-2}}{0.0141\cdot 10^{-2}}%
\htquantdef{Gamma33}{\BR_{33}}{\BRF{\tau^-}{K_S^0 (\text{particles})^- \nu_\tau}}{(0.9366 \pm 0.0292) \cdot 10^{-2}}{0.9366\cdot 10^{-2}}{0.0292\cdot 10^{-2}}%
\htquantdef{Gamma34}{\BR_{34}}{\BRF{\tau^-}{h^- \bar{K}^0 \nu_\tau}}{(0.9860 \pm 0.0138) \cdot 10^{-2}}{0.9860\cdot 10^{-2}}{0.0138\cdot 10^{-2}}%
\htquantdef{Gamma35}{\BR_{35}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \nu_\tau}}{(0.8378 \pm 0.0139) \cdot 10^{-2}}{0.8378\cdot 10^{-2}}{0.0139\cdot 10^{-2}}%
\htquantdef{Gamma37}{\BR_{37}}{\BRF{\tau^-}{K^- K^0 \nu_\tau}}{(0.1483 \pm 0.0034) \cdot 10^{-2}}{0.1483\cdot 10^{-2}}{0.0034\cdot 10^{-2}}%
\htquantdef{Gamma38}{\BR_{38}}{\BRF{\tau^-}{K^- K^0 \ge{} 0\,  \pi^0\, \nu_\tau}}{(0.2977 \pm 0.0073) \cdot 10^{-2}}{0.2977\cdot 10^{-2}}{0.0073\cdot 10^{-2}}%
\htquantdef{Gamma39}{\BR_{39}}{\BRF{\tau^-}{h^- \bar{K}^0 \pi^0 \nu_\tau}}{(0.5302 \pm 0.0134) \cdot 10^{-2}}{0.5302\cdot 10^{-2}}{0.0134\cdot 10^{-2}}%
\htquantdef{Gamma3by5}{\frac{\BR_{3}}{\BR_{5}}}{\frac{\BRF{\tau^-}{\mu^- \bar{\nu}_\mu \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{0.9761 \pm 0.0028}{0.9761}{0.0028}%
\htquantdef{Gamma40}{\BR_{40}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \pi^0 \nu_\tau}}{(0.3807 \pm 0.0129) \cdot 10^{-2}}{0.3807\cdot 10^{-2}}{0.0129\cdot 10^{-2}}%
\htquantdef{Gamma42}{\BR_{42}}{\BRF{\tau^-}{K^- \pi^0 K^0 \nu_\tau}}{(0.1494 \pm 0.0070) \cdot 10^{-2}}{0.1494\cdot 10^{-2}}{0.0070\cdot 10^{-2}}%
\htquantdef{Gamma43}{\BR_{43}}{\BRF{\tau^-}{\pi^- \bar{K}^0 \ge{} 1\,  \pi^0\, \nu_\tau}}{(0.4042 \pm 0.0260) \cdot 10^{-2}}{0.4042\cdot 10^{-2}}{0.0260\cdot 10^{-2}}%
\htquantdef{Gamma44}{\BR_{44}}{\BRF{\tau^-}{\pi^- \bar{K}^0 2\pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(2.346 \pm 2.306) \cdot 10^{-4}}{2.346\cdot 10^{-4}}{2.306\cdot 10^{-4}}%
\htquantdef{Gamma46}{\BR_{46}}{\BRF{\tau^-}{\pi^- K^0 \bar{K}^0 \nu_\tau}}{(0.1516 \pm 0.0247) \cdot 10^{-2}}{0.1516\cdot 10^{-2}}{0.0247\cdot 10^{-2}}%
\htquantdef{Gamma47}{\BR_{47}}{\BRF{\tau^-}{\pi^- K_S^0 K_S^0 \nu_\tau}}{(2.342 \pm 0.065) \cdot 10^{-4}}{2.342\cdot 10^{-4}}{0.065\cdot 10^{-4}}%
\htquantdef{Gamma48}{\BR_{48}}{\BRF{\tau^-}{\pi^- K_S^0 K_L^0 \nu_\tau}}{(0.1048 \pm 0.0247) \cdot 10^{-2}}{0.1048\cdot 10^{-2}}{0.0247\cdot 10^{-2}}%
\htquantdef{Gamma49}{\BR_{49}}{\BRF{\tau^-}{\pi^- K^0 \bar{K}^0 \pi^0 \nu_\tau}}{(3.543 \pm 1.193) \cdot 10^{-4}}{3.543\cdot 10^{-4}}{1.193\cdot 10^{-4}}%
\htquantdef{Gamma5}{\BR_{5}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}{0.17817 \pm 0.00041}{0.17817}{0.00041}%
\htquantdef{Gamma50}{\BR_{50}}{\BRF{\tau^-}{\pi^- \pi^0 K_S^0 K_S^0 \nu_\tau}}{(1.816 \pm 0.207) \cdot 10^{-5}}{1.816\cdot 10^{-5}}{0.207\cdot 10^{-5}}%
\htquantdef{Gamma51}{\BR_{51}}{\BRF{\tau^-}{\pi^- \pi^0 K_S^0 K_L^0 \nu_\tau}}{(3.179 \pm 1.192) \cdot 10^{-4}}{3.179\cdot 10^{-4}}{1.192\cdot 10^{-4}}%
\htquantdef{Gamma53}{\BR_{53}}{\BRF{\tau^-}{\bar{K}^0 h^- h^- h^+ \nu_\tau}}{(2.220 \pm 2.024) \cdot 10^{-4}}{2.220\cdot 10^{-4}}{2.024\cdot 10^{-4}}%
\htquantdef{Gamma54}{\BR_{54}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}{0.15206 \pm 0.00061}{0.15206}{0.00061}%
\htquantdef{Gamma55}{\BR_{55}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.~} K^0)}}{0.14558 \pm 0.00056}{0.14558}{0.00056}%
\htquantdef{Gamma56}{\BR_{56}}{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau}}{(9.769 \pm 0.053) \cdot 10^{-2}}{9.769\cdot 10^{-2}}{0.053\cdot 10^{-2}}%
\htquantdef{Gamma57}{\BR_{57}}{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau\;(\text{ex.~} K^0)}}{(9.428 \pm 0.053) \cdot 10^{-2}}{9.428\cdot 10^{-2}}{0.053\cdot 10^{-2}}%
\htquantdef{Gamma57by55}{\frac{\BR_{57}}{\BR_{55}}}{\frac{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau\;(\text{ex.~} K^0)}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau\;(\text{ex.~} K^0)}}}{0.6476 \pm 0.0029}{0.6476}{0.0029}%
\htquantdef{Gamma58}{\BR_{58}}{\BRF{\tau^-}{h^- h^- h^+ \nu_\tau\;(\text{ex.~} K^0, \omega)}}{(9.397 \pm 0.053) \cdot 10^{-2}}{9.397\cdot 10^{-2}}{0.053\cdot 10^{-2}}%
\htquantdef{Gamma59}{\BR_{59}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau}}{(9.279 \pm 0.051) \cdot 10^{-2}}{9.279\cdot 10^{-2}}{0.051\cdot 10^{-2}}%
\htquantdef{Gamma60}{\BR_{60}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.~} K^0)}}{(8.990 \pm 0.051) \cdot 10^{-2}}{8.990\cdot 10^{-2}}{0.051\cdot 10^{-2}}%
\htquantdef{Gamma62}{\BR_{62}}{\BRF{\tau^-}{\pi^- \pi^- \pi^+ \nu_\tau ~(\text{ex.~}K^0,\omega)}}{(8.960 \pm 0.051) \cdot 10^{-2}}{8.960\cdot 10^{-2}}{0.051\cdot 10^{-2}}%
\htquantdef{Gamma63}{\BR_{63}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 1\,  \text{neutrals}\, \nu_\tau}}{(5.327 \pm 0.049) \cdot 10^{-2}}{5.327\cdot 10^{-2}}{0.049\cdot 10^{-2}}%
\htquantdef{Gamma64}{\BR_{64}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 1\,  \pi^0\, \nu_\tau\;(\text{ex.~} K^0)}}{(5.122 \pm 0.049) \cdot 10^{-2}}{5.122\cdot 10^{-2}}{0.049\cdot 10^{-2}}%
\htquantdef{Gamma65}{\BR_{65}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau}}{(4.791 \pm 0.052) \cdot 10^{-2}}{4.791\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma66}{\BR_{66}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(4.607 \pm 0.051) \cdot 10^{-2}}{4.607\cdot 10^{-2}}{0.051\cdot 10^{-2}}%
\htquantdef{Gamma67}{\BR_{67}}{\BRF{\tau^-}{h^- h^- h^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0, \omega)}}{(2.821 \pm 0.070) \cdot 10^{-2}}{2.821\cdot 10^{-2}}{0.070\cdot 10^{-2}}%
\htquantdef{Gamma68}{\BR_{68}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau}}{(4.652 \pm 0.053) \cdot 10^{-2}}{4.652\cdot 10^{-2}}{0.053\cdot 10^{-2}}%
\htquantdef{Gamma69}{\BR_{69}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(4.520 \pm 0.052) \cdot 10^{-2}}{4.520\cdot 10^{-2}}{0.052\cdot 10^{-2}}%
\htquantdef{Gamma7}{\BR_{7}}{\BRF{\tau^-}{h^- \ge{} 0\,  K_L^0\, \nu_\tau}}{0.12019 \pm 0.00053}{0.12019}{0.00053}%
\htquantdef{Gamma70}{\BR_{70}}{\BRF{\tau^-}{\pi^- \pi^- \pi^+ \pi^0 \nu_\tau ~(\text{ex.~}K^0,\omega)}}{(2.770 \pm 0.071) \cdot 10^{-2}}{2.770\cdot 10^{-2}}{0.071\cdot 10^{-2}}%
\htquantdef{Gamma74}{\BR_{74}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 2\, \pi^0\, \nu_\tau\;(\text{ex.~} K^0)}}{(0.5148 \pm 0.0311) \cdot 10^{-2}}{0.5148\cdot 10^{-2}}{0.0311\cdot 10^{-2}}%
\htquantdef{Gamma75}{\BR_{75}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau}}{(0.5037 \pm 0.0309) \cdot 10^{-2}}{0.5037\cdot 10^{-2}}{0.0309\cdot 10^{-2}}%
\htquantdef{Gamma76}{\BR_{76}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(0.4937 \pm 0.0309) \cdot 10^{-2}}{0.4937\cdot 10^{-2}}{0.0309\cdot 10^{-2}}%
\htquantdef{Gamma76by54}{\frac{\BR_{76}}{\BR_{54}}}{\frac{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{\BRF{\tau^-}{h^- h^- h^+ \ge{} 0\, \text{neutrals} \ge{} 0\,  K_L^0\, \nu_\tau}}}{(3.247 \pm 0.202) \cdot 10^{-2}}{3.247\cdot 10^{-2}}{0.202\cdot 10^{-2}}%
\htquantdef{Gamma77}{\BR_{77}}{\BRF{\tau^-}{h^- h^- h^+ 2\pi^0 \nu_\tau ~(\text{ex.~}K^0,\omega,\eta)}}{(9.812 \pm 3.555) \cdot 10^{-4}}{9.812\cdot 10^{-4}}{3.555\cdot 10^{-4}}%
\htquantdef{Gamma78}{\BR_{78}}{\BRF{\tau^-}{h^- h^- h^+ 3\pi^0 \nu_\tau}}{(2.114 \pm 0.299) \cdot 10^{-4}}{2.114\cdot 10^{-4}}{0.299\cdot 10^{-4}}%
\htquantdef{Gamma79}{\BR_{79}}{\BRF{\tau^-}{K^- h^- h^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(0.6293 \pm 0.0140) \cdot 10^{-2}}{0.6293\cdot 10^{-2}}{0.0140\cdot 10^{-2}}%
\htquantdef{Gamma8}{\BR_{8}}{\BRF{\tau^-}{h^- \nu_\tau}}{0.11502 \pm 0.00053}{0.11502}{0.00053}%
\htquantdef{Gamma80}{\BR_{80}}{\BRF{\tau^-}{K^- \pi^- h^+ \nu_\tau\;(\text{ex.~} K^0)}}{(0.4361 \pm 0.0072) \cdot 10^{-2}}{0.4361\cdot 10^{-2}}{0.0072\cdot 10^{-2}}%
\htquantdef{Gamma800}{\BR_{800}}{\BRF{\tau^-}{\pi^- \omega \nu_\tau}}{(1.955 \pm 0.065) \cdot 10^{-2}}{1.955\cdot 10^{-2}}{0.065\cdot 10^{-2}}%
\htquantdef{Gamma802}{\BR_{802}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \nu_\tau ~(\text{ex.~}K^0,\omega)}}{(0.2923 \pm 0.0067) \cdot 10^{-2}}{0.2923\cdot 10^{-2}}{0.0067\cdot 10^{-2}}%
\htquantdef{Gamma803}{\BR_{803}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau ~(\text{ex.~}K^0,\omega,\eta)}}{(4.105 \pm 1.429) \cdot 10^{-4}}{4.105\cdot 10^{-4}}{1.429\cdot 10^{-4}}%
\htquantdef{Gamma804}{\BR_{804}}{\BRF{\tau^-}{\pi^- K_L^0 K_L^0 \nu_\tau}}{(2.342 \pm 0.065) \cdot 10^{-4}}{2.342\cdot 10^{-4}}{0.065\cdot 10^{-4}}%
\htquantdef{Gamma805}{\BR_{805}}{\BRF{\tau^-}{a_1^- (\to \pi^- \gamma) \nu_\tau}}{(4.000 \pm 2.000) \cdot 10^{-4}}{4.000\cdot 10^{-4}}{2.000\cdot 10^{-4}}%
\htquantdef{Gamma806}{\BR_{806}}{\BRF{\tau^-}{\pi^- \pi^0 K_L^0 K_L^0 \nu_\tau}}{(1.816 \pm 0.207) \cdot 10^{-5}}{1.816\cdot 10^{-5}}{0.207\cdot 10^{-5}}%
\htquantdef{Gamma809}{\BR_{809}}{\BRF{\tau^-}{\pi^- 4\pi^0 \nu_\tau\;(\text{ex.~} K^0, \eta)}}{(8.640 \pm 0.670) \cdot 10^{-4}}{8.640\cdot 10^{-4}}{0.670\cdot 10^{-4}}%
\htquantdef{Gamma80by60}{\frac{\BR_{80}}{\BR_{60}}}{\frac{\BRF{\tau^-}{K^- \pi^- h^+ \nu_\tau\;(\text{ex.~} K^0)}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.~} K^0)}}}{(4.851 \pm 0.080) \cdot 10^{-2}}{4.851\cdot 10^{-2}}{0.080\cdot 10^{-2}}%
\htquantdef{Gamma81}{\BR_{81}}{\BRF{\tau^-}{K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(8.727 \pm 1.177) \cdot 10^{-4}}{8.727\cdot 10^{-4}}{1.177\cdot 10^{-4}}%
\htquantdef{Gamma810}{\BR_{810}}{\BRF{\tau^-}{2\pi^- \pi^+ 3\pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(1.931 \pm 0.298) \cdot 10^{-4}}{1.931\cdot 10^{-4}}{0.298\cdot 10^{-4}}%
\htquantdef{Gamma811}{\BR_{811}}{\BRF{\tau^-}{\pi^- 2\pi^0 \omega \nu_\tau ~(\text{ex.~}K^0)}}{(7.139 \pm 1.586) \cdot 10^{-5}}{7.139\cdot 10^{-5}}{1.586\cdot 10^{-5}}%
\htquantdef{Gamma812}{\BR_{812}}{\BRF{\tau^-}{2\pi^- \pi^+ 3\pi^0 \nu_\tau ~(\text{ex.~}K^0, \eta, \omega, f_1)}}{(1.325 \pm 2.682) \cdot 10^{-5}}{1.325\cdot 10^{-5}}{2.682\cdot 10^{-5}}%
\htquantdef{Gamma81by69}{\frac{\BR_{81}}{\BR_{69}}}{\frac{\BRF{\tau^-}{K^- \pi^- h^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}}{(1.931 \pm 0.266) \cdot 10^{-2}}{1.931\cdot 10^{-2}}{0.266\cdot 10^{-2}}%
\htquantdef{Gamma82}{\BR_{82}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(0.4779 \pm 0.0137) \cdot 10^{-2}}{0.4779\cdot 10^{-2}}{0.0137\cdot 10^{-2}}%
\htquantdef{Gamma820}{\BR_{820}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \nu_\tau ~(\text{ex.~}K^0, \omega)}}{(8.242 \pm 0.313) \cdot 10^{-4}}{8.242\cdot 10^{-4}}{0.313\cdot 10^{-4}}%
\htquantdef{Gamma821}{\BR_{821}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \nu_\tau ~(\text{ex.~}K^0, \omega, f_1)}}{(7.719 \pm 0.295) \cdot 10^{-4}}{7.719\cdot 10^{-4}}{0.295\cdot 10^{-4}}%
\htquantdef{Gamma822}{\BR_{822}}{\BRF{\tau^-}{K^- 2\pi^- 2\pi^+ \nu_\tau ~(\text{ex.~}K^0)}}{(0.594 \pm 1.208) \cdot 10^{-6}}{0.594\cdot 10^{-6}}{1.208\cdot 10^{-6}}%
\htquantdef{Gamma83}{\BR_{83}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \ge{} 0\,  \pi^0\, \nu_\tau\;(\text{ex.~} K^0)}}{(0.3741 \pm 0.0135) \cdot 10^{-2}}{0.3741\cdot 10^{-2}}{0.0135\cdot 10^{-2}}%
\htquantdef{Gamma830}{\BR_{830}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(1.630 \pm 0.113) \cdot 10^{-4}}{1.630\cdot 10^{-4}}{0.113\cdot 10^{-4}}%
\htquantdef{Gamma831}{\BR_{831}}{\BRF{\tau^-}{2\pi^- \pi^+ \omega \nu_\tau ~(\text{ex.~}K^0)}}{(8.400 \pm 0.624) \cdot 10^{-5}}{8.400\cdot 10^{-5}}{0.624\cdot 10^{-5}}%
\htquantdef{Gamma832}{\BR_{832}}{\BRF{\tau^-}{3\pi^- 2\pi^+ \pi^0 \nu_\tau ~(\text{ex.~}K^0, \eta, \omega, f_1)}}{(3.775 \pm 0.874) \cdot 10^{-5}}{3.775\cdot 10^{-5}}{0.874\cdot 10^{-5}}%
\htquantdef{Gamma833}{\BR_{833}}{\BRF{\tau^-}{K^- 2\pi^- 2\pi^+ \pi^0 \nu_\tau ~(\text{ex.~}K^0)}}{(1.108 \pm 0.566) \cdot 10^{-6}}{1.108\cdot 10^{-6}}{0.566\cdot 10^{-6}}%
\htquantdef{Gamma84}{\BR_{84}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \nu_\tau}}{(0.3442 \pm 0.0068) \cdot 10^{-2}}{0.3442\cdot 10^{-2}}{0.0068\cdot 10^{-2}}%
\htquantdef{Gamma85}{\BR_{85}}{\BRF{\tau^-}{K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.~} K^0)}}{(0.2929 \pm 0.0067) \cdot 10^{-2}}{0.2929\cdot 10^{-2}}{0.0067\cdot 10^{-2}}%
\htquantdef{Gamma85by60}{\frac{\BR_{85}}{\BR_{60}}}{\frac{\BRF{\tau^-}{K^- \pi^+ \pi^- \nu_\tau\;(\text{ex.~}K^0)}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.~}K^0)}}}{(3.258 \pm 0.074) \cdot 10^{-2}}{3.258\cdot 10^{-2}}{0.074\cdot 10^{-2}}%
\htquantdef{Gamma87}{\BR_{87}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau}}{(0.1329 \pm 0.0119) \cdot 10^{-2}}{0.1329\cdot 10^{-2}}{0.0119\cdot 10^{-2}}%
\htquantdef{Gamma88}{\BR_{88}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}{(8.116 \pm 1.168) \cdot 10^{-4}}{8.116\cdot 10^{-4}}{1.168\cdot 10^{-4}}%
\htquantdef{Gamma89}{\BR_{89}}{\BRF{\tau^-}{K^- \pi^- \pi^+ \pi^0 \nu_\tau\;(\text{ex.~} K^0, \eta)}}{(7.762 \pm 1.168) \cdot 10^{-4}}{7.762\cdot 10^{-4}}{1.168\cdot 10^{-4}}%
\htquantdef{Gamma8by5}{\frac{\BR_{8}}{\BR_{5}}}{\frac{\BRF{\tau^-}{h^- \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{0.6456 \pm 0.0033}{0.6456}{0.0033}%
\htquantdef{Gamma9}{\BR_{9}}{\BRF{\tau^-}{\pi^- \nu_\tau}}{0.10804 \pm 0.00052}{0.10804}{0.00052}%
\htquantdef{Gamma910}{\BR_{910}}{\BRF{\tau^-}{2\pi^- \pi^+ \eta \nu_\tau ~(\eta \to 3\pi^0) ~(\text{ex.~}K^0)}}{(7.176 \pm 0.422) \cdot 10^{-5}}{7.176\cdot 10^{-5}}{0.422\cdot 10^{-5}}%
\htquantdef{Gamma911}{\BR_{911}}{\BRF{\tau^-}{\pi^- 2\pi^0 \eta \nu_\tau ~(\eta \to \pi^+ \pi^- \pi^0) ~(\text{ex.~}K^0)}}{(4.444 \pm 0.867) \cdot 10^{-5}}{4.444\cdot 10^{-5}}{0.867\cdot 10^{-5}}%
\htquantdef{Gamma92}{\BR_{92}}{\BRF{\tau^-}{\pi^- K^- K^+ \ge{} 0\,  \text{neutrals}\, \nu_\tau}}{(0.1493 \pm 0.0033) \cdot 10^{-2}}{0.1493\cdot 10^{-2}}{0.0033\cdot 10^{-2}}%
\htquantdef{Gamma920}{\BR_{920}}{\BRF{\tau^-}{\pi^- f_1 \nu_\tau ~(f_1 \to 2\pi^- 2\pi^+)}}{(5.225 \pm 0.444) \cdot 10^{-5}}{5.225\cdot 10^{-5}}{0.444\cdot 10^{-5}}%
\htquantdef{Gamma93}{\BR_{93}}{\BRF{\tau^-}{\pi^- K^- K^+ \nu_\tau}}{(0.1431 \pm 0.0027) \cdot 10^{-2}}{0.1431\cdot 10^{-2}}{0.0027\cdot 10^{-2}}%
\htquantdef{Gamma930}{\BR_{930}}{\BRF{\tau^-}{2\pi^- \pi^+ \eta \nu_\tau ~(\eta \to \pi^+\pi^-\pi^0) ~(\text{ex.~}K^0)}}{(5.033 \pm 0.296) \cdot 10^{-5}}{5.033\cdot 10^{-5}}{0.296\cdot 10^{-5}}%
\htquantdef{Gamma93by60}{\frac{\BR_{93}}{\BR_{60}}}{\frac{\BRF{\tau^-}{\pi^- K^- K^+ \nu_\tau}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \nu_\tau\;(\text{ex.~} K^0)}}}{(1.592 \pm 0.030) \cdot 10^{-2}}{1.592\cdot 10^{-2}}{0.030\cdot 10^{-2}}%
\htquantdef{Gamma94}{\BR_{94}}{\BRF{\tau^-}{\pi^- K^- K^+ \pi^0 \nu_\tau}}{(6.114 \pm 1.829) \cdot 10^{-5}}{6.114\cdot 10^{-5}}{1.829\cdot 10^{-5}}%
\htquantdef{Gamma944}{\BR_{944}}{\BRF{\tau^-}{2\pi^- \pi^+ \eta \nu_\tau ~(\eta \to \gamma\gamma) ~(\text{ex.~}K^0)}}{(8.654 \pm 0.509) \cdot 10^{-5}}{8.654\cdot 10^{-5}}{0.509\cdot 10^{-5}}%
\htquantdef{Gamma945}{\BR_{945}}{\BRF{\tau^-}{\pi^- 2\pi^0 \eta \nu_\tau}}{(1.939 \pm 0.378) \cdot 10^{-4}}{1.939\cdot 10^{-4}}{0.378\cdot 10^{-4}}%
\htquantdef{Gamma94by69}{\frac{\BR_{94}}{\BR_{69}}}{\frac{\BRF{\tau^-}{\pi^- K^- K^+ \pi^0 \nu_\tau}}{\BRF{\tau^-}{\pi^- \pi^+ \pi^- \pi^0 \nu_\tau\;(\text{ex.~} K^0)}}}{(0.1353 \pm 0.0405) \cdot 10^{-2}}{0.1353\cdot 10^{-2}}{0.0405\cdot 10^{-2}}%
\htquantdef{Gamma96}{\BR_{96}}{\BRF{\tau^-}{K^- K^- K^+ \nu_\tau}}{(2.169 \pm 0.800) \cdot 10^{-5}}{2.169\cdot 10^{-5}}{0.800\cdot 10^{-5}}%
\htquantdef{Gamma998}{\BR_{998}}{1 - \BR_{\text{All}}}{(0.0274 \pm 0.1026) \cdot 10^{-2}}{0.0274\cdot 10^{-2}}{0.1026\cdot 10^{-2}}%
\htquantdef{Gamma9by5}{\frac{\BR_{9}}{\BR_{5}}}{\frac{\BRF{\tau^-}{\pi^- \nu_\tau}}{\BRF{\tau^-}{e^- \bar{\nu}_e \nu_\tau}}}{0.6064 \pm 0.0032}{0.6064}{0.0032}%
\htquantdef{GammaAll}{\BR_{\text{All}}}{\BR_{\text{All}}}{0.9997 \pm 0.0010}{0.9997}{0.0010}%
\htquantdef{gmubyge_tau}{gmubyge_tau}{}{1.0018 \pm 0.0014}{1.0018}{0.0014}%
\htquantdef{gtaubyge_tau}{gtaubyge_tau}{}{1.0029 \pm 0.0014}{1.0029}{0.0014}%
\htquantdef{gtaubygemu_tau}{gtaubygemu_tau}{}{1.0020 \pm 0.0013}{1.0020}{0.0013}%
\htquantdef{gtaubygemu_tau_syst_Be_lept_perc}{gtaubygemu_tau_syst_Be_lept_perc}{}{0.089}{0.089}{0}%
\htquantdef{gtaubygemu_tau_syst_m_tau_perc}{gtaubygemu_tau_syst_m_tau_perc}{}{0.017}{0.017}{0}%
\htquantdef{gtaubygemu_tau_syst_tau_tau_perc}{gtaubygemu_tau_syst_tau_tau_perc}{}{0.086}{0.086}{0}%
\htquantdef{gtaubygemu_tau_unc_perc}{gtaubygemu_tau_unc_perc}{}{0.125}{0.125}{0}%
\htquantdef{gtaubygmu_fit}{gtaubygmu_fit}{}{0.9999 \pm 0.0014}{0.9999}{0.0014}%
\htquantdef{gtaubygmu_K}{gtaubygmu_K}{}{0.9879 \pm 0.0063}{0.9879}{0.0063}%
\htquantdef{gtaubygmu_pi}{gtaubygmu_pi}{}{0.9958 \pm 0.0026}{0.9958}{0.0026}%
\htquantdef{gtaubygmu_piK_fit}{gtaubygmu_piK_fit}{}{0.9947 \pm 0.0025}{0.9947}{0.0025}%
\htquantdef{gtaubygmu_tau}{gtaubygmu_tau}{}{1.0010 \pm 0.0014}{1.0010}{0.0014}%
\htquantdef{hcut}{hcut}{}{(6.626070040 \pm 0.000000081) \cdot 10^{-22}}{6.626070040\cdot 10^{-22}}{0.000000081\cdot 10^{-22}}%
\htquantdef{KmKzsNu}{KmKzsNu}{}{7.400\cdot 10^{-4}}{7.400\cdot 10^{-4}}{0}%
\htquantdef{KmPizKzsNu}{KmPizKzsNu}{}{7.500\cdot 10^{-4}}{7.500\cdot 10^{-4}}{0}%
\htquantdef{KtoENu}{KtoENu}{}{(1.5820 \pm 0.0070) \cdot 10^{-5}}{1.5820\cdot 10^{-5}}{0.0070\cdot 10^{-5}}%
\htquantdef{KtoMuNu}{KtoMuNu}{}{0.6356 \pm 0.0011}{0.6356}{0.0011}%
\htquantdef{m_e}{m_e}{}{0.5109989461 \pm 0.0000000031}{0.5109989461}{0.0000000031}%
\htquantdef{m_K}{m_K}{}{493.677 \pm 0.016}{493.677}{0.016}%
\htquantdef{m_mu}{m_mu}{}{105.6583745 \pm 0.0000024}{105.6583745}{0.0000024}%
\htquantdef{m_pi}{m_pi}{}{139.57061 \pm 0.00024}{139.57061}{0.00024}%
\htquantdef{m_s}{m_s}{}{95.00 \pm 6.70}{95.00}{6.70}%
\htquantdef{m_tau}{m_tau}{}{(1.77686 \pm 0.00012) \cdot 10^{3}}{1.77686\cdot 10^{3}}{0.00012\cdot 10^{3}}%
\htquantdef{m_tau_unc_perc}{m_tau_unc_perc}{}{0.007}{0.007}{0}%
\htquantdef{m_W}{m_W}{}{(8.0379 \pm 0.0012) \cdot 10^{4}}{8.0379\cdot 10^{4}}{0.0012\cdot 10^{4}}%
\htquantdef{MumNuNumb}{MumNuNumb}{}{0.1739}{0.1739}{0}%
\htquantdef{phspf_mebymmu}{phspf_mebymmu}{}{0.9998129491711 \pm 0.0000000000088}{0.9998129491711}{0.0000000000088}%
\htquantdef{phspf_mebymtau}{phspf_mebymtau}{}{0.999999338359 \pm 0.000000000089}{0.999999338359}{0.000000000089}%
\htquantdef{phspf_mmubymtau}{phspf_mmubymtau}{}{0.9725600 \pm 0.0000036}{0.9725600}{0.0000036}%
\htquantdef{pi}{pi}{}{3.142}{3.142}{0}%
\htquantdef{PimKmKpNu}{PimKmKpNu}{}{0.1435\cdot 10^{-2}}{0.1435\cdot 10^{-2}}{0}%
\htquantdef{PimKmPipNu}{PimKmPipNu}{}{0.2930\cdot 10^{-2}}{0.2930\cdot 10^{-2}}{0}%
\htquantdef{PimKzsKzlNu}{PimKzsKzlNu}{}{0.1080\cdot 10^{-2}}{0.1080\cdot 10^{-2}}{0}%
\htquantdef{PimKzsKzsNu}{PimKzsKzsNu}{}{2.330\cdot 10^{-4}}{2.330\cdot 10^{-4}}{0}%
\htquantdef{PimPimPipNu}{PimPimPipNu}{}{8.990\cdot 10^{-2}}{8.990\cdot 10^{-2}}{0}%
\htquantdef{PimPimPipPizNu}{PimPimPipPizNu}{}{4.620\cdot 10^{-2}}{4.620\cdot 10^{-2}}{0}%
\htquantdef{PimPizKzsNu}{PimPizKzsNu}{}{0.1910\cdot 10^{-2}}{0.1910\cdot 10^{-2}}{0}%
\htquantdef{PimPizNu}{PimPizNu}{}{0.2549}{0.2549}{0}%
\htquantdef{pitoENu}{pitoENu}{}{(1.2300 \pm 0.0040) \cdot 10^{-4}}{1.2300\cdot 10^{-4}}{0.0040\cdot 10^{-4}}%
\htquantdef{pitoMuNu}{pitoMuNu}{}{0.99987700 \pm 0.00000040}{0.99987700}{0.00000040}%
\htquantdef{R_tau}{R_tau}{}{3.6355 \pm 0.0081}{3.6355}{0.0081}%
\htquantdef{R_tau_leptonly}{R_tau_leptonly}{}{3.6370 \pm 0.0075}{3.6370}{0.0075}%
\htquantdef{R_tau_leptuniv}{R_tau_leptuniv}{}{3.6409 \pm 0.0070}{3.6409}{0.0070}%
\htquantdef{R_tau_s}{R_tau_s}{}{0.1645 \pm 0.0023}{0.1645}{0.0023}%
\htquantdef{R_tau_uni}{R_tau_uni}{}{3.6370 \pm 0.0075}{3.6370}{0.0075}%
\htquantdef{R_tau_uni_SM}{R_tau_uni_SM}{}{3.6409 \pm 0.0070}{3.6409}{0.0070}%
\htquantdef{R_tau_VA}{R_tau_VA}{}{3.4710 \pm 0.0078}{3.4710}{0.0078}%
\htquantdef{Rrad_mu_gamma}{Rrad_mu_gamma}{}{0.9958}{0.9958}{0}%
\htquantdef{Rrad_mu_W}{Rrad_mu_W}{}{1.00000103682 \pm 0.00000000031}{1.00000103682}{0.00000000031}%
\htquantdef{Rrad_SEW_tau_Knu}{Rrad_SEW_tau_Knu}{}{1.02010 \pm 0.00030}{1.02010}{0.00030}%
\htquantdef{Rrad_tau_gamma}{Rrad_tau_gamma}{}{0.9957}{0.9957}{0}%
\htquantdef{Rrad_tau_W}{Rrad_tau_W}{}{1.000296316 \pm 0.000000097}{1.000296316}{0.000000097}%
\htquantdef{Rrad_tauK_by_taupi}{Rrad_tauK_by_taupi}{}{1.00 \pm 0.00}{1.00}{0.00}%
\htquantdef{sigmataupmy4s}{sigmataupmy4s}{}{0.9190}{0.9190}{0}%
\htquantdef{tau_K}{tau_K}{}{(1.2380 \pm 0.0020) \cdot 10^{-8}}{1.2380\cdot 10^{-8}}{0.0020\cdot 10^{-8}}%
\htquantdef{tau_mu}{tau_mu}{}{(2.196981 \pm 0.000022) \cdot 10^{-6}}{2.196981\cdot 10^{-6}}{0.000022\cdot 10^{-6}}%
\htquantdef{tau_pi}{tau_pi}{}{(2.60330 \pm 0.00050) \cdot 10^{-8}}{2.60330\cdot 10^{-8}}{0.00050\cdot 10^{-8}}%
\htquantdef{tau_tau}{tau_tau}{}{290.3 \pm 0.5}{290.3}{0.5}%
\htquantdef{tau_tau_unc_perc}{tau_tau_unc_perc}{}{0.172}{0.172}{0}%
\htquantdef{Vub}{Vub}{}{(0.3940 \pm 0.0360) \cdot 10^{-2}}{0.3940\cdot 10^{-2}}{0.0360\cdot 10^{-2}}%
\htquantdef{Vud}{Vud}{}{0.97420 \pm 0.00021}{0.97420}{0.00021}%
\htquantdef{Vus}{Vus}{}{0.2195 \pm 0.0019}{0.2195}{0.0019}%
\htquantdef{Vus_by_Vud_tauKpi}{Vus_by_Vud_tauKpi}{}{0.2295 \pm 0.0016}{0.2295}{0.0016}%
\htquantdef{Vus_err_exp}{Vus_err_exp}{}{0.1576\cdot 10^{-2}}{0.1576\cdot 10^{-2}}{0}%
\htquantdef{Vus_err_exp_perc}{Vus_err_exp_perc}{}{0.7180}{0.7180}{0}%
\htquantdef{Vus_err_perc}{Vus_err_perc}{}{0.8672}{0.8672}{0}%
\htquantdef{Vus_err_th}{Vus_err_th}{}{0.0011}{0.0011}{0}%
\htquantdef{Vus_err_th_perc}{Vus_err_th_perc}{}{0.49}{0.49}{0}%
\htquantdef{Vus_mism}{Vus_mism}{}{(-0.6180 \pm 0.2122) \cdot 10^{-2}}{-0.6180\cdot 10^{-2}}{0.2122\cdot 10^{-2}}%
\htquantdef{Vus_mism_sigma}{Vus_mism_sigma}{}{-2.9}{-2.9}{0}%
\htquantdef{Vus_mism_sigma_abs}{Vus_mism_sigma_abs}{}{2.9}{2.9}{0}%
\htquantdef{Vus_tau}{Vus_tau}{}{0.2221 \pm 0.0013}{0.2221}{0.0013}%
\htquantdef{Vus_tau_mism}{Vus_tau_mism}{}{(-0.3517 \pm 0.1569) \cdot 10^{-2}}{-0.3517\cdot 10^{-2}}{0.1569\cdot 10^{-2}}%
\htquantdef{Vus_tau_mism_sigma}{Vus_tau_mism_sigma}{}{-2.2}{-2.2}{0}%
\htquantdef{Vus_tau_mism_sigma_abs}{Vus_tau_mism_sigma_abs}{}{2.2}{2.2}{0}%
\htquantdef{Vus_tau2}{Vus_tau2}{}{0.2221 \pm 0.0013}{0.2221}{0.0013}%
\htquantdef{Vus_tau2_mism}{Vus_tau2_mism}{}{(-0.3517 \pm 0.1569) \cdot 10^{-2}}{-0.3517\cdot 10^{-2}}{0.1569\cdot 10^{-2}}%
\htquantdef{Vus_tau2_mism_sigma}{Vus_tau2_mism_sigma}{}{-2.2}{-2.2}{0}%
\htquantdef{Vus_tau2_mism_sigma_abs}{Vus_tau2_mism_sigma_abs}{}{2.2}{2.2}{0}%
\htquantdef{Vus_tauKnu}{Vus_tauKnu}{}{0.2234 \pm 0.0015}{0.2234}{0.0015}%
\htquantdef{Vus_tauKnu_err_th_perc}{Vus_tauKnu_err_th_perc}{}{0.2445}{0.2445}{0}%
\htquantdef{Vus_tauKnu_mism}{Vus_tauKnu_mism}{}{(-0.2300 \pm 0.1726) \cdot 10^{-2}}{-0.2300\cdot 10^{-2}}{0.1726\cdot 10^{-2}}%
\htquantdef{Vus_tauKnu_mism_sigma}{Vus_tauKnu_mism_sigma}{}{-1.3}{-1.3}{0}%
\htquantdef{Vus_tauKnu_mism_sigma_abs}{Vus_tauKnu_mism_sigma_abs}{}{1.3}{1.3}{0}%
\htquantdef{Vus_tauKpi}{Vus_tauKpi}{}{0.2236 \pm 0.0015}{0.2236}{0.0015}%
\htquantdef{Vus_tauKpi_err_th_perc}{Vus_tauKpi_err_th_perc}{}{0.2224}{0.2224}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_dRrad_kmunu_by_pimunu}{Vus_tauKpi_err_th_perc_dRrad_kmunu_by_pimunu}{}{-8.559\cdot 10^{-2}}{-8.559\cdot 10^{-2}}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_dRrad_tauK_by_Kmu}{Vus_tauKpi_err_th_perc_dRrad_tauK_by_Kmu}{}{-0.1090}{-0.1090}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_dRrad_taupi_by_pimu}{Vus_tauKpi_err_th_perc_dRrad_taupi_by_pimu}{}{6.989\cdot 10^{-2}}{6.989\cdot 10^{-2}}{0}%
\htquantdef{Vus_tauKpi_err_th_perc_f_Kpm_by_f_pipm}{Vus_tauKpi_err_th_perc_f_Kpm_by_f_pipm}{}{-0.1592}{-0.1592}{0}%
\htquantdef{Vus_tauKpi_mism}{Vus_tauKpi_mism}{}{(-0.2098 \pm 0.1802) \cdot 10^{-2}}{-0.2098\cdot 10^{-2}}{0.1802\cdot 10^{-2}}%
\htquantdef{Vus_tauKpi_mism_sigma}{Vus_tauKpi_mism_sigma}{}{-1.2}{-1.2}{0}%
\htquantdef{Vus_tauKpi_mism_sigma_abs}{Vus_tauKpi_mism_sigma_abs}{}{1.2}{1.2}{0}%
\htquantdef{Vus_uni}{Vus_uni}{}{0.22565 \pm 0.00089}{0.22565}{0.00089}%
\htdef{couplingsCorr}{%
$\left( \frac{g_\tau}{g_e} \right)$ &   51\\
$\left( \frac{g_\mu}{g_e} \right)$ &  -50 &   49\\
$\left( \frac{g_\tau}{g_\mu} \right)_\pi$ &   23 &   25 &    2\\
$\left( \frac{g_\tau}{g_\mu} \right)_K$ &   11 &   10 &   -1 &    6\\
 & $\left( \frac{g_\tau}{g_\mu} \right)$ & $\left( \frac{g_\tau}{g_e} \right)$ & $\left( \frac{g_\mu}{g_e} \right)$ & $\left( \frac{g_\tau}{g_\mu} \right)_\pi$}%


==> tau/hflav-2018.tex <==
\htdef{UnitarityResid}{(0.03 \pm 0.10)\%}%
\htdef{MeasNum}{176}%
\htdef{QuantNum}{136}%
\htdef{QuantNumNonRatio}{119}%
\htdef{QuantNumRatio}{17}%
\htdef{QuantNumWithMeas}{86}%
\htdef{QuantNumNonRatioWithMeas}{73}%
\htdef{QuantNumRatioWithMeas}{13}%
\htdef{QuantNumPdg}{130}%
\htdef{QuantNumNonRatioPdg}{113}%
\htdef{QuantNumRatioPdg}{17}%
\htdef{QuantNumWithMeasPdg}{84}%
\htdef{QuantNumNonRatioWithMeasPdg}{71}%
\htdef{QuantNumRatioWithMeasPdg}{13}%
\htdef{IndepQuantNum}{47}%
\htdef{BaseQuantNum}{47}%
\htdef{UnitarityQuantNum}{48}%
\htdef{ConstrNum}{89}%
\htdef{ConstrNumPdg}{83}%
\htdef{Chisq}{142}%
\htdef{Dof}{129}%
\htdef{ChisqProb}{20.13\%}%
\htdef{ChisqProbRound}{20\%}%
\htmeasdef{ALEPH.Gamma10.pub.BARATE.99K}{Gamma10}{ALEPH}{Barate:1999hi}{0.00696 \pm 0.00025 \pm 0.00014}{0.00696}{\pm 0.00025}{0.00014}%
\htmeasdef{ALEPH.Gamma103.pub.SCHAEL.05C}{Gamma103}{ALEPH}{Schael:2005am}{0.00072 \pm 0.00009 \pm 0.00012}{0.00072}{\pm 0.00009}{0.00012}%
\htmeasdef{ALEPH.Gamma104.pub.SCHAEL.05C}{Gamma104}{ALEPH}{Schael:2005am}{( 0.021 \pm 0.007 \pm 0.009 ) \cdot 10^{ -2 }}{0.021e-2}{\pm 0.007e-2}{0.009e-2}%
\htmeasdef{ALEPH.Gamma126.pub.BUSKULIC.97C}{Gamma126}{ALEPH}{Buskulic:1996qs}{0.0018 \pm 0.0004 \pm 0.0002}{0.0018}{\pm 0.0004}{0.0002}%
\htmeasdef{ALEPH.Gamma128.pub.BUSKULIC.97C}{Gamma128}{ALEPH}{Buskulic:1996qs}{( 2.9 {}^{+1.3\cdot 10^{-4}}_{-1.2} \pm 0.7 ) \cdot 10^{ -4 }}{2.9e-4}{{}^{+1.3e-4}_{-1.2e-4}}{0.7e-4}%
\htmeasdef{ALEPH.Gamma13.pub.SCHAEL.05C}{Gamma13}{ALEPH}{Schael:2005am}{( 25.924 \pm 0.097 \pm 0.085 ) \cdot 10^{ -2 }}{25.924e-2}{\pm 0.097e-2}{0.085e-2}%
\htmeasdef{ALEPH.Gamma150.pub.BUSKULIC.97C}{Gamma150}{ALEPH}{Buskulic:1996qs}{0.0191 \pm 0.0007 \pm 0.0006}{0.0191}{\pm 0.0007}{0.0006}%
\htmeasdef{ALEPH.Gamma150by66.pub.BUSKULIC.96}{Gamma150by66}{ALEPH}{Buskulic:1995ty}{0.431 \pm 0.033}{0.431}{\pm 0.033}{0}%
\htmeasdef{ALEPH.Gamma152.pub.BUSKULIC.97C}{Gamma152}{ALEPH}{Buskulic:1996qs}{0.0043 \pm 0.0006 \pm 0.0005}{0.0043}{\pm 0.0006}{0.0005}%
\htmeasdef{ALEPH.Gamma16.pub.BARATE.99K}{Gamma16}{ALEPH}{Barate:1999hi}{0.00444 \pm 0.00026 \pm 0.00024}{0.00444}{\pm 0.00026}{0.00024}%
\htmeasdef{ALEPH.Gamma19.pub.SCHAEL.05C}{Gamma19}{ALEPH}{Schael:2005am}{( 9.295 \pm 0.084 \pm 0.088 ) \cdot 10^{ -2 }}{9.295e-2}{\pm 0.084e-2}{0.088e-2}%
\htmeasdef{ALEPH.Gamma23.pub.BARATE.99K}{Gamma23}{ALEPH}{Barate:1999hi}{0.00056 \pm 0.0002 \pm 0.00015}{0.00056}{\pm 0.0002}{0.00015}%
\htmeasdef{ALEPH.Gamma26.pub.SCHAEL.05C}{Gamma26}{ALEPH}{Schael:2005am}{( 1.08200 \pm 0.0709295 \pm 0.0594643 ) \cdot 10^{ -2 }}{1.08200e-2}{\pm 0.0709295e-2}{0.0594643e-2}%
\htmeasdef{ALEPH.Gamma28.pub.BARATE.99K}{Gamma28}{ALEPH}{Barate:1999hi}{0.00037 \pm 0.00021 \pm 0.00011}{0.00037}{\pm 0.00021}{0.00011}%
\htmeasdef{ALEPH.Gamma3.pub.SCHAEL.05C}{Gamma3}{ALEPH}{Schael:2005am}{0.17319 \pm 0.0007 \pm 0.00032}{0.17319}{\pm 0.0007}{0.00032}%
\htmeasdef{ALEPH.Gamma30.pub.SCHAEL.05C}{Gamma30}{ALEPH}{Schael:2005am}{0.00112 \pm 0.00037 \pm 0.00035}{0.00112}{\pm 0.00037}{0.00035}%
\htmeasdef{ALEPH.Gamma33.pub.BARATE.98E}{Gamma33}{ALEPH}{Barate:1997tt}{0.0097 \pm 0.00058 \pm 0.00062}{0.0097}{\pm 0.00058}{0.00062}%
\htmeasdef{ALEPH.Gamma35.pub.BARATE.99K}{Gamma35}{ALEPH}{Barate:1999hi}{0.00928 \pm 0.00045 \pm 0.00034}{0.00928}{\pm 0.00045}{0.00034}%
\htmeasdef{ALEPH.Gamma37.pub.BARATE.98E}{Gamma37}{ALEPH}{Barate:1997tt}{0.00158 \pm 0.00042 \pm 0.00017}{0.00158}{\pm 0.00042}{0.00017}%
\htmeasdef{ALEPH.Gamma37.pub.BARATE.99K}{Gamma37}{ALEPH}{Barate:1999hi}{0.00162 \pm 0.00021 \pm 0.00011}{0.00162}{\pm 0.00021}{0.00011}%
\htmeasdef{ALEPH.Gamma40.pub.BARATE.98E}{Gamma40}{ALEPH}{Barate:1997tt}{0.00294 \pm 0.00073 \pm 0.00037}{0.00294}{\pm 0.00073}{0.00037}%
\htmeasdef{ALEPH.Gamma40.pub.BARATE.99K}{Gamma40}{ALEPH}{Barate:1999hi}{0.00347 \pm 0.00053 \pm 0.00037}{0.00347}{\pm 0.00053}{0.00037}%
\htmeasdef{ALEPH.Gamma42.pub.BARATE.98E}{Gamma42}{ALEPH}{Barate:1997tt}{0.00152 \pm 0.00076 \pm 0.00021}{0.00152}{\pm 0.00076}{0.00021}%
\htmeasdef{ALEPH.Gamma42.pub.BARATE.99K}{Gamma42}{ALEPH}{Barate:1999hi}{0.00143 \pm 0.00025 \pm 0.00015}{0.00143}{\pm 0.00025}{0.00015}%
\htmeasdef{ALEPH.Gamma44.pub.BARATE.99R}{Gamma44}{ALEPH}{Barate:1999hj}{0.00026 \pm 0.00024}{0.00026}{\pm 0.00024}{0}%
\htmeasdef{ALEPH.Gamma47.pub.BARATE.98E}{Gamma47}{ALEPH}{Barate:1997tt}{0.00026 \pm 0.0001 \pm 5\cdot 10^{-5}}{0.00026}{\pm 0.0001}{5e-05}%
\htmeasdef{ALEPH.Gamma48.pub.BARATE.98E}{Gamma48}{ALEPH}{Barate:1997tt}{0.00101 \pm 0.00023 \pm 0.00013}{0.00101}{\pm 0.00023}{0.00013}%
\htmeasdef{ALEPH.Gamma5.pub.SCHAEL.05C}{Gamma5}{ALEPH}{Schael:2005am}{0.17837 \pm 0.00072 \pm 0.00036}{0.17837}{\pm 0.00072}{0.00036}%
\htmeasdef{ALEPH.Gamma51.pub.BARATE.98E}{Gamma51}{ALEPH}{Barate:1997tt}{( 3.1 \pm 1.1 \pm 0.5 ) \cdot 10^{ -4 }}{3.1e-4}{\pm 1.1e-4}{0.5e-4}%
\htmeasdef{ALEPH.Gamma53.pub.BARATE.98E}{Gamma53}{ALEPH}{Barate:1997tt}{0.00023 \pm 0.00019 \pm 0.00007}{0.00023}{\pm 0.00019}{0.00007}%
\htmeasdef{ALEPH.Gamma58.pub.SCHAEL.05C}{Gamma58}{ALEPH}{Schael:2005am}{0.09469 \pm 0.00062 \pm 0.00073}{0.09469}{\pm 0.00062}{0.00073}%
\htmeasdef{ALEPH.Gamma66.pub.SCHAEL.05C}{Gamma66}{ALEPH}{Schael:2005am}{0.04734 \pm 0.00059 \pm 0.00049}{0.04734}{\pm 0.00059}{0.00049}%
\htmeasdef{ALEPH.Gamma76.pub.SCHAEL.05C}{Gamma76}{ALEPH}{Schael:2005am}{0.00435 \pm 0.0003 \pm 0.00035}{0.00435}{\pm 0.0003}{0.00035}%
\htmeasdef{ALEPH.Gamma8.pub.SCHAEL.05C}{Gamma8}{ALEPH}{Schael:2005am}{( 11.524 \pm 0.070 \pm 0.078 ) \cdot 10^{ -2 }}{11.524e-2}{\pm 0.070e-2}{0.078e-2}%
\htmeasdef{ALEPH.Gamma805.pub.SCHAEL.05C}{Gamma805}{ALEPH}{Schael:2005am}{( 4 \pm 2 ) \cdot 10^{ -4 }}{4e-04}{\pm 2e-04}{0}%
\htmeasdef{ALEPH.Gamma85.pub.BARATE.98}{Gamma85}{ALEPH}{Barate:1997ma}{0.00214 \pm 0.00037 \pm 0.00029}{0.00214}{\pm 0.00037}{0.00029}%
\htmeasdef{ALEPH.Gamma88.pub.BARATE.98}{Gamma88}{ALEPH}{Barate:1997ma}{0.00061 \pm 0.00039 \pm 0.00018}{0.00061}{\pm 0.00039}{0.00018}%
\htmeasdef{ALEPH.Gamma93.pub.BARATE.98}{Gamma93}{ALEPH}{Barate:1997ma}{0.00163 \pm 0.00021 \pm 0.00017}{0.00163}{\pm 0.00021}{0.00017}%
\htmeasdef{ALEPH.Gamma94.pub.BARATE.98}{Gamma94}{ALEPH}{Barate:1997ma}{0.00075 \pm 0.00029 \pm 0.00015}{0.00075}{\pm 0.00029}{0.00015}%
\htmeasdef{ARGUS.Gamma103.pub.ALBRECHT.88B}{Gamma103}{ARGUS}{Albrecht:1987zf}{0.00064 \pm 0.00023 \pm 0.0001}{0.00064}{\pm 0.00023}{0.0001}%
\htmeasdef{ARGUS.Gamma3by5.pub.ALBRECHT.92D}{Gamma3by5}{ARGUS}{Albrecht:1991rh}{0.997 \pm 0.035 \pm 0.04}{0.997}{\pm 0.035}{0.04}%
\htmeasdef{BaBar.Gamma10.prelim.ICHEP2018}{Gamma10}{\babar}{Lusiani:2019mis}{( 7.17 \pm 0.031 \pm 0.21 ) \cdot 10^{ -3 }}{7.17e-03}{\pm 0.031e-03}{0.21e-03}%
\htmeasdef{BaBar.Gamma10by5.pub.AUBERT.10F}{Gamma10by5}{\babar}{Aubert:2009qj}{0.03882 \pm 0.00032 \pm 0.00057}{0.03882}{\pm 0.00032}{0.00057}%
\htmeasdef{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E}{Gamma128}{\babar}{delAmoSanchez:2010pc}{0.000142 \pm 1.1\cdot 10^{-5} \pm 7\cdot 10^{-6}}{0.000142}{\pm 1.1e-05}{7e-06}%
\htmeasdef{BaBar.Gamma16.prelim.ICHEP2018}{Gamma16}{\babar}{Lusiani:2019mis}{( 5.05 \pm 0.02 \pm 0.15 ) \cdot 10^{ -3 }}{5.05e-03}{\pm 0.02e-03}{0.15e-03}%
\htmeasdef{BaBar.Gamma23.prelim.ICHEP2018}{Gamma23}{\babar}{Lusiani:2019mis}{( 6.15 \pm 0.12 \pm 0.34 ) \cdot 10^{ -4 }}{6.15e-04}{\pm 0.12e-04}{0.34e-04}%
\htmeasdef{BaBar.Gamma27.prelim.ICHEP2018}{Gamma27}{\babar}{Lusiani:2019mis}{( 1.168 \pm 0.006 \pm 0.038 ) \cdot 10^{ -2 }}{1.168e-02}{\pm 0.006e-02}{0.038e-02}%
\htmeasdef{BaBar.Gamma28.prelim.ICHEP2018}{Gamma28}{\babar}{Lusiani:2019mis}{( 1.25 \pm 0.16 \pm 0.24 ) \cdot 10^{ -4 }}{1.25e-04}{\pm 0.16e-04}{0.24e-04}%
\htmeasdef{BaBar.Gamma37.pub.LEES.18B}{Gamma37}{\babar}{BaBar:2018qry}{( 14.78 \pm 0.22 \pm 0.40 ) \cdot 10^{ -4 }}{14.78e-4}{\pm 0.22e-4}{0.40e-4}%
\htmeasdef{BaBar.Gamma3by5.pub.AUBERT.10F}{Gamma3by5}{\babar}{Aubert:2009qj}{0.9796 \pm 0.0016 \pm 0.0036}{0.9796}{\pm 0.0016}{0.0036}%
\htmeasdef{BaBar.Gamma47.pub.LEES.12Y}{Gamma47}{\babar}{Lees:2012de}{( 2.31 \pm 0.04 \pm 0.08 ) \cdot 10^{ -4 }}{2.31e-4}{\pm 0.04e-4}{0.08e-4}%
\htmeasdef{BaBar.Gamma50.pub.LEES.12Y}{Gamma50}{\babar}{Lees:2012de}{( 1.60 \pm 0.20 \pm 0.22 ) \cdot 10^{ -5 }}{1.60e-5}{\pm 0.20e-5}{0.22e-5}%
\htmeasdef{BaBar.Gamma60.pub.AUBERT.08}{Gamma60}{\babar}{Aubert:2007mh}{0.0883 \pm 0.0001 \pm 0.0013}{0.0883}{\pm 0.0001}{0.0013}%
\htmeasdef{BaBar.Gamma809.prelim.ICHEP2018}{Gamma809}{\babar}{Lusiani:2019mis}{( 9.02 \pm 0.40 \pm 0.65 ) \cdot 10^{ -4 }}{9.02e-04}{\pm 0.40e-04}{0.65e-04}%
\htmeasdef{BaBar.Gamma811.pub.LEES.12X}{Gamma811}{\babar}{Lees:2012ks}{( 7.3 \pm 1.2 \pm 1.2 ) \cdot 10^{ -5 }}{7.3e-5}{\pm 1.2e-5}{1.2e-5}%
\htmeasdef{BaBar.Gamma812.pub.LEES.12X}{Gamma812}{\babar}{Lees:2012ks}{( 0.1 \pm 0.08 \pm 0.30 ) \cdot 10^{ -4 }}{0.1e-4}{\pm 0.08e-4}{0.30e-4}%
\htmeasdef{BaBar.Gamma821.pub.LEES.12X}{Gamma821}{\babar}{Lees:2012ks}{( 7.68 \pm 0.04 \pm 0.40 ) \cdot 10^{ -4 }}{7.68e-4}{\pm 0.04e-4}{0.40e-4}%
\htmeasdef{BaBar.Gamma822.pub.LEES.12X}{Gamma822}{\babar}{Lees:2012ks}{( 0.6 \pm 0.5 \pm 1.1 ) \cdot 10^{ -6 }}{0.6e-06}{\pm 0.5e-06}{1.1e-06}%
\htmeasdef{BaBar.Gamma831.pub.LEES.12X}{Gamma831}{\babar}{Lees:2012ks}{( 8.4 \pm 0.4 \pm 0.6 ) \cdot 10^{ -5 }}{8.4e-5}{\pm 0.4e-5}{0.6e-5}%
\htmeasdef{BaBar.Gamma832.pub.LEES.12X}{Gamma832}{\babar}{Lees:2012ks}{( 0.36 \pm 0.03 \pm 0.09 ) \cdot 10^{ -4 }}{0.36e-4}{\pm 0.03e-4}{0.09e-4}%
\htmeasdef{BaBar.Gamma833.pub.LEES.12X}{Gamma833}{\babar}{Lees:2012ks}{( 1.1 \pm 0.4 \pm 0.4 ) \cdot 10^{ -6 }}{1.1e-6}{\pm 0.4e-6}{0.4e-6}%
\htmeasdef{BaBar.Gamma85.pub.AUBERT.08}{Gamma85}{\babar}{Aubert:2007mh}{0.00273 \pm 2\cdot 10^{-5} \pm 9\cdot 10^{-5}}{0.00273}{\pm 2e-05}{9e-05}%
\htmeasdef{BaBar.Gamma910.pub.LEES.12X}{Gamma910}{\babar}{Lees:2012ks}{( 8.27 \pm 0.88 \pm 0.81 ) \cdot 10^{ -5 }}{8.27e-5}{\pm 0.88e-5}{0.81e-5}%
\htmeasdef{BaBar.Gamma911.pub.LEES.12X}{Gamma911}{\babar}{Lees:2012ks}{( 4.57 \pm 0.77 \pm 0.50 ) \cdot 10^{ -5 }}{4.57e-5}{\pm 0.77e-5}{0.50e-5}%
\htmeasdef{BaBar.Gamma920.pub.LEES.12X}{Gamma920}{\babar}{Lees:2012ks}{( 5.20 \pm 0.31 \pm 0.37 ) \cdot 10^{ -5 }}{5.20e-5}{\pm 0.31e-5}{0.37e-5}%
\htmeasdef{BaBar.Gamma93.pub.AUBERT.08}{Gamma93}{\babar}{Aubert:2007mh}{0.001346 \pm 1\cdot 10^{-5} \pm 3.6\cdot 10^{-5}}{0.001346}{\pm 1e-05}{3.6e-05}%
\htmeasdef{BaBar.Gamma930.pub.LEES.12X}{Gamma930}{\babar}{Lees:2012ks}{( 5.39 \pm 0.27 \pm 0.41 ) \cdot 10^{ -5 }}{5.39e-5}{\pm 0.27e-5}{0.41e-5}%
\htmeasdef{BaBar.Gamma944.pub.LEES.12X}{Gamma944}{\babar}{Lees:2012ks}{( 8.26 \pm 0.35 \pm 0.51 ) \cdot 10^{ -5 }}{8.26e-5}{\pm 0.35e-5}{0.51e-5}%
\htmeasdef{BaBar.Gamma96.pub.AUBERT.08}{Gamma96}{\babar}{Aubert:2007mh}{1.5777\cdot 10^{-5} \pm 1.3\cdot 10^{-6} \pm 1.2308\cdot 10^{-6}}{1.5777e-05}{\pm 1.3e-06}{1.2308e-06}%
\htmeasdef{BaBar.Gamma9by5.pub.AUBERT.10F}{Gamma9by5}{\babar}{Aubert:2009qj}{0.5945 \pm 0.0014 \pm 0.0061}{0.5945}{\pm 0.0014}{0.0061}%
\htmeasdef{Belle.Gamma126.pub.INAMI.09}{Gamma126}{Belle}{Inami:2008ar}{0.00135 \pm 3\cdot 10^{-5} \pm 7\cdot 10^{-5}}{0.00135}{\pm 3e-05}{7e-05}%
\htmeasdef{Belle.Gamma128.pub.INAMI.09}{Gamma128}{Belle}{Inami:2008ar}{0.000158 \pm 5\cdot 10^{-6} \pm 9\cdot 10^{-6}}{0.000158}{\pm 5e-06}{9e-06}%
\htmeasdef{Belle.Gamma13.pub.FUJIKAWA.08}{Gamma13}{Belle}{Fujikawa:2008ma}{0.2567 \pm 1\cdot 10^{-4} \pm 0.0039}{0.2567}{\pm 1e-04}{0.0039}%
\htmeasdef{Belle.Gamma130.pub.INAMI.09}{Gamma130}{Belle}{Inami:2008ar}{4.6\cdot 10^{-5} \pm 1.1\cdot 10^{-5} \pm 4\cdot 10^{-6}}{4.6e-05}{\pm 1.1e-05}{4e-06}%
\htmeasdef{Belle.Gamma132.pub.INAMI.09}{Gamma132}{Belle}{Inami:2008ar}{8.8\cdot 10^{-5} \pm 1.4\cdot 10^{-5} \pm 6\cdot 10^{-6}}{8.8e-05}{\pm 1.4e-05}{6e-06}%
\htmeasdef{Belle.Gamma35.pub.RYU.14vpc}{Gamma35}{Belle}{Ryu:2014vpc}{8.32\cdot 10^{-3} \pm 0.3\% \pm 1.8\%}{8.32e-03}{\pm 0.3\%}{1.8\%}%
\htmeasdef{Belle.Gamma37.pub.RYU.14vpc}{Gamma37}{Belle}{Ryu:2014vpc}{14.8\cdot 10^{-4} \pm 0.9\% \pm 3.7\%}{14.8e-04}{\pm 0.9\%}{3.7\%}%
\htmeasdef{Belle.Gamma40.pub.RYU.14vpc}{Gamma40}{Belle}{Ryu:2014vpc}{3.86\cdot 10^{-3} \pm 0.8\% \pm 3.5\%}{3.86e-03}{\pm 0.8\%}{3.5\%}%
\htmeasdef{Belle.Gamma42.pub.RYU.14vpc}{Gamma42}{Belle}{Ryu:2014vpc}{14.96\cdot 10^{-4} \pm 1.3\% \pm 4.9\%}{14.96e-04}{\pm 1.3\%}{4.9\%}%
\htmeasdef{Belle.Gamma47.pub.RYU.14vpc}{Gamma47}{Belle}{Ryu:2014vpc}{2.33\cdot 10^{-4} \pm 1.4\% \pm 4.0\%}{2.33e-04}{\pm 1.4\%}{4.0\%}%
\htmeasdef{Belle.Gamma50.pub.RYU.14vpc}{Gamma50}{Belle}{Ryu:2014vpc}{2.00\cdot 10^{-5} \pm 10.8\% \pm 10.1\%}{2.00e-05}{\pm 10.8\%}{10.1\%}%
\htmeasdef{Belle.Gamma60.pub.LEE.10}{Gamma60}{Belle}{Lee:2010tc}{0.0842 \pm 0 {}^{+0.0026}_{-0.0025}}{0.0842}{\pm 0}{{}^{+0.0026}_{-0.0025}}%
\htmeasdef{Belle.Gamma85.pub.LEE.10}{Gamma85}{Belle}{Lee:2010tc}{0.0033 \pm 1\cdot 10^{-5} {}^{+0.00016}_{-0.00017}}{0.0033}{\pm 1e-05}{{}^{+0.00016}_{-0.00017}}%
\htmeasdef{Belle.Gamma93.pub.LEE.10}{Gamma93}{Belle}{Lee:2010tc}{0.00155 \pm 1\cdot 10^{-5} {}^{+6\cdot 10^{-5}}_{-5\cdot 10^{-5}}}{0.00155}{\pm 1e-05}{{}^{+6e-05}_{-5e-05}}%
\htmeasdef{Belle.Gamma96.pub.LEE.10}{Gamma96}{Belle}{Lee:2010tc}{3.29\cdot 10^{-5} \pm 1.7\cdot 10^{-6} {}^{+1.9\cdot 10^{-6}}_{-2.0\cdot 10^{-6}}}{3.29e-05}{\pm 1.7e-06}{{}^{+1.9e-06}_{-2.0e-06}}%
\htmeasdef{CELLO.Gamma54.pub.BEHREND.89B}{Gamma54}{CELLO}{Behrend:1989wc}{0.15 \pm 0.004 \pm 0.003}{0.15}{\pm 0.004}{0.003}%
\htmeasdef{CLEO.Gamma10.pub.BATTLE.94}{Gamma10}{CLEO}{Battle:1994by}{0.0066 \pm 0.0007 \pm 0.0009}{0.0066}{\pm 0.0007}{0.0009}%
\htmeasdef{CLEO.Gamma102.pub.GIBAUT.94B}{Gamma102}{CLEO}{Gibaut:1994ik}{0.00097 \pm 5\cdot 10^{-5} \pm 0.00011}{0.00097}{\pm 5e-05}{0.00011}%
\htmeasdef{CLEO.Gamma103.pub.GIBAUT.94B}{Gamma103}{CLEO}{Gibaut:1994ik}{0.00077 \pm 5\cdot 10^{-5} \pm 9\cdot 10^{-5}}{0.00077}{\pm 5e-05}{9e-05}%
\htmeasdef{CLEO.Gamma104.pub.ANASTASSOV.01}{Gamma104}{CLEO}{Anastassov:2000xu}{0.00017 \pm 2\cdot 10^{-5} \pm 2\cdot 10^{-5}}{0.00017}{\pm 2e-05}{2e-05}%
\htmeasdef{CLEO.Gamma126.pub.ARTUSO.92}{Gamma126}{CLEO}{Artuso:1992qu}{0.0017 \pm 0.0002 \pm 0.0002}{0.0017}{\pm 0.0002}{0.0002}%
\htmeasdef{CLEO.Gamma128.pub.BARTELT.96}{Gamma128}{CLEO}{Bartelt:1996iv}{( 2.6 \pm 0.5 \pm 0.5 ) \cdot 10^{ -4 }}{2.6e-4}{\pm 0.5e-4}{0.5e-4}%
\htmeasdef{CLEO.Gamma13.pub.ARTUSO.94}{Gamma13}{CLEO}{Artuso:1994ii}{0.2587 \pm 0.0012 \pm 0.0042}{0.2587}{\pm 0.0012}{0.0042}%
\htmeasdef{CLEO.Gamma130.pub.BISHAI.99}{Gamma130}{CLEO}{Bishai:1998gf}{( 1.77 \pm 0.56 \pm 0.71 ) \cdot 10^{ -4 }}{1.77e-4}{\pm 0.56e-4}{0.71e-4}%
\htmeasdef{CLEO.Gamma132.pub.BISHAI.99}{Gamma132}{CLEO}{Bishai:1998gf}{( 2.2 \pm 0.70 \pm 0.22 ) \cdot 10^{ -4 }}{2.2e-4}{\pm 0.70e-4}{0.22e-4}%
\htmeasdef{CLEO.Gamma150.pub.BARINGER.87}{Gamma150}{CLEO}{Baringer:1987tr}{0.016 \pm 0.0027 \pm 0.0041}{0.016}{\pm 0.0027}{0.0041}%
\htmeasdef{CLEO.Gamma150by66.pub.BALEST.95C}{Gamma150by66}{CLEO}{Balest:1995kq}{0.464 \pm 0.016 \pm 0.017}{0.464}{\pm 0.016}{0.017}%
\htmeasdef{CLEO.Gamma152by76.pub.BORTOLETTO.93}{Gamma152by76}{CLEO}{Bortoletto:1993px}{0.81 \pm 0.06 \pm 0.06}{0.81}{\pm 0.06}{0.06}%
\htmeasdef{CLEO.Gamma16.pub.BATTLE.94}{Gamma16}{CLEO}{Battle:1994by}{0.0051 \pm 0.001 \pm 0.0007}{0.0051}{\pm 0.001}{0.0007}%
\htmeasdef{CLEO.Gamma19by13.pub.PROCARIO.93}{Gamma19by13}{CLEO}{Procario:1992hd}{0.342 \pm 0.006 \pm 0.016}{0.342}{\pm 0.006}{0.016}%
\htmeasdef{CLEO.Gamma23.pub.BATTLE.94}{Gamma23}{CLEO}{Battle:1994by}{0.0009 \pm 0.001 \pm 0.0003}{0.0009}{\pm 0.001}{0.0003}%
\htmeasdef{CLEO.Gamma26by13.pub.PROCARIO.93}{Gamma26by13}{CLEO}{Procario:1992hd}{0.044 \pm 0.003 \pm 0.005}{0.044}{\pm 0.003}{0.005}%
\htmeasdef{CLEO.Gamma29.pub.PROCARIO.93}{Gamma29}{CLEO}{Procario:1992hd}{0.0016 \pm 0.0005 \pm 0.0005}{0.0016}{\pm 0.0005}{0.0005}%
\htmeasdef{CLEO.Gamma31.pub.BATTLE.94}{Gamma31}{CLEO}{Battle:1994by}{0.017 \pm 0.0012 \pm 0.0019}{0.017}{\pm 0.0012}{0.0019}%
\htmeasdef{CLEO.Gamma34.pub.COAN.96}{Gamma34}{CLEO}{Coan:1996iu}{0.00855 \pm 0.00036 \pm 0.00073}{0.00855}{\pm 0.00036}{0.00073}%
\htmeasdef{CLEO.Gamma37.pub.COAN.96}{Gamma37}{CLEO}{Coan:1996iu}{0.00151 \pm 0.00021 \pm 0.00022}{0.00151}{\pm 0.00021}{0.00022}%
\htmeasdef{CLEO.Gamma39.pub.COAN.96}{Gamma39}{CLEO}{Coan:1996iu}{0.00562 \pm 0.0005 \pm 0.00048}{0.00562}{\pm 0.0005}{0.00048}%
\htmeasdef{CLEO.Gamma3by5.pub.ANASTASSOV.97}{Gamma3by5}{CLEO}{Anastassov:1996tc}{0.9777 \pm 0.0063 \pm 0.0087}{0.9777}{\pm 0.0063}{0.0087}%
\htmeasdef{CLEO.Gamma42.pub.COAN.96}{Gamma42}{CLEO}{Coan:1996iu}{0.00145 \pm 0.00036 \pm 0.0002}{0.00145}{\pm 0.00036}{0.0002}%
\htmeasdef{CLEO.Gamma47.pub.COAN.96}{Gamma47}{CLEO}{Coan:1996iu}{0.00023 \pm 5\cdot 10^{-5} \pm 3\cdot 10^{-5}}{0.00023}{\pm 5e-05}{3e-05}%
\htmeasdef{CLEO.Gamma5.pub.ANASTASSOV.97}{Gamma5}{CLEO}{Anastassov:1996tc}{0.1776 \pm 0.0006 \pm 0.0017}{0.1776}{\pm 0.0006}{0.0017}%
\htmeasdef{CLEO.Gamma57.pub.BALEST.95C}{Gamma57}{CLEO}{Balest:1995kq}{0.0951 \pm 0.0007 \pm 0.002}{0.0951}{\pm 0.0007}{0.002}%
\htmeasdef{CLEO.Gamma66.pub.BALEST.95C}{Gamma66}{CLEO}{Balest:1995kq}{0.0423 \pm 0.0006 \pm 0.0022}{0.0423}{\pm 0.0006}{0.0022}%
\htmeasdef{CLEO.Gamma69.pub.EDWARDS.00A}{Gamma69}{CLEO}{Edwards:1999fj}{0.0419 \pm 0.001 \pm 0.0021}{0.0419}{\pm 0.001}{0.0021}%
\htmeasdef{CLEO.Gamma76by54.pub.BORTOLETTO.93}{Gamma76by54}{CLEO}{Bortoletto:1993px}{0.034 \pm 0.002 \pm 0.003}{0.034}{\pm 0.002}{0.003}%
\htmeasdef{CLEO.Gamma78.pub.ANASTASSOV.01}{Gamma78}{CLEO}{Anastassov:2000xu}{0.00022 \pm 3\cdot 10^{-5} \pm 4\cdot 10^{-5}}{0.00022}{\pm 3e-05}{4e-05}%
\htmeasdef{CLEO.Gamma8.pub.ANASTASSOV.97}{Gamma8}{CLEO}{Anastassov:1996tc}{0.1152 \pm 0.0005 \pm 0.0012}{0.1152}{\pm 0.0005}{0.0012}%
\htmeasdef{CLEO.Gamma80by60.pub.RICHICHI.99}{Gamma80by60}{CLEO}{Richichi:1998bc}{0.0544 \pm 0.0021 \pm 0.0053}{0.0544}{\pm 0.0021}{0.0053}%
\htmeasdef{CLEO.Gamma81by69.pub.RICHICHI.99}{Gamma81by69}{CLEO}{Richichi:1998bc}{0.0261 \pm 0.0045 \pm 0.0042}{0.0261}{\pm 0.0045}{0.0042}%
\htmeasdef{CLEO.Gamma93by60.pub.RICHICHI.99}{Gamma93by60}{CLEO}{Richichi:1998bc}{0.016 \pm 0.0015 \pm 0.003}{0.016}{\pm 0.0015}{0.003}%
\htmeasdef{CLEO.Gamma94by69.pub.RICHICHI.99}{Gamma94by69}{CLEO}{Richichi:1998bc}{0.0079 \pm 0.0044 \pm 0.0016}{0.0079}{\pm 0.0044}{0.0016}%
\htmeasdef{CLEO3.Gamma151.pub.ARMS.05}{Gamma151}{CLEO3}{Arms:2005qg}{( 4.1 \pm 0.6 \pm 0.7 ) \cdot 10^{ -4 }}{4.1e-4}{\pm 0.6e-4}{0.7e-4}%
\htmeasdef{CLEO3.Gamma60.pub.BRIERE.03}{Gamma60}{CLEO3}{Briere:2003fr}{0.0913 \pm 0.0005 \pm 0.0046}{0.0913}{\pm 0.0005}{0.0046}%
\htmeasdef{CLEO3.Gamma85.pub.BRIERE.03}{Gamma85}{CLEO3}{Briere:2003fr}{0.00384 \pm 0.00014 \pm 0.00038}{0.00384}{\pm 0.00014}{0.00038}%
\htmeasdef{CLEO3.Gamma88.pub.ARMS.05}{Gamma88}{CLEO3}{Arms:2005qg}{0.00074 \pm 8\cdot 10^{-5} \pm 0.00011}{0.00074}{\pm 8e-05}{0.00011}%
\htmeasdef{CLEO3.Gamma93.pub.BRIERE.03}{Gamma93}{CLEO3}{Briere:2003fr}{0.00155 \pm 6\cdot 10^{-5} \pm 9\cdot 10^{-5}}{0.00155}{\pm 6e-05}{9e-05}%
\htmeasdef{CLEO3.Gamma94.pub.ARMS.05}{Gamma94}{CLEO3}{Arms:2005qg}{( 5.5 \pm 1.4 \pm 1.2 ) \cdot 10^{ -5 }}{5.5e-05}{\pm 1.4e-05}{1.2e-05}%
\htmeasdef{DELPHI.Gamma10.pub.ABREU.94K}{Gamma10}{DELPHI}{Abreu:1994fi}{0.0085 \pm 0.0018}{0.0085}{\pm 0.0018}{0}%
\htmeasdef{DELPHI.Gamma103.pub.ABDALLAH.06A}{Gamma103}{DELPHI}{Abdallah:2003cw}{0.00097 \pm 0.00015 \pm 5\cdot 10^{-5}}{0.00097}{\pm 0.00015}{5e-05}%
\htmeasdef{DELPHI.Gamma104.pub.ABDALLAH.06A}{Gamma104}{DELPHI}{Abdallah:2003cw}{0.00016 \pm 0.00012 \pm 6\cdot 10^{-5}}{0.00016}{\pm 0.00012}{6e-05}%
\htmeasdef{DELPHI.Gamma13.pub.ABDALLAH.06A}{Gamma13}{DELPHI}{Abdallah:2003cw}{0.2574 \pm 0.00201 \pm 0.00138}{0.2574}{\pm 0.00201}{0.00138}%
\htmeasdef{DELPHI.Gamma19.pub.ABDALLAH.06A}{Gamma19}{DELPHI}{Abdallah:2003cw}{0.09498 \pm 0.0032 \pm 0.00275}{0.09498}{\pm 0.0032}{0.00275}%
\htmeasdef{DELPHI.Gamma25.pub.ABDALLAH.06A}{Gamma25}{DELPHI}{Abdallah:2003cw}{0.01403 \pm 0.00214 \pm 0.00224}{0.01403}{\pm 0.00214}{0.00224}%
\htmeasdef{DELPHI.Gamma3.pub.ABREU.99X}{Gamma3}{DELPHI}{Abreu:1999rb}{0.17325 \pm 0.00095 \pm 0.00077}{0.17325}{\pm 0.00095}{0.00077}%
\htmeasdef{DELPHI.Gamma31.pub.ABREU.94K}{Gamma31}{DELPHI}{Abreu:1994fi}{0.0154 \pm 0.0024}{0.0154}{\pm 0.0024}{0}%
\htmeasdef{DELPHI.Gamma5.pub.ABREU.99X}{Gamma5}{DELPHI}{Abreu:1999rb}{0.17877 \pm 0.00109 \pm 0.0011}{0.17877}{\pm 0.00109}{0.0011}%
\htmeasdef{DELPHI.Gamma57.pub.ABDALLAH.06A}{Gamma57}{DELPHI}{Abdallah:2003cw}{0.09317 \pm 0.0009 \pm 0.00082}{0.09317}{\pm 0.0009}{0.00082}%
\htmeasdef{DELPHI.Gamma66.pub.ABDALLAH.06A}{Gamma66}{DELPHI}{Abdallah:2003cw}{0.04545 \pm 0.00106 \pm 0.00103}{0.04545}{\pm 0.00106}{0.00103}%
\htmeasdef{DELPHI.Gamma7.pub.ABREU.92N}{Gamma7}{DELPHI}{Abreu:1992gn}{0.124 \pm 0.007 \pm 0.007}{0.124}{\pm 0.007}{0.007}%
\htmeasdef{DELPHI.Gamma74.pub.ABDALLAH.06A}{Gamma74}{DELPHI}{Abdallah:2003cw}{0.00561 \pm 0.00068 \pm 0.00095}{0.00561}{\pm 0.00068}{0.00095}%
\htmeasdef{DELPHI.Gamma8.pub.ABDALLAH.06A}{Gamma8}{DELPHI}{Abdallah:2003cw}{0.11571 \pm 0.0012 \pm 0.00114}{0.11571}{\pm 0.0012}{0.00114}%
\htmeasdef{HRS.Gamma102.pub.BYLSMA.87}{Gamma102}{HRS}{Bylsma:1986zy}{0.00102 \pm 0.00029}{0.00102}{\pm 0.00029}{0}%
\htmeasdef{HRS.Gamma103.pub.BYLSMA.87}{Gamma103}{HRS}{Bylsma:1986zy}{0.00051 \pm 0.0002}{0.00051}{\pm 0.0002}{0}%
\htmeasdef{L3.Gamma102.pub.ACHARD.01D}{Gamma102}{L3}{Achard:2001pk}{0.0017 \pm 0.00022 \pm 0.00026}{0.0017}{\pm 0.00022}{0.00026}%
\htmeasdef{L3.Gamma13.pub.ACCIARRI.95}{Gamma13}{L3}{Acciarri:1994vr}{0.2505 \pm 0.0035 \pm 0.005}{0.2505}{\pm 0.0035}{0.005}%
\htmeasdef{L3.Gamma19.pub.ACCIARRI.95}{Gamma19}{L3}{Acciarri:1994vr}{0.0888 \pm 0.0037 \pm 0.0042}{0.0888}{\pm 0.0037}{0.0042}%
\htmeasdef{L3.Gamma26.pub.ACCIARRI.95}{Gamma26}{L3}{Acciarri:1994vr}{0.017 \pm 0.0024 \pm 0.0038}{0.017}{\pm 0.0024}{0.0038}%
\htmeasdef{L3.Gamma3.pub.ACCIARRI.01F}{Gamma3}{L3}{Acciarri:2001sg}{0.17342 \pm 0.0011 \pm 0.00067}{0.17342}{\pm 0.0011}{0.00067}%
\htmeasdef{L3.Gamma35.pub.ACCIARRI.95F}{Gamma35}{L3}{Acciarri:1995kx}{0.0095 \pm 0.0015 \pm 0.0006}{0.0095}{\pm 0.0015}{0.0006}%
\htmeasdef{L3.Gamma40.pub.ACCIARRI.95F}{Gamma40}{L3}{Acciarri:1995kx}{0.0041 \pm 0.0012 \pm 0.0003}{0.0041}{\pm 0.0012}{0.0003}%
\htmeasdef{L3.Gamma5.pub.ACCIARRI.01F}{Gamma5}{L3}{Acciarri:2001sg}{0.17806 \pm 0.00104 \pm 0.00076}{0.17806}{\pm 0.00104}{0.00076}%
\htmeasdef{L3.Gamma54.pub.ADEVA.91F}{Gamma54}{L3}{Adeva:1991qq}{0.144 \pm 0.006 \pm 0.003}{0.144}{\pm 0.006}{0.003}%
\htmeasdef{L3.Gamma55.pub.ACHARD.01D}{Gamma55}{L3}{Achard:2001pk}{0.14556 \pm 0.00105 \pm 0.00076}{0.14556}{\pm 0.00105}{0.00076}%
\htmeasdef{L3.Gamma7.pub.ACCIARRI.95}{Gamma7}{L3}{Acciarri:1994vr}{0.1247 \pm 0.0026 \pm 0.0043}{0.1247}{\pm 0.0026}{0.0043}%
\htmeasdef{OPAL.Gamma10.pub.ABBIENDI.01J}{Gamma10}{OPAL}{Abbiendi:2000ee}{0.00658 \pm 0.00027 \pm 0.00029}{0.00658}{\pm 0.00027}{0.00029}%
\htmeasdef{OPAL.Gamma103.pub.ACKERSTAFF.99E}{Gamma103}{OPAL}{Ackerstaff:1998ia}{0.00091 \pm 0.00014 \pm 6\cdot 10^{-5}}{0.00091}{\pm 0.00014}{6e-05}%
\htmeasdef{OPAL.Gamma104.pub.ACKERSTAFF.99E}{Gamma104}{OPAL}{Ackerstaff:1998ia}{0.00027 \pm 0.00018 \pm 9\cdot 10^{-5}}{0.00027}{\pm 0.00018}{9e-05}%
\htmeasdef{OPAL.Gamma13.pub.ACKERSTAFF.98M}{Gamma13}{OPAL}{Ackerstaff:1997tx}{0.2589 \pm 0.0017 \pm 0.0029}{0.2589}{\pm 0.0017}{0.0029}%
\htmeasdef{OPAL.Gamma16.pub.ABBIENDI.04J}{Gamma16}{OPAL}{Abbiendi:2004xa}{0.00471 \pm 0.00059 \pm 0.00023}{0.00471}{\pm 0.00059}{0.00023}%
\htmeasdef{OPAL.Gamma17.pub.ACKERSTAFF.98M}{Gamma17}{OPAL}{Ackerstaff:1997tx}{0.0991 \pm 0.0031 \pm 0.0027}{0.0991}{\pm 0.0031}{0.0027}%
\htmeasdef{OPAL.Gamma3.pub.ABBIENDI.03}{Gamma3}{OPAL}{Abbiendi:2002jw}{0.1734 \pm 0.0009 \pm 0.0006}{0.1734}{\pm 0.0009}{0.0006}%
\htmeasdef{OPAL.Gamma31.pub.ABBIENDI.01J}{Gamma31}{OPAL}{Abbiendi:2000ee}{0.01528 \pm 0.00039 \pm 0.0004}{0.01528}{\pm 0.00039}{0.0004}%
\htmeasdef{OPAL.Gamma33.pub.AKERS.94G}{Gamma33}{OPAL}{Akers:1994td}{0.0097 \pm 0.0009 \pm 0.0006}{0.0097}{\pm 0.0009}{0.0006}%
\htmeasdef{OPAL.Gamma35.pub.ABBIENDI.00C}{Gamma35}{OPAL}{Abbiendi:1999pm}{0.00933 \pm 0.00068 \pm 0.00049}{0.00933}{\pm 0.00068}{0.00049}%
\htmeasdef{OPAL.Gamma38.pub.ABBIENDI.00C}{Gamma38}{OPAL}{Abbiendi:1999pm}{0.0033 \pm 0.00055 \pm 0.00039}{0.0033}{\pm 0.00055}{0.00039}%
\htmeasdef{OPAL.Gamma43.pub.ABBIENDI.00C}{Gamma43}{OPAL}{Abbiendi:1999pm}{0.00324 \pm 0.00074 \pm 0.00066}{0.00324}{\pm 0.00074}{0.00066}%
\htmeasdef{OPAL.Gamma5.pub.ABBIENDI.99H}{Gamma5}{OPAL}{Abbiendi:1998cx}{0.1781 \pm 0.0009 \pm 0.0006}{0.1781}{\pm 0.0009}{0.0006}%
\htmeasdef{OPAL.Gamma55.pub.AKERS.95Y}{Gamma55}{OPAL}{Akers:1995ry}{0.1496 \pm 0.0009 \pm 0.0022}{0.1496}{\pm 0.0009}{0.0022}%
\htmeasdef{OPAL.Gamma57by55.pub.AKERS.95Y}{Gamma57by55}{OPAL}{Akers:1995ry}{0.66 \pm 0.004 \pm 0.014}{0.66}{\pm 0.004}{0.014}%
\htmeasdef{OPAL.Gamma7.pub.ALEXANDER.91D}{Gamma7}{OPAL}{Alexander:1991am}{0.121 \pm 0.007 \pm 0.005}{0.121}{\pm 0.007}{0.005}%
\htmeasdef{OPAL.Gamma8.pub.ACKERSTAFF.98M}{Gamma8}{OPAL}{Ackerstaff:1997tx}{0.1198 \pm 0.0013 \pm 0.0016}{0.1198}{\pm 0.0013}{0.0016}%
\htmeasdef{OPAL.Gamma85.pub.ABBIENDI.04J}{Gamma85}{OPAL}{Abbiendi:2004xa}{0.00415 \pm 0.00053 \pm 0.0004}{0.00415}{\pm 0.00053}{0.0004}%
\htmeasdef{OPAL.Gamma92.pub.ABBIENDI.00D}{Gamma92}{OPAL}{Abbiendi:1999cq}{0.00159 \pm 0.00053 \pm 0.0002}{0.00159}{\pm 0.00053}{0.0002}%
\htmeasdef{TPC.Gamma54.pub.AIHARA.87B}{Gamma54}{TPC}{Aihara:1986mw}{0.151 \pm 0.008 \pm 0.006}{0.151}{\pm 0.008}{0.006}%
\htmeasdef{TPC.Gamma82.pub.BAUER.94}{Gamma82}{TPC}{Bauer:1993wn}{0.0058 {}^{+0.0015}_{-0.0013} \pm 0.0012}{0.0058}{{}^{+0.0015}_{-0.0013}}{0.0012}%
\htmeasdef{TPC.Gamma92.pub.BAUER.94}{Gamma92}{TPC}{Bauer:1993wn}{0.0015 {}^{+0.0009}_{-0.0007} \pm 0.0003}{0.0015}{{}^{+0.0009}_{-0.0007}}{0.0003}%
\htdef{Gamma1.qt}{\ensuremath{0.8521 \pm 0.0011}}%
\htdef{Gamma2.qt}{\ensuremath{0.8455 \pm 0.0010}}%
\htdef{Gamma3.qt}{\ensuremath{0.17392 \pm 0.00039}}%
\htdef{ALEPH.Gamma3.pub.SCHAEL.05C,qt}{\ensuremath{0.17319 \pm 0.00070 \pm 0.00032}}%
\htdef{DELPHI.Gamma3.pub.ABREU.99X,qt}{\ensuremath{0.17325 \pm 0.00095 \pm 0.00077}}%
\htdef{L3.Gamma3.pub.ACCIARRI.01F,qt}{\ensuremath{0.17342 \pm 0.00110 \pm 0.00067}}%
\htdef{OPAL.Gamma3.pub.ABBIENDI.03,qt}{\ensuremath{0.17340 \pm 0.00090 \pm 0.00060}}%
\htdef{Gamma3by5.qt}{\ensuremath{0.9761 \pm 0.0028}}%
\htdef{ARGUS.Gamma3by5.pub.ALBRECHT.92D,qt}{\ensuremath{0.9970 \pm 0.0350 \pm 0.0400}}%
\htdef{BaBar.Gamma3by5.pub.AUBERT.10F,qt}{\ensuremath{0.9796 \pm 0.0016 \pm 0.0036}}%
\htdef{CLEO.Gamma3by5.pub.ANASTASSOV.97,qt}{\ensuremath{0.9777 \pm 0.0063 \pm 0.0087}}%
\htdef{Gamma5.qt}{\ensuremath{0.17817 \pm 0.00041}}%
\htdef{ALEPH.Gamma5.pub.SCHAEL.05C,qt}{\ensuremath{0.17837 \pm 0.00072 \pm 0.00036}}%
\htdef{CLEO.Gamma5.pub.ANASTASSOV.97,qt}{\ensuremath{0.17760 \pm 0.00060 \pm 0.00170}}%
\htdef{DELPHI.Gamma5.pub.ABREU.99X,qt}{\ensuremath{0.17877 \pm 0.00109 \pm 0.00110}}%
\htdef{L3.Gamma5.pub.ACCIARRI.01F,qt}{\ensuremath{0.17806 \pm 0.00104 \pm 0.00076}}%
\htdef{OPAL.Gamma5.pub.ABBIENDI.99H,qt}{\ensuremath{0.17810 \pm 0.00090 \pm 0.00060}}%
\htdef{Gamma7.qt}{\ensuremath{0.12019 \pm 0.00053}}%
\htdef{DELPHI.Gamma7.pub.ABREU.92N,qt}{\ensuremath{0.12400 \pm 0.00700 \pm 0.00700}}%
\htdef{L3.Gamma7.pub.ACCIARRI.95,qt}{\ensuremath{0.12470 \pm 0.00260 \pm 0.00430}}%
\htdef{OPAL.Gamma7.pub.ALEXANDER.91D,qt}{\ensuremath{0.12100 \pm 0.00700 \pm 0.00500}}%
\htdef{Gamma8.qt}{\ensuremath{0.11502 \pm 0.00053}}%
\htdef{ALEPH.Gamma8.pub.SCHAEL.05C,qt}{\ensuremath{0.11524 \pm 0.00070 \pm 0.00078}}%
\htdef{CLEO.Gamma8.pub.ANASTASSOV.97,qt}{\ensuremath{0.11520 \pm 0.00050 \pm 0.00120}}%
\htdef{DELPHI.Gamma8.pub.ABDALLAH.06A,qt}{\ensuremath{0.11571 \pm 0.00120 \pm 0.00114}}%
\htdef{OPAL.Gamma8.pub.ACKERSTAFF.98M,qt}{\ensuremath{0.11980 \pm 0.00130 \pm 0.00160}}%
\htdef{Gamma8by5.qt}{\ensuremath{0.6456 \pm 0.0033}}%
\htdef{Gamma9.qt}{\ensuremath{0.10804 \pm 0.00052}}%
\htdef{Gamma9by5.qt}{\ensuremath{0.6064 \pm 0.0032}}%
\htdef{BaBar.Gamma9by5.pub.AUBERT.10F,qt}{\ensuremath{0.5945 \pm 0.0014 \pm 0.0061}}%
\htdef{Gamma10.qt}{\ensuremath{(0.6986 \pm 0.0085) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma10.pub.BARATE.99K,qt}{\ensuremath{(0.6960 \pm 0.0250 \pm 0.0140) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma10.prelim.ICHEP2018,qt}{\ensuremath{(0.7170 \pm 0.0031 \pm 0.0210) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma10.pub.BATTLE.94,qt}{\ensuremath{(0.6600 \pm 0.0700 \pm 0.0900) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma10.pub.ABREU.94K,qt}{\ensuremath{(0.8500 \pm 0.1800 \pm 0.0000) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma10.pub.ABBIENDI.01J,qt}{\ensuremath{(0.6580 \pm 0.0270 \pm 0.0290) \cdot 10^{-2} }}%
\htdef{Gamma10by5.qt}{\ensuremath{(3.921 \pm 0.048) \cdot 10^{-2}}}%
\htdef{BaBar.Gamma10by5.pub.AUBERT.10F,qt}{\ensuremath{(3.882 \pm 0.032 \pm 0.057) \cdot 10^{-2} }}%
\htdef{Gamma10by9.qt}{\ensuremath{(6.467 \pm 0.084) \cdot 10^{-2}}}%
\htdef{Gamma11.qt}{\ensuremath{0.36996 \pm 0.00094}}%
\htdef{Gamma12.qt}{\ensuremath{0.36495 \pm 0.00094}}%
\htdef{Gamma13.qt}{\ensuremath{0.25938 \pm 0.00090}}%
\htdef{ALEPH.Gamma13.pub.SCHAEL.05C,qt}{\ensuremath{0.25924 \pm 0.00097 \pm 0.00085}}%
\htdef{Belle.Gamma13.pub.FUJIKAWA.08,qt}{\ensuremath{0.25670 \pm 0.00010 \pm 0.00390}}%
\htdef{CLEO.Gamma13.pub.ARTUSO.94,qt}{\ensuremath{0.25870 \pm 0.00120 \pm 0.00420}}%
\htdef{DELPHI.Gamma13.pub.ABDALLAH.06A,qt}{\ensuremath{0.25740 \pm 0.00201 \pm 0.00138}}%
\htdef{L3.Gamma13.pub.ACCIARRI.95,qt}{\ensuremath{0.25050 \pm 0.00350 \pm 0.00500}}%
\htdef{OPAL.Gamma13.pub.ACKERSTAFF.98M,qt}{\ensuremath{0.25890 \pm 0.00170 \pm 0.00290}}%
\htdef{Gamma14.qt}{\ensuremath{0.25447 \pm 0.00091}}%
\htdef{Gamma16.qt}{\ensuremath{(0.4904 \pm 0.0092) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma16.pub.BARATE.99K,qt}{\ensuremath{(0.4440 \pm 0.0260 \pm 0.0240) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma16.prelim.ICHEP2018,qt}{\ensuremath{(0.5050 \pm 0.0020 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma16.pub.BATTLE.94,qt}{\ensuremath{(0.5100 \pm 0.1000 \pm 0.0700) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma16.pub.ABBIENDI.04J,qt}{\ensuremath{(0.4710 \pm 0.0590 \pm 0.0230) \cdot 10^{-2} }}%
\htdef{Gamma17.qt}{\ensuremath{0.10793 \pm 0.00091}}%
\htdef{OPAL.Gamma17.pub.ACKERSTAFF.98M,qt}{\ensuremath{0.09910 \pm 0.00310 \pm 0.00270}}%
\htdef{Gamma18.qt}{\ensuremath{(9.421 \pm 0.092) \cdot 10^{-2}}}%
\htdef{Gamma19.qt}{\ensuremath{(9.270 \pm 0.092) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma19.pub.SCHAEL.05C,qt}{\ensuremath{(9.295 \pm 0.084 \pm 0.088) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma19.pub.ABDALLAH.06A,qt}{\ensuremath{(9.498 \pm 0.320 \pm 0.275) \cdot 10^{-2} }}%
\htdef{L3.Gamma19.pub.ACCIARRI.95,qt}{\ensuremath{(8.880 \pm 0.370 \pm 0.420) \cdot 10^{-2} }}%
\htdef{Gamma19by13.qt}{\ensuremath{0.3574 \pm 0.0042}}%
\htdef{CLEO.Gamma19by13.pub.PROCARIO.93,qt}{\ensuremath{0.3420 \pm 0.0060 \pm 0.0160}}%
\htdef{Gamma20.qt}{\ensuremath{(9.211 \pm 0.092) \cdot 10^{-2}}}%
\htdef{Gamma23.qt}{\ensuremath{(0.0585 \pm 0.0027) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma23.pub.BARATE.99K,qt}{\ensuremath{(0.0560 \pm 0.0200 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma23.prelim.ICHEP2018,qt}{\ensuremath{(0.0615 \pm 0.0012 \pm 0.0034) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma23.pub.BATTLE.94,qt}{\ensuremath{(0.0900 \pm 0.1000 \pm 0.0300) \cdot 10^{-2} }}%
\htdef{Gamma24.qt}{\ensuremath{(1.372 \pm 0.034) \cdot 10^{-2}}}%
\htdef{Gamma25.qt}{\ensuremath{(1.288 \pm 0.034) \cdot 10^{-2}}}%
\htdef{DELPHI.Gamma25.pub.ABDALLAH.06A,qt}{\ensuremath{(1.403 \pm 0.214 \pm 0.224) \cdot 10^{-2} }}%
\htdef{Gamma26.qt}{\ensuremath{(1.236 \pm 0.030) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma26.pub.SCHAEL.05C,qt}{\ensuremath{(1.082 \pm 0.071 \pm 0.059) \cdot 10^{-2} }}%
\htdef{L3.Gamma26.pub.ACCIARRI.95,qt}{\ensuremath{(1.700 \pm 0.240 \pm 0.380) \cdot 10^{-2} }}%
\htdef{Gamma26by13.qt}{\ensuremath{(4.764 \pm 0.118) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma26by13.pub.PROCARIO.93,qt}{\ensuremath{(4.400 \pm 0.300 \pm 0.500) \cdot 10^{-2} }}%
\htdef{Gamma27.qt}{\ensuremath{(1.1381 \pm 0.0292) \cdot 10^{-2}}}%
\htdef{BaBar.Gamma27.prelim.ICHEP2018,qt}{\ensuremath{(1.1680 \pm 0.0060 \pm 0.0380) \cdot 10^{-2} }}%
\htdef{Gamma28.qt}{\ensuremath{(1.127 \pm 0.263) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma28.pub.BARATE.99K,qt}{\ensuremath{(3.700 \pm 2.100 \pm 1.100) \cdot 10^{-4} }}%
\htdef{BaBar.Gamma28.prelim.ICHEP2018,qt}{\ensuremath{(1.250 \pm 0.160 \pm 0.240) \cdot 10^{-4} }}%
\htdef{Gamma29.qt}{\ensuremath{(0.1333 \pm 0.0071) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma29.pub.PROCARIO.93,qt}{\ensuremath{(0.1600 \pm 0.0500 \pm 0.0500) \cdot 10^{-2} }}%
\htdef{Gamma30.qt}{\ensuremath{(0.0864 \pm 0.0067) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma30.pub.SCHAEL.05C,qt}{\ensuremath{(0.1120 \pm 0.0370 \pm 0.0350) \cdot 10^{-2} }}%
\htdef{Gamma31.qt}{\ensuremath{(1.568 \pm 0.018) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma31.pub.BATTLE.94,qt}{\ensuremath{(1.700 \pm 0.120 \pm 0.190) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma31.pub.ABREU.94K,qt}{\ensuremath{(1.540 \pm 0.240 \pm 0.000) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma31.pub.ABBIENDI.01J,qt}{\ensuremath{(1.528 \pm 0.039 \pm 0.040) \cdot 10^{-2} }}%
\htdef{Gamma32.qt}{\ensuremath{(0.8729 \pm 0.0141) \cdot 10^{-2}}}%
\htdef{Gamma33.qt}{\ensuremath{(0.9366 \pm 0.0292) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma33.pub.BARATE.98E,qt}{\ensuremath{(0.9700 \pm 0.0580 \pm 0.0620) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma33.pub.AKERS.94G,qt}{\ensuremath{(0.9700 \pm 0.0900 \pm 0.0600) \cdot 10^{-2} }}%
\htdef{Gamma34.qt}{\ensuremath{(0.9860 \pm 0.0138) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma34.pub.COAN.96,qt}{\ensuremath{(0.8550 \pm 0.0360 \pm 0.0730) \cdot 10^{-2} }}%
\htdef{Gamma35.qt}{\ensuremath{(0.8378 \pm 0.0139) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma35.pub.BARATE.99K,qt}{\ensuremath{(0.9280 \pm 0.0450 \pm 0.0340) \cdot 10^{-2} }}%
\htdef{Belle.Gamma35.pub.RYU.14vpc,qt}{\ensuremath{(0.8320 \pm 0.0025 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{L3.Gamma35.pub.ACCIARRI.95F,qt}{\ensuremath{(0.9500 \pm 0.1500 \pm 0.0600) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma35.pub.ABBIENDI.00C,qt}{\ensuremath{(0.9330 \pm 0.0680 \pm 0.0490) \cdot 10^{-2} }}%
\htdef{Gamma37.qt}{\ensuremath{(0.1483 \pm 0.0034) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma37.pub.BARATE.98E,qt}{\ensuremath{(0.1580 \pm 0.0420 \pm 0.0170) \cdot 10^{-2} }}%
\htdef{ALEPH.Gamma37.pub.BARATE.99K,qt}{\ensuremath{(0.1620 \pm 0.0210 \pm 0.0110) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma37.pub.LEES.18B,qt}{\ensuremath{(0.1478 \pm 0.0022 \pm 0.0040) \cdot 10^{-2} }}%
\htdef{Belle.Gamma37.pub.RYU.14vpc,qt}{\ensuremath{(0.1480 \pm 0.0013 \pm 0.0055) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma37.pub.COAN.96,qt}{\ensuremath{(0.1510 \pm 0.0210 \pm 0.0220) \cdot 10^{-2} }}%
\htdef{Gamma38.qt}{\ensuremath{(0.2977 \pm 0.0073) \cdot 10^{-2}}}%
\htdef{OPAL.Gamma38.pub.ABBIENDI.00C,qt}{\ensuremath{(0.3300 \pm 0.0550 \pm 0.0390) \cdot 10^{-2} }}%
\htdef{Gamma39.qt}{\ensuremath{(0.5302 \pm 0.0134) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma39.pub.COAN.96,qt}{\ensuremath{(0.5620 \pm 0.0500 \pm 0.0480) \cdot 10^{-2} }}%
\htdef{Gamma40.qt}{\ensuremath{(0.3807 \pm 0.0129) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma40.pub.BARATE.98E,qt}{\ensuremath{(0.2940 \pm 0.0730 \pm 0.0370) \cdot 10^{-2} }}%
\htdef{ALEPH.Gamma40.pub.BARATE.99K,qt}{\ensuremath{(0.3470 \pm 0.0530 \pm 0.0370) \cdot 10^{-2} }}%
\htdef{Belle.Gamma40.pub.RYU.14vpc,qt}{\ensuremath{(0.3860 \pm 0.0031 \pm 0.0135) \cdot 10^{-2} }}%
\htdef{L3.Gamma40.pub.ACCIARRI.95F,qt}{\ensuremath{(0.4100 \pm 0.1200 \pm 0.0300) \cdot 10^{-2} }}%
\htdef{Gamma42.qt}{\ensuremath{(0.1494 \pm 0.0070) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma42.pub.BARATE.98E,qt}{\ensuremath{(0.1520 \pm 0.0760 \pm 0.0210) \cdot 10^{-2} }}%
\htdef{ALEPH.Gamma42.pub.BARATE.99K,qt}{\ensuremath{(0.1430 \pm 0.0250 \pm 0.0150) \cdot 10^{-2} }}%
\htdef{Belle.Gamma42.pub.RYU.14vpc,qt}{\ensuremath{(0.1496 \pm 0.0019 \pm 0.0073) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma42.pub.COAN.96,qt}{\ensuremath{(0.1450 \pm 0.0360 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{Gamma43.qt}{\ensuremath{(0.4042 \pm 0.0260) \cdot 10^{-2}}}%
\htdef{OPAL.Gamma43.pub.ABBIENDI.00C,qt}{\ensuremath{(0.3240 \pm 0.0740 \pm 0.0660) \cdot 10^{-2} }}%
\htdef{Gamma44.qt}{\ensuremath{(2.346 \pm 2.306) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma44.pub.BARATE.99R,qt}{\ensuremath{(2.600 \pm 2.400 \pm 0.000) \cdot 10^{-4} }}%
\htdef{Gamma46.qt}{\ensuremath{(0.1516 \pm 0.0247) \cdot 10^{-2}}}%
\htdef{Gamma47.qt}{\ensuremath{(2.342 \pm 0.065) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma47.pub.BARATE.98E,qt}{\ensuremath{(2.600 \pm 1.000 \pm 0.500) \cdot 10^{-4} }}%
\htdef{BaBar.Gamma47.pub.LEES.12Y,qt}{\ensuremath{(2.310 \pm 0.040 \pm 0.080) \cdot 10^{-4} }}%
\htdef{Belle.Gamma47.pub.RYU.14vpc,qt}{\ensuremath{(2.330 \pm 0.033 \pm 0.093) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma47.pub.COAN.96,qt}{\ensuremath{(2.300 \pm 0.500 \pm 0.300) \cdot 10^{-4} }}%
\htdef{Gamma48.qt}{\ensuremath{(0.1048 \pm 0.0247) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma48.pub.BARATE.98E,qt}{\ensuremath{(0.1010 \pm 0.0230 \pm 0.0130) \cdot 10^{-2} }}%
\htdef{Gamma49.qt}{\ensuremath{(3.543 \pm 1.193) \cdot 10^{-4}}}%
\htdef{Gamma50.qt}{\ensuremath{(1.816 \pm 0.207) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma50.pub.LEES.12Y,qt}{\ensuremath{(1.600 \pm 0.200 \pm 0.220) \cdot 10^{-5} }}%
\htdef{Belle.Gamma50.pub.RYU.14vpc,qt}{\ensuremath{(2.000 \pm 0.216 \pm 0.202) \cdot 10^{-5} }}%
\htdef{Gamma51.qt}{\ensuremath{(3.179 \pm 1.192) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma51.pub.BARATE.98E,qt}{\ensuremath{(3.100 \pm 1.100 \pm 0.500) \cdot 10^{-4} }}%
\htdef{Gamma53.qt}{\ensuremath{(2.220 \pm 2.024) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma53.pub.BARATE.98E,qt}{\ensuremath{(2.300 \pm 1.900 \pm 0.700) \cdot 10^{-4} }}%
\htdef{Gamma54.qt}{\ensuremath{0.15206 \pm 0.00061}}%
\htdef{CELLO.Gamma54.pub.BEHREND.89B,qt}{\ensuremath{0.15000 \pm 0.00400 \pm 0.00300}}%
\htdef{L3.Gamma54.pub.ADEVA.91F,qt}{\ensuremath{0.14400 \pm 0.00600 \pm 0.00300}}%
\htdef{TPC.Gamma54.pub.AIHARA.87B,qt}{\ensuremath{0.15100 \pm 0.00800 \pm 0.00600}}%
\htdef{Gamma55.qt}{\ensuremath{0.14558 \pm 0.00056}}%
\htdef{L3.Gamma55.pub.ACHARD.01D,qt}{\ensuremath{0.14556 \pm 0.00105 \pm 0.00076}}%
\htdef{OPAL.Gamma55.pub.AKERS.95Y,qt}{\ensuremath{0.14960 \pm 0.00090 \pm 0.00220}}%
\htdef{Gamma56.qt}{\ensuremath{(9.769 \pm 0.053) \cdot 10^{-2}}}%
\htdef{Gamma57.qt}{\ensuremath{(9.428 \pm 0.053) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma57.pub.BALEST.95C,qt}{\ensuremath{(9.510 \pm 0.070 \pm 0.200) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma57.pub.ABDALLAH.06A,qt}{\ensuremath{(9.317 \pm 0.090 \pm 0.082) \cdot 10^{-2} }}%
\htdef{Gamma57by55.qt}{\ensuremath{0.6476 \pm 0.0029}}%
\htdef{OPAL.Gamma57by55.pub.AKERS.95Y,qt}{\ensuremath{0.6600 \pm 0.0040 \pm 0.0140}}%
\htdef{Gamma58.qt}{\ensuremath{(9.397 \pm 0.053) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma58.pub.SCHAEL.05C,qt}{\ensuremath{(9.469 \pm 0.062 \pm 0.073) \cdot 10^{-2} }}%
\htdef{Gamma59.qt}{\ensuremath{(9.279 \pm 0.051) \cdot 10^{-2}}}%
\htdef{Gamma60.qt}{\ensuremath{(8.990 \pm 0.051) \cdot 10^{-2}}}%
\htdef{BaBar.Gamma60.pub.AUBERT.08,qt}{\ensuremath{(8.830 \pm 0.010 \pm 0.130) \cdot 10^{-2} }}%
\htdef{Belle.Gamma60.pub.LEE.10,qt}{\ensuremath{(8.420 \pm 0.000 {}^{+0.260}_{-0.250}) \cdot 10^{-2} }}%
\htdef{CLEO3.Gamma60.pub.BRIERE.03,qt}{\ensuremath{(9.130 \pm 0.050 \pm 0.460) \cdot 10^{-2} }}%
\htdef{Gamma62.qt}{\ensuremath{(8.960 \pm 0.051) \cdot 10^{-2}}}%
\htdef{Gamma63.qt}{\ensuremath{(5.327 \pm 0.049) \cdot 10^{-2}}}%
\htdef{Gamma64.qt}{\ensuremath{(5.122 \pm 0.049) \cdot 10^{-2}}}%
\htdef{Gamma65.qt}{\ensuremath{(4.791 \pm 0.052) \cdot 10^{-2}}}%
\htdef{Gamma66.qt}{\ensuremath{(4.607 \pm 0.051) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma66.pub.SCHAEL.05C,qt}{\ensuremath{(4.734 \pm 0.059 \pm 0.049) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma66.pub.BALEST.95C,qt}{\ensuremath{(4.230 \pm 0.060 \pm 0.220) \cdot 10^{-2} }}%
\htdef{DELPHI.Gamma66.pub.ABDALLAH.06A,qt}{\ensuremath{(4.545 \pm 0.106 \pm 0.103) \cdot 10^{-2} }}%
\htdef{Gamma67.qt}{\ensuremath{(2.821 \pm 0.070) \cdot 10^{-2}}}%
\htdef{Gamma68.qt}{\ensuremath{(4.652 \pm 0.053) \cdot 10^{-2}}}%
\htdef{Gamma69.qt}{\ensuremath{(4.520 \pm 0.052) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma69.pub.EDWARDS.00A,qt}{\ensuremath{(4.190 \pm 0.100 \pm 0.210) \cdot 10^{-2} }}%
\htdef{Gamma70.qt}{\ensuremath{(2.770 \pm 0.071) \cdot 10^{-2}}}%
\htdef{Gamma74.qt}{\ensuremath{(0.5148 \pm 0.0311) \cdot 10^{-2}}}%
\htdef{DELPHI.Gamma74.pub.ABDALLAH.06A,qt}{\ensuremath{(0.5610 \pm 0.0680 \pm 0.0950) \cdot 10^{-2} }}%
\htdef{Gamma75.qt}{\ensuremath{(0.5037 \pm 0.0309) \cdot 10^{-2}}}%
\htdef{Gamma76.qt}{\ensuremath{(0.4937 \pm 0.0309) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma76.pub.SCHAEL.05C,qt}{\ensuremath{(0.4350 \pm 0.0300 \pm 0.0350) \cdot 10^{-2} }}%
\htdef{Gamma76by54.qt}{\ensuremath{(3.247 \pm 0.202) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma76by54.pub.BORTOLETTO.93,qt}{\ensuremath{(3.400 \pm 0.200 \pm 0.300) \cdot 10^{-2} }}%
\htdef{Gamma77.qt}{\ensuremath{(9.812 \pm 3.555) \cdot 10^{-4}}}%
\htdef{Gamma78.qt}{\ensuremath{(2.114 \pm 0.299) \cdot 10^{-4}}}%
\htdef{CLEO.Gamma78.pub.ANASTASSOV.01,qt}{\ensuremath{(2.200 \pm 0.300 \pm 0.400) \cdot 10^{-4} }}%
\htdef{Gamma79.qt}{\ensuremath{(0.6293 \pm 0.0140) \cdot 10^{-2}}}%
\htdef{Gamma80.qt}{\ensuremath{(0.4361 \pm 0.0072) \cdot 10^{-2}}}%
\htdef{Gamma80by60.qt}{\ensuremath{(4.851 \pm 0.080) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma80by60.pub.RICHICHI.99,qt}{\ensuremath{(5.440 \pm 0.210 \pm 0.530) \cdot 10^{-2} }}%
\htdef{Gamma81.qt}{\ensuremath{(8.727 \pm 1.177) \cdot 10^{-4}}}%
\htdef{Gamma81by69.qt}{\ensuremath{(1.931 \pm 0.266) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma81by69.pub.RICHICHI.99,qt}{\ensuremath{(2.610 \pm 0.450 \pm 0.420) \cdot 10^{-2} }}%
\htdef{Gamma82.qt}{\ensuremath{(0.4779 \pm 0.0137) \cdot 10^{-2}}}%
\htdef{TPC.Gamma82.pub.BAUER.94,qt}{\ensuremath{(0.5800 {}^{+0.1500}_{-0.1300} \pm 0.1200) \cdot 10^{-2} }}%
\htdef{Gamma83.qt}{\ensuremath{(0.3741 \pm 0.0135) \cdot 10^{-2}}}%
\htdef{Gamma84.qt}{\ensuremath{(0.3442 \pm 0.0068) \cdot 10^{-2}}}%
\htdef{Gamma85.qt}{\ensuremath{(0.2929 \pm 0.0067) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma85.pub.BARATE.98,qt}{\ensuremath{(0.2140 \pm 0.0370 \pm 0.0290) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma85.pub.AUBERT.08,qt}{\ensuremath{(0.2730 \pm 0.0020 \pm 0.0090) \cdot 10^{-2} }}%
\htdef{Belle.Gamma85.pub.LEE.10,qt}{\ensuremath{(0.3300 \pm 0.0010 {}^{+0.0160}_{-0.0170}) \cdot 10^{-2} }}%
\htdef{CLEO3.Gamma85.pub.BRIERE.03,qt}{\ensuremath{(0.3840 \pm 0.0140 \pm 0.0380) \cdot 10^{-2} }}%
\htdef{OPAL.Gamma85.pub.ABBIENDI.04J,qt}{\ensuremath{(0.4150 \pm 0.0530 \pm 0.0400) \cdot 10^{-2} }}%
\htdef{Gamma85by60.qt}{\ensuremath{(3.258 \pm 0.074) \cdot 10^{-2}}}%
\htdef{Gamma87.qt}{\ensuremath{(0.1329 \pm 0.0119) \cdot 10^{-2}}}%
\htdef{Gamma88.qt}{\ensuremath{(8.116 \pm 1.168) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma88.pub.BARATE.98,qt}{\ensuremath{(6.100 \pm 3.900 \pm 1.800) \cdot 10^{-4} }}%
\htdef{CLEO3.Gamma88.pub.ARMS.05,qt}{\ensuremath{(7.400 \pm 0.800 \pm 1.100) \cdot 10^{-4} }}%
\htdef{Gamma89.qt}{\ensuremath{(7.762 \pm 1.168) \cdot 10^{-4}}}%
\htdef{Gamma92.qt}{\ensuremath{(0.1493 \pm 0.0033) \cdot 10^{-2}}}%
\htdef{OPAL.Gamma92.pub.ABBIENDI.00D,qt}{\ensuremath{(0.1590 \pm 0.0530 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{TPC.Gamma92.pub.BAUER.94,qt}{\ensuremath{(0.1500 {}^{+0.0900}_{-0.0700} \pm 0.0300) \cdot 10^{-2} }}%
\htdef{Gamma93.qt}{\ensuremath{(0.1431 \pm 0.0027) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma93.pub.BARATE.98,qt}{\ensuremath{(0.1630 \pm 0.0210 \pm 0.0170) \cdot 10^{-2} }}%
\htdef{BaBar.Gamma93.pub.AUBERT.08,qt}{\ensuremath{(0.1346 \pm 0.0010 \pm 0.0036) \cdot 10^{-2} }}%
\htdef{Belle.Gamma93.pub.LEE.10,qt}{\ensuremath{(0.1550 \pm 0.0010 {}^{+0.0060}_{-0.0050}) \cdot 10^{-2} }}%
\htdef{CLEO3.Gamma93.pub.BRIERE.03,qt}{\ensuremath{(0.1550 \pm 0.0060 \pm 0.0090) \cdot 10^{-2} }}%
\htdef{Gamma93by60.qt}{\ensuremath{(1.592 \pm 0.030) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma93by60.pub.RICHICHI.99,qt}{\ensuremath{(1.600 \pm 0.150 \pm 0.300) \cdot 10^{-2} }}%
\htdef{Gamma94.qt}{\ensuremath{(0.611 \pm 0.183) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma94.pub.BARATE.98,qt}{\ensuremath{(7.500 \pm 2.900 \pm 1.500) \cdot 10^{-4} }}%
\htdef{CLEO3.Gamma94.pub.ARMS.05,qt}{\ensuremath{(0.550 \pm 0.140 \pm 0.120) \cdot 10^{-4} }}%
\htdef{Gamma94by69.qt}{\ensuremath{(0.1353 \pm 0.0405) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma94by69.pub.RICHICHI.99,qt}{\ensuremath{(0.7900 \pm 0.4400 \pm 0.1600) \cdot 10^{-2} }}%
\htdef{Gamma96.qt}{\ensuremath{(2.169 \pm 0.800) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma96.pub.AUBERT.08,qt}{\ensuremath{(1.578 \pm 0.130 \pm 0.123) \cdot 10^{-5} }}%
\htdef{Belle.Gamma96.pub.LEE.10,qt}{\ensuremath{(3.290 \pm 0.170 {}^{+0.190}_{-0.200}) \cdot 10^{-5} }}%
\htdef{Gamma102.qt}{\ensuremath{(0.0990 \pm 0.0037) \cdot 10^{-2}}}%
\htdef{CLEO.Gamma102.pub.GIBAUT.94B,qt}{\ensuremath{(0.0970 \pm 0.0050 \pm 0.0110) \cdot 10^{-2} }}%
\htdef{HRS.Gamma102.pub.BYLSMA.87,qt}{\ensuremath{(0.1020 \pm 0.0290 \pm 0.0000) \cdot 10^{-2} }}%
\htdef{L3.Gamma102.pub.ACHARD.01D,qt}{\ensuremath{(0.1700 \pm 0.0220 \pm 0.0260) \cdot 10^{-2} }}%
\htdef{Gamma103.qt}{\ensuremath{(8.260 \pm 0.314) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma103.pub.SCHAEL.05C,qt}{\ensuremath{(7.200 \pm 0.900 \pm 1.200) \cdot 10^{-4} }}%
\htdef{ARGUS.Gamma103.pub.ALBRECHT.88B,qt}{\ensuremath{(6.400 \pm 2.300 \pm 1.000) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma103.pub.GIBAUT.94B,qt}{\ensuremath{(7.700 \pm 0.500 \pm 0.900) \cdot 10^{-4} }}%
\htdef{DELPHI.Gamma103.pub.ABDALLAH.06A,qt}{\ensuremath{(9.700 \pm 1.500 \pm 0.500) \cdot 10^{-4} }}%
\htdef{HRS.Gamma103.pub.BYLSMA.87,qt}{\ensuremath{(5.100 \pm 2.000 \pm 0.000) \cdot 10^{-4} }}%
\htdef{OPAL.Gamma103.pub.ACKERSTAFF.99E,qt}{\ensuremath{(9.100 \pm 1.400 \pm 0.600) \cdot 10^{-4} }}%
\htdef{Gamma104.qt}{\ensuremath{(1.641 \pm 0.114) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma104.pub.SCHAEL.05C,qt}{\ensuremath{(2.100 \pm 0.700 \pm 0.900) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma104.pub.ANASTASSOV.01,qt}{\ensuremath{(1.700 \pm 0.200 \pm 0.200) \cdot 10^{-4} }}%
\htdef{DELPHI.Gamma104.pub.ABDALLAH.06A,qt}{\ensuremath{(1.600 \pm 1.200 \pm 0.600) \cdot 10^{-4} }}%
\htdef{OPAL.Gamma104.pub.ACKERSTAFF.99E,qt}{\ensuremath{(2.700 \pm 1.800 \pm 0.900) \cdot 10^{-4} }}%
\htdef{Gamma106.qt}{\ensuremath{(0.7532 \pm 0.0356) \cdot 10^{-2}}}%
\htdef{Gamma110.qt}{\ensuremath{(2.931 \pm 0.041) \cdot 10^{-2}}}%
\htdef{Gamma126.qt}{\ensuremath{(0.1386 \pm 0.0072) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma126.pub.BUSKULIC.97C,qt}{\ensuremath{(0.1800 \pm 0.0400 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{Belle.Gamma126.pub.INAMI.09,qt}{\ensuremath{(0.1350 \pm 0.0030 \pm 0.0070) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma126.pub.ARTUSO.92,qt}{\ensuremath{(0.1700 \pm 0.0200 \pm 0.0200) \cdot 10^{-2} }}%
\htdef{Gamma128.qt}{\ensuremath{(1.543 \pm 0.080) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma128.pub.BUSKULIC.97C,qt}{\ensuremath{(2.900 {}^{+1.300}_{-1.200} \pm 0.700) \cdot 10^{-4} }}%
\htdef{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,qt}{\ensuremath{(1.420 \pm 0.110 \pm 0.070) \cdot 10^{-4} }}%
\htdef{Belle.Gamma128.pub.INAMI.09,qt}{\ensuremath{(1.580 \pm 0.050 \pm 0.090) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma128.pub.BARTELT.96,qt}{\ensuremath{(2.600 \pm 0.500 \pm 0.500) \cdot 10^{-4} }}%
\htdef{Gamma130.qt}{\ensuremath{(0.483 \pm 0.116) \cdot 10^{-4}}}%
\htdef{Belle.Gamma130.pub.INAMI.09,qt}{\ensuremath{(0.460 \pm 0.110 \pm 0.040) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma130.pub.BISHAI.99,qt}{\ensuremath{(1.770 \pm 0.560 \pm 0.710) \cdot 10^{-4} }}%
\htdef{Gamma132.qt}{\ensuremath{(0.936 \pm 0.149) \cdot 10^{-4}}}%
\htdef{Belle.Gamma132.pub.INAMI.09,qt}{\ensuremath{(0.880 \pm 0.140 \pm 0.060) \cdot 10^{-4} }}%
\htdef{CLEO.Gamma132.pub.BISHAI.99,qt}{\ensuremath{(2.200 \pm 0.700 \pm 0.220) \cdot 10^{-4} }}%
\htdef{Gamma136.qt}{\ensuremath{(2.196 \pm 0.129) \cdot 10^{-4}}}%
\htdef{Gamma149.qt}{\ensuremath{(2.402 \pm 0.075) \cdot 10^{-2}}}%
\htdef{Gamma150.qt}{\ensuremath{(1.996 \pm 0.064) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma150.pub.BUSKULIC.97C,qt}{\ensuremath{(1.910 \pm 0.070 \pm 0.060) \cdot 10^{-2} }}%
\htdef{CLEO.Gamma150.pub.BARINGER.87,qt}{\ensuremath{(1.600 \pm 0.270 \pm 0.410) \cdot 10^{-2} }}%
\htdef{Gamma150by66.qt}{\ensuremath{0.4331 \pm 0.0139}}%
\htdef{ALEPH.Gamma150by66.pub.BUSKULIC.96,qt}{\ensuremath{0.4310 \pm 0.0330 \pm 0.0000}}%
\htdef{CLEO.Gamma150by66.pub.BALEST.95C,qt}{\ensuremath{0.4640 \pm 0.0160 \pm 0.0170}}%
\htdef{Gamma151.qt}{\ensuremath{(4.100 \pm 0.922) \cdot 10^{-4}}}%
\htdef{CLEO3.Gamma151.pub.ARMS.05,qt}{\ensuremath{(4.100 \pm 0.600 \pm 0.700) \cdot 10^{-4} }}%
\htdef{Gamma152.qt}{\ensuremath{(0.4066 \pm 0.0419) \cdot 10^{-2}}}%
\htdef{ALEPH.Gamma152.pub.BUSKULIC.97C,qt}{\ensuremath{(0.4300 \pm 0.0600 \pm 0.0500) \cdot 10^{-2} }}%
\htdef{Gamma152by54.qt}{\ensuremath{(2.674 \pm 0.275) \cdot 10^{-2}}}%
\htdef{Gamma152by76.qt}{\ensuremath{0.8236 \pm 0.0757}}%
\htdef{CLEO.Gamma152by76.pub.BORTOLETTO.93,qt}{\ensuremath{0.8100 \pm 0.0600 \pm 0.0600}}%
\htdef{Gamma167.qt}{\ensuremath{(4.409 \pm 1.626) \cdot 10^{-5}}}%
\htdef{Gamma168.qt}{\ensuremath{(2.169 \pm 0.800) \cdot 10^{-5}}}%
\htdef{Gamma169.qt}{\ensuremath{(1.499 \pm 0.553) \cdot 10^{-5}}}%
\htdef{Gamma800.qt}{\ensuremath{(1.955 \pm 0.065) \cdot 10^{-2}}}%
\htdef{Gamma802.qt}{\ensuremath{(0.2923 \pm 0.0067) \cdot 10^{-2}}}%
\htdef{Gamma803.qt}{\ensuremath{(4.105 \pm 1.429) \cdot 10^{-4}}}%
\htdef{Gamma804.qt}{\ensuremath{(2.342 \pm 0.065) \cdot 10^{-4}}}%
\htdef{Gamma805.qt}{\ensuremath{(4.000 \pm 2.000) \cdot 10^{-4}}}%
\htdef{ALEPH.Gamma805.pub.SCHAEL.05C,qt}{\ensuremath{(4.000 \pm 2.000 \pm 0.000) \cdot 10^{-4} }}%
\htdef{Gamma806.qt}{\ensuremath{(1.816 \pm 0.207) \cdot 10^{-5}}}%
\htdef{Gamma809.qt}{\ensuremath{(8.640 \pm 0.670) \cdot 10^{-4}}}%
\htdef{BaBar.Gamma809.prelim.ICHEP2018,qt}{\ensuremath{(9.020 \pm 0.400 \pm 0.650) \cdot 10^{-4} }}%
\htdef{Gamma810.qt}{\ensuremath{(1.931 \pm 0.298) \cdot 10^{-4}}}%
\htdef{Gamma811.qt}{\ensuremath{(7.139 \pm 1.586) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma811.pub.LEES.12X,qt}{\ensuremath{(7.300 \pm 1.200 \pm 1.200) \cdot 10^{-5} }}%
\htdef{Gamma812.qt}{\ensuremath{(1.325 \pm 2.682) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma812.pub.LEES.12X,qt}{\ensuremath{(1.000 \pm 0.800 \pm 3.000) \cdot 10^{-5} }}%
\htdef{Gamma820.qt}{\ensuremath{(8.242 \pm 0.313) \cdot 10^{-4}}}%
\htdef{Gamma821.qt}{\ensuremath{(7.719 \pm 0.295) \cdot 10^{-4}}}%
\htdef{BaBar.Gamma821.pub.LEES.12X,qt}{\ensuremath{(7.680 \pm 0.040 \pm 0.400) \cdot 10^{-4} }}%
\htdef{Gamma822.qt}{\ensuremath{(0.594 \pm 1.208) \cdot 10^{-6}}}%
\htdef{BaBar.Gamma822.pub.LEES.12X,qt}{\ensuremath{(0.600 \pm 0.500 \pm 1.100) \cdot 10^{-6} }}%
\htdef{Gamma830.qt}{\ensuremath{(1.630 \pm 0.113) \cdot 10^{-4}}}%
\htdef{Gamma831.qt}{\ensuremath{(8.400 \pm 0.624) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma831.pub.LEES.12X,qt}{\ensuremath{(8.400 \pm 0.400 \pm 0.600) \cdot 10^{-5} }}%
\htdef{Gamma832.qt}{\ensuremath{(3.775 \pm 0.874) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma832.pub.LEES.12X,qt}{\ensuremath{(3.600 \pm 0.300 \pm 0.900) \cdot 10^{-5} }}%
\htdef{Gamma833.qt}{\ensuremath{(1.108 \pm 0.566) \cdot 10^{-6}}}%
\htdef{BaBar.Gamma833.pub.LEES.12X,qt}{\ensuremath{(1.100 \pm 0.400 \pm 0.400) \cdot 10^{-6} }}%
\htdef{Gamma910.qt}{\ensuremath{(7.176 \pm 0.422) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma910.pub.LEES.12X,qt}{\ensuremath{(8.270 \pm 0.880 \pm 0.810) \cdot 10^{-5} }}%
\htdef{Gamma911.qt}{\ensuremath{(4.444 \pm 0.867) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma911.pub.LEES.12X,qt}{\ensuremath{(4.570 \pm 0.770 \pm 0.500) \cdot 10^{-5} }}%
\htdef{Gamma920.qt}{\ensuremath{(5.225 \pm 0.444) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma920.pub.LEES.12X,qt}{\ensuremath{(5.200 \pm 0.310 \pm 0.370) \cdot 10^{-5} }}%
\htdef{Gamma930.qt}{\ensuremath{(5.033 \pm 0.296) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma930.pub.LEES.12X,qt}{\ensuremath{(5.390 \pm 0.270 \pm 0.410) \cdot 10^{-5} }}%
\htdef{Gamma944.qt}{\ensuremath{(8.654 \pm 0.509) \cdot 10^{-5}}}%
\htdef{BaBar.Gamma944.pub.LEES.12X,qt}{\ensuremath{(8.260 \pm 0.350 \pm 0.510) \cdot 10^{-5} }}%
\htdef{Gamma945.qt}{\ensuremath{(1.939 \pm 0.378) \cdot 10^{-4}}}%
\htdef{Gamma998.qt}{\ensuremath{(0.0274 \pm 0.1026) \cdot 10^{-2}}}%
\htdef{Gamma1.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma1.gn} = \htuse{Gamma1.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma1.qt} & average &}%
\htdef{Gamma2.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma2.gn} = \htuse{Gamma2.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma2.qt} & average &}%
\htdef{Gamma3.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma3.qt} & average & \\
\htuse{ALEPH.Gamma3.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma3.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma3.pub.SCHAEL.05C,ref} \\
\htuse{DELPHI.Gamma3.pub.ABREU.99X,qt} & \htuse{DELPHI.Gamma3.pub.ABREU.99X,exp} & \htuse{DELPHI.Gamma3.pub.ABREU.99X,ref} \\
\htuse{L3.Gamma3.pub.ACCIARRI.01F,qt} & \htuse{L3.Gamma3.pub.ACCIARRI.01F,exp} & \htuse{L3.Gamma3.pub.ACCIARRI.01F,ref} \\
\htuse{OPAL.Gamma3.pub.ABBIENDI.03,qt} & \htuse{OPAL.Gamma3.pub.ABBIENDI.03,exp} & \htuse{OPAL.Gamma3.pub.ABBIENDI.03,ref}
}%
\htdef{Gamma3by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma3by5.qt} & average & \\
\htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D,qt} & \htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D,exp} & \htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D,ref} \\
\htuse{BaBar.Gamma3by5.pub.AUBERT.10F,qt} & \htuse{BaBar.Gamma3by5.pub.AUBERT.10F,exp} & \htuse{BaBar.Gamma3by5.pub.AUBERT.10F,ref} \\
\htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97,qt} & \htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97,exp} & \htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97,ref}
}%
\htdef{Gamma5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma5.qt} & average & \\
\htuse{ALEPH.Gamma5.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma5.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma5.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma5.pub.ANASTASSOV.97,qt} & \htuse{CLEO.Gamma5.pub.ANASTASSOV.97,exp} & \htuse{CLEO.Gamma5.pub.ANASTASSOV.97,ref} \\
\htuse{DELPHI.Gamma5.pub.ABREU.99X,qt} & \htuse{DELPHI.Gamma5.pub.ABREU.99X,exp} & \htuse{DELPHI.Gamma5.pub.ABREU.99X,ref} \\
\htuse{L3.Gamma5.pub.ACCIARRI.01F,qt} & \htuse{L3.Gamma5.pub.ACCIARRI.01F,exp} & \htuse{L3.Gamma5.pub.ACCIARRI.01F,ref} \\
\htuse{OPAL.Gamma5.pub.ABBIENDI.99H,qt} & \htuse{OPAL.Gamma5.pub.ABBIENDI.99H,exp} & \htuse{OPAL.Gamma5.pub.ABBIENDI.99H,ref}
}%
\htdef{Gamma7.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma7.qt} & average & \\
\htuse{DELPHI.Gamma7.pub.ABREU.92N,qt} & \htuse{DELPHI.Gamma7.pub.ABREU.92N,exp} & \htuse{DELPHI.Gamma7.pub.ABREU.92N,ref} \\
\htuse{L3.Gamma7.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma7.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma7.pub.ACCIARRI.95,ref} \\
\htuse{OPAL.Gamma7.pub.ALEXANDER.91D,qt} & \htuse{OPAL.Gamma7.pub.ALEXANDER.91D,exp} & \htuse{OPAL.Gamma7.pub.ALEXANDER.91D,ref}
}%
\htdef{Gamma8.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma8.qt} & average & \\
\htuse{ALEPH.Gamma8.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma8.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma8.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma8.pub.ANASTASSOV.97,qt} & \htuse{CLEO.Gamma8.pub.ANASTASSOV.97,exp} & \htuse{CLEO.Gamma8.pub.ANASTASSOV.97,ref} \\
\htuse{DELPHI.Gamma8.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma8.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma8.pub.ABDALLAH.06A,ref} \\
\htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M,qt} & \htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M,exp} & \htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M,ref}
}%
\htdef{Gamma8by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma8by5.gn} = \htuse{Gamma8by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma8by5.qt} & average &}%
\htdef{Gamma9.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma9.gn} = \htuse{Gamma9.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma9.qt} & average &}%
\htdef{Gamma9by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma9by5.gn} = \htuse{Gamma9by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma9by5.qt} & average & \\
\htuse{BaBar.Gamma9by5.pub.AUBERT.10F,qt} & \htuse{BaBar.Gamma9by5.pub.AUBERT.10F,exp} & \htuse{BaBar.Gamma9by5.pub.AUBERT.10F,ref}
}%
\htdef{Gamma10.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma10.qt} & average & \\
\htuse{ALEPH.Gamma10.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma10.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma10.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma10.prelim.ICHEP2018,qt} & \htuse{BaBar.Gamma10.prelim.ICHEP2018,exp} & \htuse{BaBar.Gamma10.prelim.ICHEP2018,ref} \\
\htuse{CLEO.Gamma10.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma10.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma10.pub.BATTLE.94,ref} \\
\htuse{DELPHI.Gamma10.pub.ABREU.94K,qt} & \htuse{DELPHI.Gamma10.pub.ABREU.94K,exp} & \htuse{DELPHI.Gamma10.pub.ABREU.94K,ref} \\
\htuse{OPAL.Gamma10.pub.ABBIENDI.01J,qt} & \htuse{OPAL.Gamma10.pub.ABBIENDI.01J,exp} & \htuse{OPAL.Gamma10.pub.ABBIENDI.01J,ref}
}%
\htdef{Gamma10by5.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma10by5.gn} = \htuse{Gamma10by5.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma10by5.qt} & average & \\
\htuse{BaBar.Gamma10by5.pub.AUBERT.10F,qt} & \htuse{BaBar.Gamma10by5.pub.AUBERT.10F,exp} & \htuse{BaBar.Gamma10by5.pub.AUBERT.10F,ref}
}%
\htdef{Gamma10by9.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma10by9.gn} = \htuse{Gamma10by9.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma10by9.qt} & average &}%
\htdef{Gamma11.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma11.gn} = \htuse{Gamma11.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma11.qt} & average &}%
\htdef{Gamma12.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma12.gn} = \htuse{Gamma12.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma12.qt} & average &}%
\htdef{Gamma13.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma13.qt} & average & \\
\htuse{ALEPH.Gamma13.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma13.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma13.pub.SCHAEL.05C,ref} \\
\htuse{Belle.Gamma13.pub.FUJIKAWA.08,qt} & \htuse{Belle.Gamma13.pub.FUJIKAWA.08,exp} & \htuse{Belle.Gamma13.pub.FUJIKAWA.08,ref} \\
\htuse{CLEO.Gamma13.pub.ARTUSO.94,qt} & \htuse{CLEO.Gamma13.pub.ARTUSO.94,exp} & \htuse{CLEO.Gamma13.pub.ARTUSO.94,ref} \\
\htuse{DELPHI.Gamma13.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma13.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma13.pub.ABDALLAH.06A,ref} \\
\htuse{L3.Gamma13.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma13.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma13.pub.ACCIARRI.95,ref} \\
\htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M,qt} & \htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M,exp} & \htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M,ref}
}%
\htdef{Gamma14.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma14.gn} = \htuse{Gamma14.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma14.qt} & average &}%
\htdef{Gamma16.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma16.qt} & average & \\
\htuse{ALEPH.Gamma16.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma16.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma16.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma16.prelim.ICHEP2018,qt} & \htuse{BaBar.Gamma16.prelim.ICHEP2018,exp} & \htuse{BaBar.Gamma16.prelim.ICHEP2018,ref} \\
\htuse{CLEO.Gamma16.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma16.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma16.pub.BATTLE.94,ref} \\
\htuse{OPAL.Gamma16.pub.ABBIENDI.04J,qt} & \htuse{OPAL.Gamma16.pub.ABBIENDI.04J,exp} & \htuse{OPAL.Gamma16.pub.ABBIENDI.04J,ref}
}%
\htdef{Gamma17.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma17.gn} = \htuse{Gamma17.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma17.qt} & average & \\
\htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M,qt} & \htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M,exp} & \htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M,ref}
}%
\htdef{Gamma18.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma18.gn} = \htuse{Gamma18.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma18.qt} & average &}%
\htdef{Gamma19.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma19.qt} & average & \\
\htuse{ALEPH.Gamma19.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma19.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma19.pub.SCHAEL.05C,ref} \\
\htuse{DELPHI.Gamma19.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma19.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma19.pub.ABDALLAH.06A,ref} \\
\htuse{L3.Gamma19.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma19.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma19.pub.ACCIARRI.95,ref}
}%
\htdef{Gamma19by13.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma19by13.gn} = \htuse{Gamma19by13.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma19by13.qt} & average & \\
\htuse{CLEO.Gamma19by13.pub.PROCARIO.93,qt} & \htuse{CLEO.Gamma19by13.pub.PROCARIO.93,exp} & \htuse{CLEO.Gamma19by13.pub.PROCARIO.93,ref}
}%
\htdef{Gamma20.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma20.gn} = \htuse{Gamma20.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma20.qt} & average &}%
\htdef{Gamma23.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma23.qt} & average & \\
\htuse{ALEPH.Gamma23.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma23.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma23.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma23.prelim.ICHEP2018,qt} & \htuse{BaBar.Gamma23.prelim.ICHEP2018,exp} & \htuse{BaBar.Gamma23.prelim.ICHEP2018,ref} \\
\htuse{CLEO.Gamma23.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma23.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma23.pub.BATTLE.94,ref}
}%
\htdef{Gamma24.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma24.gn} = \htuse{Gamma24.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma24.qt} & average &}%
\htdef{Gamma25.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma25.gn} = \htuse{Gamma25.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma25.qt} & average & \\
\htuse{DELPHI.Gamma25.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma25.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma25.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma26.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma26.gn} = \htuse{Gamma26.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma26.qt} & average & \\
\htuse{ALEPH.Gamma26.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma26.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma26.pub.SCHAEL.05C,ref} \\
\htuse{L3.Gamma26.pub.ACCIARRI.95,qt} & \htuse{L3.Gamma26.pub.ACCIARRI.95,exp} & \htuse{L3.Gamma26.pub.ACCIARRI.95,ref}
}%
\htdef{Gamma26by13.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma26by13.gn} = \htuse{Gamma26by13.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma26by13.qt} & average & \\
\htuse{CLEO.Gamma26by13.pub.PROCARIO.93,qt} & \htuse{CLEO.Gamma26by13.pub.PROCARIO.93,exp} & \htuse{CLEO.Gamma26by13.pub.PROCARIO.93,ref}
}%
\htdef{Gamma27.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma27.gn} = \htuse{Gamma27.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma27.qt} & average & \\
\htuse{BaBar.Gamma27.prelim.ICHEP2018,qt} & \htuse{BaBar.Gamma27.prelim.ICHEP2018,exp} & \htuse{BaBar.Gamma27.prelim.ICHEP2018,ref}
}%
\htdef{Gamma28.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma28.gn} = \htuse{Gamma28.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma28.qt} & average & \\
\htuse{ALEPH.Gamma28.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma28.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma28.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma28.prelim.ICHEP2018,qt} & \htuse{BaBar.Gamma28.prelim.ICHEP2018,exp} & \htuse{BaBar.Gamma28.prelim.ICHEP2018,ref}
}%
\htdef{Gamma29.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma29.gn} = \htuse{Gamma29.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma29.qt} & average & \\
\htuse{CLEO.Gamma29.pub.PROCARIO.93,qt} & \htuse{CLEO.Gamma29.pub.PROCARIO.93,exp} & \htuse{CLEO.Gamma29.pub.PROCARIO.93,ref}
}%
\htdef{Gamma30.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma30.gn} = \htuse{Gamma30.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma30.qt} & average & \\
\htuse{ALEPH.Gamma30.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma30.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma30.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma31.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma31.qt} & average & \\
\htuse{CLEO.Gamma31.pub.BATTLE.94,qt} & \htuse{CLEO.Gamma31.pub.BATTLE.94,exp} & \htuse{CLEO.Gamma31.pub.BATTLE.94,ref} \\
\htuse{DELPHI.Gamma31.pub.ABREU.94K,qt} & \htuse{DELPHI.Gamma31.pub.ABREU.94K,exp} & \htuse{DELPHI.Gamma31.pub.ABREU.94K,ref} \\
\htuse{OPAL.Gamma31.pub.ABBIENDI.01J,qt} & \htuse{OPAL.Gamma31.pub.ABBIENDI.01J,exp} & \htuse{OPAL.Gamma31.pub.ABBIENDI.01J,ref}
}%
\htdef{Gamma32.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma32.gn} = \htuse{Gamma32.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma32.qt} & average &}%
\htdef{Gamma33.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma33.gn} = \htuse{Gamma33.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma33.qt} & average & \\
\htuse{ALEPH.Gamma33.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma33.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma33.pub.BARATE.98E,ref} \\
\htuse{OPAL.Gamma33.pub.AKERS.94G,qt} & \htuse{OPAL.Gamma33.pub.AKERS.94G,exp} & \htuse{OPAL.Gamma33.pub.AKERS.94G,ref}
}%
\htdef{Gamma34.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma34.gn} = \htuse{Gamma34.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma34.qt} & average & \\
\htuse{CLEO.Gamma34.pub.COAN.96,qt} & \htuse{CLEO.Gamma34.pub.COAN.96,exp} & \htuse{CLEO.Gamma34.pub.COAN.96,ref}
}%
\htdef{Gamma35.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma35.qt} & average & \\
\htuse{ALEPH.Gamma35.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma35.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma35.pub.BARATE.99K,ref} \\
\htuse{Belle.Gamma35.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma35.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma35.pub.RYU.14vpc,ref} \\
\htuse{L3.Gamma35.pub.ACCIARRI.95F,qt} & \htuse{L3.Gamma35.pub.ACCIARRI.95F,exp} & \htuse{L3.Gamma35.pub.ACCIARRI.95F,ref} \\
\htuse{OPAL.Gamma35.pub.ABBIENDI.00C,qt} & \htuse{OPAL.Gamma35.pub.ABBIENDI.00C,exp} & \htuse{OPAL.Gamma35.pub.ABBIENDI.00C,ref}
}%
\htdef{Gamma37.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma37.qt} & average & \\
\htuse{ALEPH.Gamma37.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma37.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma37.pub.BARATE.98E,ref} \\
\htuse{ALEPH.Gamma37.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma37.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma37.pub.BARATE.99K,ref} \\
\htuse{BaBar.Gamma37.pub.LEES.18B,qt} & \htuse{BaBar.Gamma37.pub.LEES.18B,exp} & \htuse{BaBar.Gamma37.pub.LEES.18B,ref} \\
\htuse{Belle.Gamma37.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma37.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma37.pub.RYU.14vpc,ref} \\
\htuse{CLEO.Gamma37.pub.COAN.96,qt} & \htuse{CLEO.Gamma37.pub.COAN.96,exp} & \htuse{CLEO.Gamma37.pub.COAN.96,ref}
}%
\htdef{Gamma38.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma38.gn} = \htuse{Gamma38.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma38.qt} & average & \\
\htuse{OPAL.Gamma38.pub.ABBIENDI.00C,qt} & \htuse{OPAL.Gamma38.pub.ABBIENDI.00C,exp} & \htuse{OPAL.Gamma38.pub.ABBIENDI.00C,ref}
}%
\htdef{Gamma39.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma39.gn} = \htuse{Gamma39.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma39.qt} & average & \\
\htuse{CLEO.Gamma39.pub.COAN.96,qt} & \htuse{CLEO.Gamma39.pub.COAN.96,exp} & \htuse{CLEO.Gamma39.pub.COAN.96,ref}
}%
\htdef{Gamma40.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma40.qt} & average & \\
\htuse{ALEPH.Gamma40.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma40.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma40.pub.BARATE.98E,ref} \\
\htuse{ALEPH.Gamma40.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma40.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma40.pub.BARATE.99K,ref} \\
\htuse{Belle.Gamma40.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma40.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma40.pub.RYU.14vpc,ref} \\
\htuse{L3.Gamma40.pub.ACCIARRI.95F,qt} & \htuse{L3.Gamma40.pub.ACCIARRI.95F,exp} & \htuse{L3.Gamma40.pub.ACCIARRI.95F,ref}
}%
\htdef{Gamma42.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma42.qt} & average & \\
\htuse{ALEPH.Gamma42.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma42.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma42.pub.BARATE.98E,ref} \\
\htuse{ALEPH.Gamma42.pub.BARATE.99K,qt} & \htuse{ALEPH.Gamma42.pub.BARATE.99K,exp} & \htuse{ALEPH.Gamma42.pub.BARATE.99K,ref} \\
\htuse{Belle.Gamma42.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma42.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma42.pub.RYU.14vpc,ref} \\
\htuse{CLEO.Gamma42.pub.COAN.96,qt} & \htuse{CLEO.Gamma42.pub.COAN.96,exp} & \htuse{CLEO.Gamma42.pub.COAN.96,ref}
}%
\htdef{Gamma43.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma43.gn} = \htuse{Gamma43.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma43.qt} & average & \\
\htuse{OPAL.Gamma43.pub.ABBIENDI.00C,qt} & \htuse{OPAL.Gamma43.pub.ABBIENDI.00C,exp} & \htuse{OPAL.Gamma43.pub.ABBIENDI.00C,ref}
}%
\htdef{Gamma44.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma44.gn} = \htuse{Gamma44.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma44.qt} & average & \\
\htuse{ALEPH.Gamma44.pub.BARATE.99R,qt} & \htuse{ALEPH.Gamma44.pub.BARATE.99R,exp} & \htuse{ALEPH.Gamma44.pub.BARATE.99R,ref}
}%
\htdef{Gamma46.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma46.gn} = \htuse{Gamma46.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma46.qt} & average &}%
\htdef{Gamma47.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma47.qt} & average & \\
\htuse{ALEPH.Gamma47.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma47.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma47.pub.BARATE.98E,ref} \\
\htuse{BaBar.Gamma47.pub.LEES.12Y,qt} & \htuse{BaBar.Gamma47.pub.LEES.12Y,exp} & \htuse{BaBar.Gamma47.pub.LEES.12Y,ref} \\
\htuse{Belle.Gamma47.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma47.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma47.pub.RYU.14vpc,ref} \\
\htuse{CLEO.Gamma47.pub.COAN.96,qt} & \htuse{CLEO.Gamma47.pub.COAN.96,exp} & \htuse{CLEO.Gamma47.pub.COAN.96,ref}
}%
\htdef{Gamma48.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma48.gn} = \htuse{Gamma48.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma48.qt} & average & \\
\htuse{ALEPH.Gamma48.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma48.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma48.pub.BARATE.98E,ref}
}%
\htdef{Gamma49.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma49.gn} = \htuse{Gamma49.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma49.qt} & average &}%
\htdef{Gamma50.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma50.gn} = \htuse{Gamma50.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma50.qt} & average & \\
\htuse{BaBar.Gamma50.pub.LEES.12Y,qt} & \htuse{BaBar.Gamma50.pub.LEES.12Y,exp} & \htuse{BaBar.Gamma50.pub.LEES.12Y,ref} \\
\htuse{Belle.Gamma50.pub.RYU.14vpc,qt} & \htuse{Belle.Gamma50.pub.RYU.14vpc,exp} & \htuse{Belle.Gamma50.pub.RYU.14vpc,ref}
}%
\htdef{Gamma51.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma51.gn} = \htuse{Gamma51.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma51.qt} & average & \\
\htuse{ALEPH.Gamma51.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma51.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma51.pub.BARATE.98E,ref}
}%
\htdef{Gamma53.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma53.gn} = \htuse{Gamma53.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma53.qt} & average & \\
\htuse{ALEPH.Gamma53.pub.BARATE.98E,qt} & \htuse{ALEPH.Gamma53.pub.BARATE.98E,exp} & \htuse{ALEPH.Gamma53.pub.BARATE.98E,ref}
}%
\htdef{Gamma54.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma54.qt} & average & \\
\htuse{CELLO.Gamma54.pub.BEHREND.89B,qt} & \htuse{CELLO.Gamma54.pub.BEHREND.89B,exp} & \htuse{CELLO.Gamma54.pub.BEHREND.89B,ref} \\
\htuse{L3.Gamma54.pub.ADEVA.91F,qt} & \htuse{L3.Gamma54.pub.ADEVA.91F,exp} & \htuse{L3.Gamma54.pub.ADEVA.91F,ref} \\
\htuse{TPC.Gamma54.pub.AIHARA.87B,qt} & \htuse{TPC.Gamma54.pub.AIHARA.87B,exp} & \htuse{TPC.Gamma54.pub.AIHARA.87B,ref}
}%
\htdef{Gamma55.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma55.gn} = \htuse{Gamma55.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma55.qt} & average & \\
\htuse{L3.Gamma55.pub.ACHARD.01D,qt} & \htuse{L3.Gamma55.pub.ACHARD.01D,exp} & \htuse{L3.Gamma55.pub.ACHARD.01D,ref} \\
\htuse{OPAL.Gamma55.pub.AKERS.95Y,qt} & \htuse{OPAL.Gamma55.pub.AKERS.95Y,exp} & \htuse{OPAL.Gamma55.pub.AKERS.95Y,ref}
}%
\htdef{Gamma56.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma56.gn} = \htuse{Gamma56.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma56.qt} & average &}%
\htdef{Gamma57.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma57.gn} = \htuse{Gamma57.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma57.qt} & average & \\
\htuse{CLEO.Gamma57.pub.BALEST.95C,qt} & \htuse{CLEO.Gamma57.pub.BALEST.95C,exp} & \htuse{CLEO.Gamma57.pub.BALEST.95C,ref} \\
\htuse{DELPHI.Gamma57.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma57.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma57.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma57by55.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma57by55.gn} = \htuse{Gamma57by55.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma57by55.qt} & average & \\
\htuse{OPAL.Gamma57by55.pub.AKERS.95Y,qt} & \htuse{OPAL.Gamma57by55.pub.AKERS.95Y,exp} & \htuse{OPAL.Gamma57by55.pub.AKERS.95Y,ref}
}%
\htdef{Gamma58.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma58.gn} = \htuse{Gamma58.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma58.qt} & average & \\
\htuse{ALEPH.Gamma58.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma58.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma58.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma59.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma59.gn} = \htuse{Gamma59.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma59.qt} & average &}%
\htdef{Gamma60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma60.qt} & average & \\
\htuse{BaBar.Gamma60.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma60.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma60.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma60.pub.LEE.10,qt} & \htuse{Belle.Gamma60.pub.LEE.10,exp} & \htuse{Belle.Gamma60.pub.LEE.10,ref} \\
\htuse{CLEO3.Gamma60.pub.BRIERE.03,qt} & \htuse{CLEO3.Gamma60.pub.BRIERE.03,exp} & \htuse{CLEO3.Gamma60.pub.BRIERE.03,ref}
}%
\htdef{Gamma62.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma62.gn} = \htuse{Gamma62.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma62.qt} & average &}%
\htdef{Gamma63.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma63.gn} = \htuse{Gamma63.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma63.qt} & average &}%
\htdef{Gamma64.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma64.gn} = \htuse{Gamma64.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma64.qt} & average &}%
\htdef{Gamma65.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma65.gn} = \htuse{Gamma65.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma65.qt} & average &}%
\htdef{Gamma66.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma66.qt} & average & \\
\htuse{ALEPH.Gamma66.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma66.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma66.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma66.pub.BALEST.95C,qt} & \htuse{CLEO.Gamma66.pub.BALEST.95C,exp} & \htuse{CLEO.Gamma66.pub.BALEST.95C,ref} \\
\htuse{DELPHI.Gamma66.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma66.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma66.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma67.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma67.gn} = \htuse{Gamma67.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma67.qt} & average &}%
\htdef{Gamma68.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma68.gn} = \htuse{Gamma68.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma68.qt} & average &}%
\htdef{Gamma69.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma69.gn} = \htuse{Gamma69.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma69.qt} & average & \\
\htuse{CLEO.Gamma69.pub.EDWARDS.00A,qt} & \htuse{CLEO.Gamma69.pub.EDWARDS.00A,exp} & \htuse{CLEO.Gamma69.pub.EDWARDS.00A,ref}
}%
\htdef{Gamma70.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma70.gn} = \htuse{Gamma70.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma70.qt} & average &}%
\htdef{Gamma74.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma74.gn} = \htuse{Gamma74.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma74.qt} & average & \\
\htuse{DELPHI.Gamma74.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma74.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma74.pub.ABDALLAH.06A,ref}
}%
\htdef{Gamma75.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma75.gn} = \htuse{Gamma75.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma75.qt} & average &}%
\htdef{Gamma76.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma76.gn} = \htuse{Gamma76.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma76.qt} & average & \\
\htuse{ALEPH.Gamma76.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma76.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma76.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma76by54.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma76by54.gn} = \htuse{Gamma76by54.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma76by54.qt} & average & \\
\htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93,qt} & \htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93,exp} & \htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93,ref}
}%
\htdef{Gamma77.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma77.gn} = \htuse{Gamma77.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma77.qt} & average &}%
\htdef{Gamma78.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma78.gn} = \htuse{Gamma78.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma78.qt} & average & \\
\htuse{CLEO.Gamma78.pub.ANASTASSOV.01,qt} & \htuse{CLEO.Gamma78.pub.ANASTASSOV.01,exp} & \htuse{CLEO.Gamma78.pub.ANASTASSOV.01,ref}
}%
\htdef{Gamma79.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma79.gn} = \htuse{Gamma79.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma79.qt} & average &}%
\htdef{Gamma80.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma80.gn} = \htuse{Gamma80.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma80.qt} & average &}%
\htdef{Gamma80by60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma80by60.gn} = \htuse{Gamma80by60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma80by60.qt} & average & \\
\htuse{CLEO.Gamma80by60.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma80by60.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma80by60.pub.RICHICHI.99,ref}
}%
\htdef{Gamma81.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma81.gn} = \htuse{Gamma81.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma81.qt} & average &}%
\htdef{Gamma81by69.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma81by69.gn} = \htuse{Gamma81by69.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma81by69.qt} & average & \\
\htuse{CLEO.Gamma81by69.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma81by69.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma81by69.pub.RICHICHI.99,ref}
}%
\htdef{Gamma82.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma82.gn} = \htuse{Gamma82.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma82.qt} & average & \\
\htuse{TPC.Gamma82.pub.BAUER.94,qt} & \htuse{TPC.Gamma82.pub.BAUER.94,exp} & \htuse{TPC.Gamma82.pub.BAUER.94,ref}
}%
\htdef{Gamma83.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma83.gn} = \htuse{Gamma83.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma83.qt} & average &}%
\htdef{Gamma84.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma84.gn} = \htuse{Gamma84.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma84.qt} & average &}%
\htdef{Gamma85.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma85.qt} & average & \\
\htuse{ALEPH.Gamma85.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma85.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma85.pub.BARATE.98,ref} \\
\htuse{BaBar.Gamma85.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma85.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma85.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma85.pub.LEE.10,qt} & \htuse{Belle.Gamma85.pub.LEE.10,exp} & \htuse{Belle.Gamma85.pub.LEE.10,ref} \\
\htuse{CLEO3.Gamma85.pub.BRIERE.03,qt} & \htuse{CLEO3.Gamma85.pub.BRIERE.03,exp} & \htuse{CLEO3.Gamma85.pub.BRIERE.03,ref} \\
\htuse{OPAL.Gamma85.pub.ABBIENDI.04J,qt} & \htuse{OPAL.Gamma85.pub.ABBIENDI.04J,exp} & \htuse{OPAL.Gamma85.pub.ABBIENDI.04J,ref}
}%
\htdef{Gamma85by60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma85by60.gn} = \htuse{Gamma85by60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma85by60.qt} & average &}%
\htdef{Gamma87.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma87.gn} = \htuse{Gamma87.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma87.qt} & average &}%
\htdef{Gamma88.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma88.gn} = \htuse{Gamma88.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma88.qt} & average & \\
\htuse{ALEPH.Gamma88.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma88.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma88.pub.BARATE.98,ref} \\
\htuse{CLEO3.Gamma88.pub.ARMS.05,qt} & \htuse{CLEO3.Gamma88.pub.ARMS.05,exp} & \htuse{CLEO3.Gamma88.pub.ARMS.05,ref}
}%
\htdef{Gamma89.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma89.gn} = \htuse{Gamma89.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma89.qt} & average &}%
\htdef{Gamma92.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma92.gn} = \htuse{Gamma92.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma92.qt} & average & \\
\htuse{OPAL.Gamma92.pub.ABBIENDI.00D,qt} & \htuse{OPAL.Gamma92.pub.ABBIENDI.00D,exp} & \htuse{OPAL.Gamma92.pub.ABBIENDI.00D,ref} \\
\htuse{TPC.Gamma92.pub.BAUER.94,qt} & \htuse{TPC.Gamma92.pub.BAUER.94,exp} & \htuse{TPC.Gamma92.pub.BAUER.94,ref}
}%
\htdef{Gamma93.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma93.qt} & average & \\
\htuse{ALEPH.Gamma93.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma93.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma93.pub.BARATE.98,ref} \\
\htuse{BaBar.Gamma93.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma93.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma93.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma93.pub.LEE.10,qt} & \htuse{Belle.Gamma93.pub.LEE.10,exp} & \htuse{Belle.Gamma93.pub.LEE.10,ref} \\
\htuse{CLEO3.Gamma93.pub.BRIERE.03,qt} & \htuse{CLEO3.Gamma93.pub.BRIERE.03,exp} & \htuse{CLEO3.Gamma93.pub.BRIERE.03,ref}
}%
\htdef{Gamma93by60.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma93by60.gn} = \htuse{Gamma93by60.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma93by60.qt} & average & \\
\htuse{CLEO.Gamma93by60.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma93by60.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma93by60.pub.RICHICHI.99,ref}
}%
\htdef{Gamma94.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma94.gn} = \htuse{Gamma94.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma94.qt} & average & \\
\htuse{ALEPH.Gamma94.pub.BARATE.98,qt} & \htuse{ALEPH.Gamma94.pub.BARATE.98,exp} & \htuse{ALEPH.Gamma94.pub.BARATE.98,ref} \\
\htuse{CLEO3.Gamma94.pub.ARMS.05,qt} & \htuse{CLEO3.Gamma94.pub.ARMS.05,exp} & \htuse{CLEO3.Gamma94.pub.ARMS.05,ref}
}%
\htdef{Gamma94by69.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma94by69.gn} = \htuse{Gamma94by69.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma94by69.qt} & average & \\
\htuse{CLEO.Gamma94by69.pub.RICHICHI.99,qt} & \htuse{CLEO.Gamma94by69.pub.RICHICHI.99,exp} & \htuse{CLEO.Gamma94by69.pub.RICHICHI.99,ref}
}%
\htdef{Gamma96.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma96.gn} = \htuse{Gamma96.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma96.qt} & average & \\
\htuse{BaBar.Gamma96.pub.AUBERT.08,qt} & \htuse{BaBar.Gamma96.pub.AUBERT.08,exp} & \htuse{BaBar.Gamma96.pub.AUBERT.08,ref} \\
\htuse{Belle.Gamma96.pub.LEE.10,qt} & \htuse{Belle.Gamma96.pub.LEE.10,exp} & \htuse{Belle.Gamma96.pub.LEE.10,ref}
}%
\htdef{Gamma102.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma102.qt} & average & \\
\htuse{CLEO.Gamma102.pub.GIBAUT.94B,qt} & \htuse{CLEO.Gamma102.pub.GIBAUT.94B,exp} & \htuse{CLEO.Gamma102.pub.GIBAUT.94B,ref} \\
\htuse{HRS.Gamma102.pub.BYLSMA.87,qt} & \htuse{HRS.Gamma102.pub.BYLSMA.87,exp} & \htuse{HRS.Gamma102.pub.BYLSMA.87,ref} \\
\htuse{L3.Gamma102.pub.ACHARD.01D,qt} & \htuse{L3.Gamma102.pub.ACHARD.01D,exp} & \htuse{L3.Gamma102.pub.ACHARD.01D,ref}
}%
\htdef{Gamma103.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma103.qt} & average & \\
\htuse{ALEPH.Gamma103.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma103.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma103.pub.SCHAEL.05C,ref} \\
\htuse{ARGUS.Gamma103.pub.ALBRECHT.88B,qt} & \htuse{ARGUS.Gamma103.pub.ALBRECHT.88B,exp} & \htuse{ARGUS.Gamma103.pub.ALBRECHT.88B,ref} \\
\htuse{CLEO.Gamma103.pub.GIBAUT.94B,qt} & \htuse{CLEO.Gamma103.pub.GIBAUT.94B,exp} & \htuse{CLEO.Gamma103.pub.GIBAUT.94B,ref} \\
\htuse{DELPHI.Gamma103.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma103.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma103.pub.ABDALLAH.06A,ref} \\
\htuse{HRS.Gamma103.pub.BYLSMA.87,qt} & \htuse{HRS.Gamma103.pub.BYLSMA.87,exp} & \htuse{HRS.Gamma103.pub.BYLSMA.87,ref} \\
\htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E,qt} & \htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E,exp} & \htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E,ref}
}%
\htdef{Gamma104.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma104.qt} & average & \\
\htuse{ALEPH.Gamma104.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma104.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma104.pub.SCHAEL.05C,ref} \\
\htuse{CLEO.Gamma104.pub.ANASTASSOV.01,qt} & \htuse{CLEO.Gamma104.pub.ANASTASSOV.01,exp} & \htuse{CLEO.Gamma104.pub.ANASTASSOV.01,ref} \\
\htuse{DELPHI.Gamma104.pub.ABDALLAH.06A,qt} & \htuse{DELPHI.Gamma104.pub.ABDALLAH.06A,exp} & \htuse{DELPHI.Gamma104.pub.ABDALLAH.06A,ref} \\
\htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E,qt} & \htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E,exp} & \htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E,ref}
}%
\htdef{Gamma106.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma106.gn} = \htuse{Gamma106.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma106.qt} & average &}%
\htdef{Gamma110.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma110.gn} = \htuse{Gamma110.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma110.qt} & average &}%
\htdef{Gamma126.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma126.qt} & average & \\
\htuse{ALEPH.Gamma126.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma126.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma126.pub.BUSKULIC.97C,ref} \\
\htuse{Belle.Gamma126.pub.INAMI.09,qt} & \htuse{Belle.Gamma126.pub.INAMI.09,exp} & \htuse{Belle.Gamma126.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma126.pub.ARTUSO.92,qt} & \htuse{CLEO.Gamma126.pub.ARTUSO.92,exp} & \htuse{CLEO.Gamma126.pub.ARTUSO.92,ref}
}%
\htdef{Gamma128.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma128.qt} & average & \\
\htuse{ALEPH.Gamma128.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma128.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma128.pub.BUSKULIC.97C,ref} \\
\htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,qt} & \htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,exp} & \htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E,ref} \\
\htuse{Belle.Gamma128.pub.INAMI.09,qt} & \htuse{Belle.Gamma128.pub.INAMI.09,exp} & \htuse{Belle.Gamma128.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma128.pub.BARTELT.96,qt} & \htuse{CLEO.Gamma128.pub.BARTELT.96,exp} & \htuse{CLEO.Gamma128.pub.BARTELT.96,ref}
}%
\htdef{Gamma130.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma130.gn} = \htuse{Gamma130.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma130.qt} & average & \\
\htuse{Belle.Gamma130.pub.INAMI.09,qt} & \htuse{Belle.Gamma130.pub.INAMI.09,exp} & \htuse{Belle.Gamma130.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma130.pub.BISHAI.99,qt} & \htuse{CLEO.Gamma130.pub.BISHAI.99,exp} & \htuse{CLEO.Gamma130.pub.BISHAI.99,ref}
}%
\htdef{Gamma132.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma132.gn} = \htuse{Gamma132.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma132.qt} & average & \\
\htuse{Belle.Gamma132.pub.INAMI.09,qt} & \htuse{Belle.Gamma132.pub.INAMI.09,exp} & \htuse{Belle.Gamma132.pub.INAMI.09,ref} \\
\htuse{CLEO.Gamma132.pub.BISHAI.99,qt} & \htuse{CLEO.Gamma132.pub.BISHAI.99,exp} & \htuse{CLEO.Gamma132.pub.BISHAI.99,ref}
}%
\htdef{Gamma136.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma136.gn} = \htuse{Gamma136.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma136.qt} & average &}%
\htdef{Gamma149.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma149.gn} = \htuse{Gamma149.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma149.qt} & average &}%
\htdef{Gamma150.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma150.gn} = \htuse{Gamma150.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma150.qt} & average & \\
\htuse{ALEPH.Gamma150.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma150.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma150.pub.BUSKULIC.97C,ref} \\
\htuse{CLEO.Gamma150.pub.BARINGER.87,qt} & \htuse{CLEO.Gamma150.pub.BARINGER.87,exp} & \htuse{CLEO.Gamma150.pub.BARINGER.87,ref}
}%
\htdef{Gamma150by66.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma150by66.gn} = \htuse{Gamma150by66.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma150by66.qt} & average & \\
\htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96,qt} & \htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96,exp} & \htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96,ref} \\
\htuse{CLEO.Gamma150by66.pub.BALEST.95C,qt} & \htuse{CLEO.Gamma150by66.pub.BALEST.95C,exp} & \htuse{CLEO.Gamma150by66.pub.BALEST.95C,ref}
}%
\htdef{Gamma151.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma151.gn} = \htuse{Gamma151.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma151.qt} & average & \\
\htuse{CLEO3.Gamma151.pub.ARMS.05,qt} & \htuse{CLEO3.Gamma151.pub.ARMS.05,exp} & \htuse{CLEO3.Gamma151.pub.ARMS.05,ref}
}%
\htdef{Gamma152.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma152.gn} = \htuse{Gamma152.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma152.qt} & average & \\
\htuse{ALEPH.Gamma152.pub.BUSKULIC.97C,qt} & \htuse{ALEPH.Gamma152.pub.BUSKULIC.97C,exp} & \htuse{ALEPH.Gamma152.pub.BUSKULIC.97C,ref}
}%
\htdef{Gamma152by54.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma152by54.gn} = \htuse{Gamma152by54.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma152by54.qt} & average &}%
\htdef{Gamma152by76.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma152by76.gn} = \htuse{Gamma152by76.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma152by76.qt} & average & \\
\htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93,qt} & \htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93,exp} & \htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93,ref}
}%
\htdef{Gamma167.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma167.gn} = \htuse{Gamma167.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma167.qt} & average &}%
\htdef{Gamma168.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma168.gn} = \htuse{Gamma168.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma168.qt} & average &}%
\htdef{Gamma169.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma169.gn} = \htuse{Gamma169.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma169.qt} & average &}%
\htdef{Gamma800.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma800.gn} = \htuse{Gamma800.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma800.qt} & average &}%
\htdef{Gamma802.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma802.gn} = \htuse{Gamma802.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma802.qt} & average &}%
\htdef{Gamma803.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma803.gn} = \htuse{Gamma803.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma803.qt} & average &}%
\htdef{Gamma804.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma804.gn} = \htuse{Gamma804.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma804.qt} & average &}%
\htdef{Gamma805.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma805.gn} = \htuse{Gamma805.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma805.qt} & average & \\
\htuse{ALEPH.Gamma805.pub.SCHAEL.05C,qt} & \htuse{ALEPH.Gamma805.pub.SCHAEL.05C,exp} & \htuse{ALEPH.Gamma805.pub.SCHAEL.05C,ref}
}%
\htdef{Gamma806.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma806.gn} = \htuse{Gamma806.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma806.qt} & average &}%
\htdef{Gamma809.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma809.gn} = \htuse{Gamma809.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma809.qt} & average & \\
\htuse{BaBar.Gamma809.prelim.ICHEP2018,qt} & \htuse{BaBar.Gamma809.prelim.ICHEP2018,exp} & \htuse{BaBar.Gamma809.prelim.ICHEP2018,ref}
}%
\htdef{Gamma810.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma810.gn} = \htuse{Gamma810.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma810.qt} & average &}%
\htdef{Gamma811.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma811.gn} = \htuse{Gamma811.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma811.qt} & average & \\
\htuse{BaBar.Gamma811.pub.LEES.12X,qt} & \htuse{BaBar.Gamma811.pub.LEES.12X,exp} & \htuse{BaBar.Gamma811.pub.LEES.12X,ref}
}%
\htdef{Gamma812.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma812.gn} = \htuse{Gamma812.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma812.qt} & average & \\
\htuse{BaBar.Gamma812.pub.LEES.12X,qt} & \htuse{BaBar.Gamma812.pub.LEES.12X,exp} & \htuse{BaBar.Gamma812.pub.LEES.12X,ref}
}%
\htdef{Gamma820.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma820.gn} = \htuse{Gamma820.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma820.qt} & average &}%
\htdef{Gamma821.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma821.gn} = \htuse{Gamma821.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma821.qt} & average & \\
\htuse{BaBar.Gamma821.pub.LEES.12X,qt} & \htuse{BaBar.Gamma821.pub.LEES.12X,exp} & \htuse{BaBar.Gamma821.pub.LEES.12X,ref}
}%
\htdef{Gamma822.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma822.gn} = \htuse{Gamma822.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma822.qt} & average & \\
\htuse{BaBar.Gamma822.pub.LEES.12X,qt} & \htuse{BaBar.Gamma822.pub.LEES.12X,exp} & \htuse{BaBar.Gamma822.pub.LEES.12X,ref}
}%
\htdef{Gamma830.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma830.gn} = \htuse{Gamma830.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma830.qt} & average &}%
\htdef{Gamma831.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma831.gn} = \htuse{Gamma831.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma831.qt} & average & \\
\htuse{BaBar.Gamma831.pub.LEES.12X,qt} & \htuse{BaBar.Gamma831.pub.LEES.12X,exp} & \htuse{BaBar.Gamma831.pub.LEES.12X,ref}
}%
\htdef{Gamma832.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma832.gn} = \htuse{Gamma832.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma832.qt} & average & \\
\htuse{BaBar.Gamma832.pub.LEES.12X,qt} & \htuse{BaBar.Gamma832.pub.LEES.12X,exp} & \htuse{BaBar.Gamma832.pub.LEES.12X,ref}
}%
\htdef{Gamma833.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma833.gn} = \htuse{Gamma833.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma833.qt} & average & \\
\htuse{BaBar.Gamma833.pub.LEES.12X,qt} & \htuse{BaBar.Gamma833.pub.LEES.12X,exp} & \htuse{BaBar.Gamma833.pub.LEES.12X,ref}
}%
\htdef{Gamma910.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma910.gn} = \htuse{Gamma910.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma910.qt} & average & \\
\htuse{BaBar.Gamma910.pub.LEES.12X,qt} & \htuse{BaBar.Gamma910.pub.LEES.12X,exp} & \htuse{BaBar.Gamma910.pub.LEES.12X,ref}
}%
\htdef{Gamma911.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma911.gn} = \htuse{Gamma911.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma911.qt} & average & \\
\htuse{BaBar.Gamma911.pub.LEES.12X,qt} & \htuse{BaBar.Gamma911.pub.LEES.12X,exp} & \htuse{BaBar.Gamma911.pub.LEES.12X,ref}
}%
\htdef{Gamma920.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma920.gn} = \htuse{Gamma920.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma920.qt} & average & \\
\htuse{BaBar.Gamma920.pub.LEES.12X,qt} & \htuse{BaBar.Gamma920.pub.LEES.12X,exp} & \htuse{BaBar.Gamma920.pub.LEES.12X,ref}
}%
\htdef{Gamma930.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma930.gn} = \htuse{Gamma930.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma930.qt} & average & \\
\htuse{BaBar.Gamma930.pub.LEES.12X,qt} & \htuse{BaBar.Gamma930.pub.LEES.12X,exp} & \htuse{BaBar.Gamma930.pub.LEES.12X,ref}
}%
\htdef{Gamma944.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma944.gn} = \htuse{Gamma944.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma944.qt} & average & \\
\htuse{BaBar.Gamma944.pub.LEES.12X,qt} & \htuse{BaBar.Gamma944.pub.LEES.12X,exp} & \htuse{BaBar.Gamma944.pub.LEES.12X,ref}
}%
\htdef{Gamma945.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma945.gn} = \htuse{Gamma945.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma945.qt} & average &}%
\htdef{Gamma998.qm}{%
\begin{ensuredisplaymath}
\htuse{Gamma998.gn} = \htuse{Gamma998.td}
\end{ensuredisplaymath} & & \\
\htuse{Gamma998.qt} & average &}%
\htdef{BrVal}{%
\htuse{Gamma1.qm} \\
\midrule
\htuse{Gamma2.qm} \\
\midrule
\htuse{Gamma3.qm} \\
\midrule
\htuse{Gamma3by5.qm} \\
\midrule
\htuse{Gamma5.qm} \\
\midrule
\htuse{Gamma7.qm} \\
\midrule
\htuse{Gamma8.qm} \\
\midrule
\htuse{Gamma8by5.qm} \\
\midrule
\htuse{Gamma9.qm} \\
\midrule
\htuse{Gamma9by5.qm} \\
\midrule
\htuse{Gamma10.qm} \\
\midrule
\htuse{Gamma10by5.qm} \\
\midrule
\htuse{Gamma10by9.qm} \\
\midrule
\htuse{Gamma11.qm} \\
\midrule
\htuse{Gamma12.qm} \\
\midrule
\htuse{Gamma13.qm} \\
\midrule
\htuse{Gamma14.qm} \\
\midrule
\htuse{Gamma16.qm} \\
\midrule
\htuse{Gamma17.qm} \\
\midrule
\htuse{Gamma18.qm} \\
\midrule
\htuse{Gamma19.qm} \\
\midrule
\htuse{Gamma19by13.qm} \\
\midrule
\htuse{Gamma20.qm} \\
\midrule
\htuse{Gamma23.qm} \\
\midrule
\htuse{Gamma24.qm} \\
\midrule
\htuse{Gamma25.qm} \\
\midrule
\htuse{Gamma26.qm} \\
\midrule
\htuse{Gamma26by13.qm} \\
\midrule
\htuse{Gamma27.qm} \\
\midrule
\htuse{Gamma28.qm} \\
\midrule
\htuse{Gamma29.qm} \\
\midrule
\htuse{Gamma30.qm} \\
\midrule
\htuse{Gamma31.qm} \\
\midrule
\htuse{Gamma32.qm} \\
\midrule
\htuse{Gamma33.qm} \\
\midrule
\htuse{Gamma34.qm} \\
\midrule
\htuse{Gamma35.qm} \\
\midrule
\htuse{Gamma37.qm} \\
\midrule
\htuse{Gamma38.qm} \\
\midrule
\htuse{Gamma39.qm} \\
\midrule
\htuse{Gamma40.qm} \\
\midrule
\htuse{Gamma42.qm} \\
\midrule
\htuse{Gamma43.qm} \\
\midrule
\htuse{Gamma44.qm} \\
\midrule
\htuse{Gamma46.qm} \\
\midrule
\htuse{Gamma47.qm} \\
\midrule
\htuse{Gamma48.qm} \\
\midrule
\htuse{Gamma49.qm} \\
\midrule
\htuse{Gamma50.qm} \\
\midrule
\htuse{Gamma51.qm} \\
\midrule
\htuse{Gamma53.qm} \\
\midrule
\htuse{Gamma54.qm} \\
\midrule
\htuse{Gamma55.qm} \\
\midrule
\htuse{Gamma56.qm} \\
\midrule
\htuse{Gamma57.qm} \\
\midrule
\htuse{Gamma57by55.qm} \\
\midrule
\htuse{Gamma58.qm} \\
\midrule
\htuse{Gamma59.qm} \\
\midrule
\htuse{Gamma60.qm} \\
\midrule
\htuse{Gamma62.qm} \\
\midrule
\htuse{Gamma63.qm} \\
\midrule
\htuse{Gamma64.qm} \\
\midrule
\htuse{Gamma65.qm} \\
\midrule
\htuse{Gamma66.qm} \\
\midrule
\htuse{Gamma67.qm} \\
\midrule
\htuse{Gamma68.qm} \\
\midrule
\htuse{Gamma69.qm} \\
\midrule
\htuse{Gamma70.qm} \\
\midrule
\htuse{Gamma74.qm} \\
\midrule
\htuse{Gamma75.qm} \\
\midrule
\htuse{Gamma76.qm} \\
\midrule
\htuse{Gamma76by54.qm} \\
\midrule
\htuse{Gamma77.qm} \\
\midrule
\htuse{Gamma78.qm} \\
\midrule
\htuse{Gamma79.qm} \\
\midrule
\htuse{Gamma80.qm} \\
\midrule
\htuse{Gamma80by60.qm} \\
\midrule
\htuse{Gamma81.qm} \\
\midrule
\htuse{Gamma81by69.qm} \\
\midrule
\htuse{Gamma82.qm} \\
\midrule
\htuse{Gamma83.qm} \\
\midrule
\htuse{Gamma84.qm} \\
\midrule
\htuse{Gamma85.qm} \\
\midrule
\htuse{Gamma85by60.qm} \\
\midrule
\htuse{Gamma87.qm} \\
\midrule
\htuse{Gamma88.qm} \\
\midrule
\htuse{Gamma89.qm} \\
\midrule
\htuse{Gamma92.qm} \\
\midrule
\htuse{Gamma93.qm} \\
\midrule
\htuse{Gamma93by60.qm} \\
\midrule
\htuse{Gamma94.qm} \\
\midrule
\htuse{Gamma94by69.qm} \\
\midrule
\htuse{Gamma96.qm} \\
\midrule
\htuse{Gamma102.qm} \\
\midrule
\htuse{Gamma103.qm} \\
\midrule
\htuse{Gamma104.qm} \\
\midrule
\htuse{Gamma106.qm} \\
\midrule
\htuse{Gamma110.qm} \\
\midrule
\htuse{Gamma126.qm} \\
\midrule
\htuse{Gamma128.qm} \\
\midrule
\htuse{Gamma130.qm} \\
\midrule
\htuse{Gamma132.qm} \\
\midrule
\htuse{Gamma136.qm} \\
\midrule
\htuse{Gamma149.qm} \\
\midrule
\htuse{Gamma150.qm} \\
\midrule
\htuse{Gamma150by66.qm} \\
\midrule
\htuse{Gamma151.qm} \\
\midrule
\htuse{Gamma152.qm} \\
\midrule
\htuse{Gamma152by54.qm} \\
\midrule
\htuse{Gamma152by76.qm} \\
\midrule
\htuse{Gamma167.qm} \\
\midrule
\htuse{Gamma168.qm} \\
\midrule
\htuse{Gamma169.qm} \\
\midrule
\htuse{Gamma800.qm} \\
\midrule
\htuse{Gamma802.qm} \\
\midrule
\htuse{Gamma803.qm} \\
\midrule
\htuse{Gamma804.qm} \\
\midrule
\htuse{Gamma805.qm} \\
\midrule
\htuse{Gamma806.qm} \\
\midrule
\htuse{Gamma809.qm} \\
\midrule
\htuse{Gamma810.qm} \\
\midrule
\htuse{Gamma811.qm} \\
\midrule
\htuse{Gamma812.qm} \\
\midrule
\htuse{Gamma820.qm} \\
\midrule
\htuse{Gamma821.qm} \\
\midrule
\htuse{Gamma822.qm} \\
\midrule
\htuse{Gamma830.qm} \\
\midrule
\htuse{Gamma831.qm} \\
\midrule
\htuse{Gamma832.qm} \\
\midrule
\htuse{Gamma833.qm} \\
\midrule
\htuse{Gamma910.qm} \\
\midrule
\htuse{Gamma911.qm} \\
\midrule
\htuse{Gamma920.qm} \\
\midrule
\htuse{Gamma930.qm} \\
\midrule
\htuse{Gamma944.qm} \\
\midrule
\htuse{Gamma945.qm} \\
\midrule
\htuse{Gamma998.qm}}%
\htdef{BARATE 98.cite}{\cite{Barate:1997ma}}%
\htdef{BARATE 98.collab}{ALEPH}%
\htdef{BARATE 98.ref}{BARATE 98 (ALEPH) \cite{Barate:1997ma}}%
\htdef{BARATE 98.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma85.pub.BARATE.98}
\\
\begin{ensuredisplaymath}
\htuse{Gamma88.gn} = \htuse{Gamma88.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma88.pub.BARATE.98}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma93.pub.BARATE.98}
\\
\begin{ensuredisplaymath}
\htuse{Gamma94.gn} = \htuse{Gamma94.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma94.pub.BARATE.98}}%
\htdef{BARATE 98E.cite}{\cite{Barate:1997tt}}%
\htdef{BARATE 98E.collab}{ALEPH}%
\htdef{BARATE 98E.ref}{BARATE 98E (ALEPH) \cite{Barate:1997tt}}%
\htdef{BARATE 98E.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma33.gn} = \htuse{Gamma33.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma33.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma37.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma40.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma42.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma47.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma48.gn} = \htuse{Gamma48.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma48.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma51.gn} = \htuse{Gamma51.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma51.pub.BARATE.98E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma53.gn} = \htuse{Gamma53.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma53.pub.BARATE.98E}}%
\htdef{BARATE 99K.cite}{\cite{Barate:1999hi}}%
\htdef{BARATE 99K.collab}{ALEPH}%
\htdef{BARATE 99K.ref}{BARATE 99K (ALEPH) \cite{Barate:1999hi}}%
\htdef{BARATE 99K.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma10.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma16.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma23.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma28.gn} = \htuse{Gamma28.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma28.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma35.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma37.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma40.pub.BARATE.99K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma42.pub.BARATE.99K}}%
\htdef{BARATE 99R.cite}{\cite{Barate:1999hj}}%
\htdef{BARATE 99R.collab}{ALEPH}%
\htdef{BARATE 99R.ref}{BARATE 99R (ALEPH) \cite{Barate:1999hj}}%
\htdef{BARATE 99R.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma44.gn} = \htuse{Gamma44.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma44.pub.BARATE.99R}}%
\htdef{BUSKULIC 96.cite}{\cite{Buskulic:1995ty}}%
\htdef{BUSKULIC 96.collab}{ALEPH}%
\htdef{BUSKULIC 96.ref}{BUSKULIC 96 (ALEPH) \cite{Buskulic:1995ty}}%
\htdef{BUSKULIC 96.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma150by66.gn} = \htuse{Gamma150by66.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma150by66.pub.BUSKULIC.96}}%
\htdef{BUSKULIC 97C.cite}{\cite{Buskulic:1996qs}}%
\htdef{BUSKULIC 97C.collab}{ALEPH}%
\htdef{BUSKULIC 97C.ref}{BUSKULIC 97C (ALEPH) \cite{Buskulic:1996qs}}%
\htdef{BUSKULIC 97C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma126.pub.BUSKULIC.97C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma128.pub.BUSKULIC.97C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma150.gn} = \htuse{Gamma150.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma150.pub.BUSKULIC.97C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma152.gn} = \htuse{Gamma152.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma152.pub.BUSKULIC.97C}}%
\htdef{SCHAEL 05C.cite}{\cite{Schael:2005am}}%
\htdef{SCHAEL 05C.collab}{ALEPH}%
\htdef{SCHAEL 05C.ref}{SCHAEL 05C (ALEPH) \cite{Schael:2005am}}%
\htdef{SCHAEL 05C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma3.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma5.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma8.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma13.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma19.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma26.gn} = \htuse{Gamma26.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma26.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma30.gn} = \htuse{Gamma30.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma30.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma58.gn} = \htuse{Gamma58.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma58.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma66.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma76.gn} = \htuse{Gamma76.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma76.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma103.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma104.pub.SCHAEL.05C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma805.gn} = \htuse{Gamma805.td}
\end{ensuredisplaymath} & \htuse{ALEPH.Gamma805.pub.SCHAEL.05C}}%
\htdef{ALBRECHT 88B.cite}{\cite{Albrecht:1987zf}}%
\htdef{ALBRECHT 88B.collab}{ARGUS}%
\htdef{ALBRECHT 88B.ref}{ALBRECHT 88B (ARGUS) \cite{Albrecht:1987zf}}%
\htdef{ALBRECHT 88B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{ARGUS.Gamma103.pub.ALBRECHT.88B}}%
\htdef{ALBRECHT 92D.cite}{\cite{Albrecht:1991rh}}%
\htdef{ALBRECHT 92D.collab}{ARGUS}%
\htdef{ALBRECHT 92D.ref}{ALBRECHT 92D (ARGUS) \cite{Albrecht:1991rh}}%
\htdef{ALBRECHT 92D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & \htuse{ARGUS.Gamma3by5.pub.ALBRECHT.92D}}%
\htdef{AUBERT 08.cite}{\cite{Aubert:2007mh}}%
\htdef{AUBERT 08.collab}{\babar}%
\htdef{AUBERT 08.ref}{AUBERT 08 (\babar) \cite{Aubert:2007mh}}%
\htdef{AUBERT 08.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma60.pub.AUBERT.08}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma85.pub.AUBERT.08}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma93.pub.AUBERT.08}
\\
\begin{ensuredisplaymath}
\htuse{Gamma96.gn} = \htuse{Gamma96.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma96.pub.AUBERT.08}}%
\htdef{AUBERT 10F.cite}{\cite{Aubert:2009qj}}%
\htdef{AUBERT 10F.collab}{\babar}%
\htdef{AUBERT 10F.ref}{AUBERT 10F (\babar) \cite{Aubert:2009qj}}%
\htdef{AUBERT 10F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma3by5.pub.AUBERT.10F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma9by5.gn} = \htuse{Gamma9by5.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma9by5.pub.AUBERT.10F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma10by5.gn} = \htuse{Gamma10by5.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma10by5.pub.AUBERT.10F}}%
\htdef{DEL-AMO-SANCHEZ 11E.cite}{\cite{delAmoSanchez:2010pc}}%
\htdef{DEL-AMO-SANCHEZ 11E.collab}{\babar}%
\htdef{DEL-AMO-SANCHEZ 11E.ref}{DEL-AMO-SANCHEZ 11E (\babar) \cite{delAmoSanchez:2010pc}}%
\htdef{DEL-AMO-SANCHEZ 11E.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma128.pub.DEL-AMO-SANCHEZ.11E}}%
\htdef{LEES 12X.cite}{\cite{Lees:2012ks}}%
\htdef{LEES 12X.collab}{\babar}%
\htdef{LEES 12X.ref}{LEES 12X (\babar) \cite{Lees:2012ks}}%
\htdef{LEES 12X.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma811.gn} = \htuse{Gamma811.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma811.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma812.gn} = \htuse{Gamma812.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma812.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma821.gn} = \htuse{Gamma821.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma821.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma822.gn} = \htuse{Gamma822.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma822.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma831.gn} = \htuse{Gamma831.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma831.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma832.gn} = \htuse{Gamma832.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma832.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma833.gn} = \htuse{Gamma833.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma833.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma910.gn} = \htuse{Gamma910.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma910.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma911.gn} = \htuse{Gamma911.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma911.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma920.gn} = \htuse{Gamma920.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma920.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma930.gn} = \htuse{Gamma930.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma930.pub.LEES.12X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma944.gn} = \htuse{Gamma944.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma944.pub.LEES.12X}}%
\htdef{LEES 12Y.cite}{\cite{Lees:2012de}}%
\htdef{LEES 12Y.collab}{\babar}%
\htdef{LEES 12Y.ref}{LEES 12Y (\babar) \cite{Lees:2012de}}%
\htdef{LEES 12Y.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma47.pub.LEES.12Y}
\\
\begin{ensuredisplaymath}
\htuse{Gamma50.gn} = \htuse{Gamma50.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma50.pub.LEES.12Y}}%
\htdef{LEES 18B.cite}{\cite{BaBar:2018qry}}%
\htdef{LEES 18B.collab}{\babar}%
\htdef{LEES 18B.ref}{LEES 18B (\babar) \cite{BaBar:2018qry}}%
\htdef{LEES 18B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma37.pub.LEES.18B}}%
\htdef{BaBar prelim. ICHEP2018.cite}{\cite{Lusiani:2019mis}}%
\htdef{BaBar prelim. ICHEP2018.collab}{BaBar}%
\htdef{BaBar prelim. ICHEP2018.ref}{\babar prelim. ICHEP2018 \cite{Lusiani:2019mis}}%
\htdef{BaBar prelim. ICHEP2018.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma10.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma16.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma23.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma27.gn} = \htuse{Gamma27.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma27.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma28.gn} = \htuse{Gamma28.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma28.prelim.ICHEP2018}
\\
\begin{ensuredisplaymath}
\htuse{Gamma809.gn} = \htuse{Gamma809.td}
\end{ensuredisplaymath} & \htuse{BaBar.Gamma809.prelim.ICHEP2018}}%
\htdef{FUJIKAWA 08.cite}{\cite{Fujikawa:2008ma}}%
\htdef{FUJIKAWA 08.collab}{Belle}%
\htdef{FUJIKAWA 08.ref}{FUJIKAWA 08 (Belle) \cite{Fujikawa:2008ma}}%
\htdef{FUJIKAWA 08.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma13.pub.FUJIKAWA.08}}%
\htdef{INAMI 09.cite}{\cite{Inami:2008ar}}%
\htdef{INAMI 09.collab}{Belle}%
\htdef{INAMI 09.ref}{INAMI 09 (Belle) \cite{Inami:2008ar}}%
\htdef{INAMI 09.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma126.pub.INAMI.09}
\\
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma128.pub.INAMI.09}
\\
\begin{ensuredisplaymath}
\htuse{Gamma130.gn} = \htuse{Gamma130.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma130.pub.INAMI.09}
\\
\begin{ensuredisplaymath}
\htuse{Gamma132.gn} = \htuse{Gamma132.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma132.pub.INAMI.09}}%
\htdef{LEE 10.cite}{\cite{Lee:2010tc}}%
\htdef{LEE 10.collab}{Belle}%
\htdef{LEE 10.ref}{LEE 10 (Belle) \cite{Lee:2010tc}}%
\htdef{LEE 10.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma60.pub.LEE.10}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma85.pub.LEE.10}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma93.pub.LEE.10}
\\
\begin{ensuredisplaymath}
\htuse{Gamma96.gn} = \htuse{Gamma96.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma96.pub.LEE.10}}%
\htdef{RYU 14vpc.cite}{\cite{Ryu:2014vpc}}%
\htdef{RYU 14vpc.collab}{Belle}%
\htdef{RYU 14vpc.ref}{RYU 14vpc (Belle) \cite{Ryu:2014vpc}}%
\htdef{RYU 14vpc.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma35.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma37.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma40.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma42.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma47.pub.RYU.14vpc}
\\
\begin{ensuredisplaymath}
\htuse{Gamma50.gn} = \htuse{Gamma50.td}
\end{ensuredisplaymath} & \htuse{Belle.Gamma50.pub.RYU.14vpc}}%
\htdef{BEHREND 89B.cite}{\cite{Behrend:1989wc}}%
\htdef{BEHREND 89B.collab}{CELLO}%
\htdef{BEHREND 89B.ref}{BEHREND 89B (CELLO) \cite{Behrend:1989wc}}%
\htdef{BEHREND 89B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & \htuse{CELLO.Gamma54.pub.BEHREND.89B}}%
\htdef{ANASTASSOV 01.cite}{\cite{Anastassov:2000xu}}%
\htdef{ANASTASSOV 01.collab}{CLEO}%
\htdef{ANASTASSOV 01.ref}{ANASTASSOV 01 (CLEO) \cite{Anastassov:2000xu}}%
\htdef{ANASTASSOV 01.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma78.gn} = \htuse{Gamma78.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma78.pub.ANASTASSOV.01}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma104.pub.ANASTASSOV.01}}%
\htdef{ANASTASSOV 97.cite}{\cite{Anastassov:1996tc}}%
\htdef{ANASTASSOV 97.collab}{CLEO}%
\htdef{ANASTASSOV 97.ref}{ANASTASSOV 97 (CLEO) \cite{Anastassov:1996tc}}%
\htdef{ANASTASSOV 97.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3by5.gn} = \htuse{Gamma3by5.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma3by5.pub.ANASTASSOV.97}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma5.pub.ANASTASSOV.97}
\\
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma8.pub.ANASTASSOV.97}}%
\htdef{ARTUSO 92.cite}{\cite{Artuso:1992qu}}%
\htdef{ARTUSO 92.collab}{CLEO}%
\htdef{ARTUSO 92.ref}{ARTUSO 92 (CLEO) \cite{Artuso:1992qu}}%
\htdef{ARTUSO 92.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma126.gn} = \htuse{Gamma126.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma126.pub.ARTUSO.92}}%
\htdef{ARTUSO 94.cite}{\cite{Artuso:1994ii}}%
\htdef{ARTUSO 94.collab}{CLEO}%
\htdef{ARTUSO 94.ref}{ARTUSO 94 (CLEO) \cite{Artuso:1994ii}}%
\htdef{ARTUSO 94.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma13.pub.ARTUSO.94}}%
\htdef{BALEST 95C.cite}{\cite{Balest:1995kq}}%
\htdef{BALEST 95C.collab}{CLEO}%
\htdef{BALEST 95C.ref}{BALEST 95C (CLEO) \cite{Balest:1995kq}}%
\htdef{BALEST 95C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma57.gn} = \htuse{Gamma57.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma57.pub.BALEST.95C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma66.pub.BALEST.95C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma150by66.gn} = \htuse{Gamma150by66.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma150by66.pub.BALEST.95C}}%
\htdef{BARINGER 87.cite}{\cite{Baringer:1987tr}}%
\htdef{BARINGER 87.collab}{CLEO}%
\htdef{BARINGER 87.ref}{BARINGER 87 (CLEO) \cite{Baringer:1987tr}}%
\htdef{BARINGER 87.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma150.gn} = \htuse{Gamma150.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma150.pub.BARINGER.87}}%
\htdef{BARTELT 96.cite}{\cite{Bartelt:1996iv}}%
\htdef{BARTELT 96.collab}{CLEO}%
\htdef{BARTELT 96.ref}{BARTELT 96 (CLEO) \cite{Bartelt:1996iv}}%
\htdef{BARTELT 96.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma128.gn} = \htuse{Gamma128.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma128.pub.BARTELT.96}}%
\htdef{BATTLE 94.cite}{\cite{Battle:1994by}}%
\htdef{BATTLE 94.collab}{CLEO}%
\htdef{BATTLE 94.ref}{BATTLE 94 (CLEO) \cite{Battle:1994by}}%
\htdef{BATTLE 94.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma10.pub.BATTLE.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma16.pub.BATTLE.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma23.gn} = \htuse{Gamma23.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma23.pub.BATTLE.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma31.pub.BATTLE.94}}%
\htdef{BISHAI 99.cite}{\cite{Bishai:1998gf}}%
\htdef{BISHAI 99.collab}{CLEO}%
\htdef{BISHAI 99.ref}{BISHAI 99 (CLEO) \cite{Bishai:1998gf}}%
\htdef{BISHAI 99.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma130.gn} = \htuse{Gamma130.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma130.pub.BISHAI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma132.gn} = \htuse{Gamma132.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma132.pub.BISHAI.99}}%
\htdef{BORTOLETTO 93.cite}{\cite{Bortoletto:1993px}}%
\htdef{BORTOLETTO 93.collab}{CLEO}%
\htdef{BORTOLETTO 93.ref}{BORTOLETTO 93 (CLEO) \cite{Bortoletto:1993px}}%
\htdef{BORTOLETTO 93.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma76by54.gn} = \htuse{Gamma76by54.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma76by54.pub.BORTOLETTO.93}
\\
\begin{ensuredisplaymath}
\htuse{Gamma152by76.gn} = \htuse{Gamma152by76.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma152by76.pub.BORTOLETTO.93}}%
\htdef{COAN 96.cite}{\cite{Coan:1996iu}}%
\htdef{COAN 96.collab}{CLEO}%
\htdef{COAN 96.ref}{COAN 96 (CLEO) \cite{Coan:1996iu}}%
\htdef{COAN 96.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma34.gn} = \htuse{Gamma34.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma34.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma37.gn} = \htuse{Gamma37.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma37.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma39.gn} = \htuse{Gamma39.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma39.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma42.gn} = \htuse{Gamma42.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma42.pub.COAN.96}
\\
\begin{ensuredisplaymath}
\htuse{Gamma47.gn} = \htuse{Gamma47.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma47.pub.COAN.96}}%
\htdef{EDWARDS 00A.cite}{\cite{Edwards:1999fj}}%
\htdef{EDWARDS 00A.collab}{CLEO}%
\htdef{EDWARDS 00A.ref}{EDWARDS 00A (CLEO) \cite{Edwards:1999fj}}%
\htdef{EDWARDS 00A.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma69.gn} = \htuse{Gamma69.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma69.pub.EDWARDS.00A}}%
\htdef{GIBAUT 94B.cite}{\cite{Gibaut:1994ik}}%
\htdef{GIBAUT 94B.collab}{CLEO}%
\htdef{GIBAUT 94B.ref}{GIBAUT 94B (CLEO) \cite{Gibaut:1994ik}}%
\htdef{GIBAUT 94B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma102.pub.GIBAUT.94B}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma103.pub.GIBAUT.94B}}%
\htdef{PROCARIO 93.cite}{\cite{Procario:1992hd}}%
\htdef{PROCARIO 93.collab}{CLEO}%
\htdef{PROCARIO 93.ref}{PROCARIO 93 (CLEO) \cite{Procario:1992hd}}%
\htdef{PROCARIO 93.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma19by13.gn} = \htuse{Gamma19by13.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma19by13.pub.PROCARIO.93}
\\
\begin{ensuredisplaymath}
\htuse{Gamma26by13.gn} = \htuse{Gamma26by13.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma26by13.pub.PROCARIO.93}
\\
\begin{ensuredisplaymath}
\htuse{Gamma29.gn} = \htuse{Gamma29.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma29.pub.PROCARIO.93}}%
\htdef{RICHICHI 99.cite}{\cite{Richichi:1998bc}}%
\htdef{RICHICHI 99.collab}{CLEO}%
\htdef{RICHICHI 99.ref}{RICHICHI 99 (CLEO) \cite{Richichi:1998bc}}%
\htdef{RICHICHI 99.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma80by60.gn} = \htuse{Gamma80by60.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma80by60.pub.RICHICHI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma81by69.gn} = \htuse{Gamma81by69.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma81by69.pub.RICHICHI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93by60.gn} = \htuse{Gamma93by60.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma93by60.pub.RICHICHI.99}
\\
\begin{ensuredisplaymath}
\htuse{Gamma94by69.gn} = \htuse{Gamma94by69.td}
\end{ensuredisplaymath} & \htuse{CLEO.Gamma94by69.pub.RICHICHI.99}}%
\htdef{ARMS 05.cite}{\cite{Arms:2005qg}}%
\htdef{ARMS 05.collab}{CLEO3}%
\htdef{ARMS 05.ref}{ARMS 05 (CLEO3) \cite{Arms:2005qg}}%
\htdef{ARMS 05.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma88.gn} = \htuse{Gamma88.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma88.pub.ARMS.05}
\\
\begin{ensuredisplaymath}
\htuse{Gamma94.gn} = \htuse{Gamma94.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma94.pub.ARMS.05}
\\
\begin{ensuredisplaymath}
\htuse{Gamma151.gn} = \htuse{Gamma151.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma151.pub.ARMS.05}}%
\htdef{BRIERE 03.cite}{\cite{Briere:2003fr}}%
\htdef{BRIERE 03.collab}{CLEO3}%
\htdef{BRIERE 03.ref}{BRIERE 03 (CLEO3) \cite{Briere:2003fr}}%
\htdef{BRIERE 03.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma60.gn} = \htuse{Gamma60.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma60.pub.BRIERE.03}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma85.pub.BRIERE.03}
\\
\begin{ensuredisplaymath}
\htuse{Gamma93.gn} = \htuse{Gamma93.td}
\end{ensuredisplaymath} & \htuse{CLEO3.Gamma93.pub.BRIERE.03}}%
\htdef{ABDALLAH 06A.cite}{\cite{Abdallah:2003cw}}%
\htdef{ABDALLAH 06A.collab}{DELPHI}%
\htdef{ABDALLAH 06A.ref}{ABDALLAH 06A (DELPHI) \cite{Abdallah:2003cw}}%
\htdef{ABDALLAH 06A.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma8.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma13.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma19.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma25.gn} = \htuse{Gamma25.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma25.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma57.gn} = \htuse{Gamma57.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma57.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma66.gn} = \htuse{Gamma66.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma66.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma74.gn} = \htuse{Gamma74.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma74.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma103.pub.ABDALLAH.06A}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma104.pub.ABDALLAH.06A}}%
\htdef{ABREU 92N.cite}{\cite{Abreu:1992gn}}%
\htdef{ABREU 92N.collab}{DELPHI}%
\htdef{ABREU 92N.ref}{ABREU 92N (DELPHI) \cite{Abreu:1992gn}}%
\htdef{ABREU 92N.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma7.pub.ABREU.92N}}%
\htdef{ABREU 94K.cite}{\cite{Abreu:1994fi}}%
\htdef{ABREU 94K.collab}{DELPHI}%
\htdef{ABREU 94K.ref}{ABREU 94K (DELPHI) \cite{Abreu:1994fi}}%
\htdef{ABREU 94K.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma10.pub.ABREU.94K}
\\
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma31.pub.ABREU.94K}}%
\htdef{ABREU 99X.cite}{\cite{Abreu:1999rb}}%
\htdef{ABREU 99X.collab}{DELPHI}%
\htdef{ABREU 99X.ref}{ABREU 99X (DELPHI) \cite{Abreu:1999rb}}%
\htdef{ABREU 99X.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma3.pub.ABREU.99X}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{DELPHI.Gamma5.pub.ABREU.99X}}%
\htdef{BYLSMA 87.cite}{\cite{Bylsma:1986zy}}%
\htdef{BYLSMA 87.collab}{HRS}%
\htdef{BYLSMA 87.ref}{BYLSMA 87 (HRS) \cite{Bylsma:1986zy}}%
\htdef{BYLSMA 87.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & \htuse{HRS.Gamma102.pub.BYLSMA.87}
\\
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{HRS.Gamma103.pub.BYLSMA.87}}%
\htdef{ACCIARRI 01F.cite}{\cite{Acciarri:2001sg}}%
\htdef{ACCIARRI 01F.collab}{L3}%
\htdef{ACCIARRI 01F.ref}{ACCIARRI 01F (L3) \cite{Acciarri:2001sg}}%
\htdef{ACCIARRI 01F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma3.pub.ACCIARRI.01F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma5.pub.ACCIARRI.01F}}%
\htdef{ACCIARRI 95.cite}{\cite{Acciarri:1994vr}}%
\htdef{ACCIARRI 95.collab}{L3}%
\htdef{ACCIARRI 95.ref}{ACCIARRI 95 (L3) \cite{Acciarri:1994vr}}%
\htdef{ACCIARRI 95.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma7.pub.ACCIARRI.95}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma13.pub.ACCIARRI.95}
\\
\begin{ensuredisplaymath}
\htuse{Gamma19.gn} = \htuse{Gamma19.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma19.pub.ACCIARRI.95}
\\
\begin{ensuredisplaymath}
\htuse{Gamma26.gn} = \htuse{Gamma26.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma26.pub.ACCIARRI.95}}%
\htdef{ACCIARRI 95F.cite}{\cite{Acciarri:1995kx}}%
\htdef{ACCIARRI 95F.collab}{L3}%
\htdef{ACCIARRI 95F.ref}{ACCIARRI 95F (L3) \cite{Acciarri:1995kx}}%
\htdef{ACCIARRI 95F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma35.pub.ACCIARRI.95F}
\\
\begin{ensuredisplaymath}
\htuse{Gamma40.gn} = \htuse{Gamma40.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma40.pub.ACCIARRI.95F}}%
\htdef{ACHARD 01D.cite}{\cite{Achard:2001pk}}%
\htdef{ACHARD 01D.collab}{L3}%
\htdef{ACHARD 01D.ref}{ACHARD 01D (L3) \cite{Achard:2001pk}}%
\htdef{ACHARD 01D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma55.gn} = \htuse{Gamma55.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma55.pub.ACHARD.01D}
\\
\begin{ensuredisplaymath}
\htuse{Gamma102.gn} = \htuse{Gamma102.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma102.pub.ACHARD.01D}}%
\htdef{ADEVA 91F.cite}{\cite{Adeva:1991qq}}%
\htdef{ADEVA 91F.collab}{L3}%
\htdef{ADEVA 91F.ref}{ADEVA 91F (L3) \cite{Adeva:1991qq}}%
\htdef{ADEVA 91F.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & \htuse{L3.Gamma54.pub.ADEVA.91F}}%
\htdef{ABBIENDI 00C.cite}{\cite{Abbiendi:1999pm}}%
\htdef{ABBIENDI 00C.collab}{OPAL}%
\htdef{ABBIENDI 00C.ref}{ABBIENDI 00C (OPAL) \cite{Abbiendi:1999pm}}%
\htdef{ABBIENDI 00C.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma35.gn} = \htuse{Gamma35.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma35.pub.ABBIENDI.00C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma38.gn} = \htuse{Gamma38.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma38.pub.ABBIENDI.00C}
\\
\begin{ensuredisplaymath}
\htuse{Gamma43.gn} = \htuse{Gamma43.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma43.pub.ABBIENDI.00C}}%
\htdef{ABBIENDI 00D.cite}{\cite{Abbiendi:1999cq}}%
\htdef{ABBIENDI 00D.collab}{OPAL}%
\htdef{ABBIENDI 00D.ref}{ABBIENDI 00D (OPAL) \cite{Abbiendi:1999cq}}%
\htdef{ABBIENDI 00D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma92.gn} = \htuse{Gamma92.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma92.pub.ABBIENDI.00D}}%
\htdef{ABBIENDI 01J.cite}{\cite{Abbiendi:2000ee}}%
\htdef{ABBIENDI 01J.collab}{OPAL}%
\htdef{ABBIENDI 01J.ref}{ABBIENDI 01J (OPAL) \cite{Abbiendi:2000ee}}%
\htdef{ABBIENDI 01J.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma10.gn} = \htuse{Gamma10.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma10.pub.ABBIENDI.01J}
\\
\begin{ensuredisplaymath}
\htuse{Gamma31.gn} = \htuse{Gamma31.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma31.pub.ABBIENDI.01J}}%
\htdef{ABBIENDI 03.cite}{\cite{Abbiendi:2002jw}}%
\htdef{ABBIENDI 03.collab}{OPAL}%
\htdef{ABBIENDI 03.ref}{ABBIENDI 03 (OPAL) \cite{Abbiendi:2002jw}}%
\htdef{ABBIENDI 03.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma3.gn} = \htuse{Gamma3.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma3.pub.ABBIENDI.03}}%
\htdef{ABBIENDI 04J.cite}{\cite{Abbiendi:2004xa}}%
\htdef{ABBIENDI 04J.collab}{OPAL}%
\htdef{ABBIENDI 04J.ref}{ABBIENDI 04J (OPAL) \cite{Abbiendi:2004xa}}%
\htdef{ABBIENDI 04J.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma16.gn} = \htuse{Gamma16.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma16.pub.ABBIENDI.04J}
\\
\begin{ensuredisplaymath}
\htuse{Gamma85.gn} = \htuse{Gamma85.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma85.pub.ABBIENDI.04J}}%
\htdef{ABBIENDI 99H.cite}{\cite{Abbiendi:1998cx}}%
\htdef{ABBIENDI 99H.collab}{OPAL}%
\htdef{ABBIENDI 99H.ref}{ABBIENDI 99H (OPAL) \cite{Abbiendi:1998cx}}%
\htdef{ABBIENDI 99H.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma5.gn} = \htuse{Gamma5.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma5.pub.ABBIENDI.99H}}%
\htdef{ACKERSTAFF 98M.cite}{\cite{Ackerstaff:1997tx}}%
\htdef{ACKERSTAFF 98M.collab}{OPAL}%
\htdef{ACKERSTAFF 98M.ref}{ACKERSTAFF 98M (OPAL) \cite{Ackerstaff:1997tx}}%
\htdef{ACKERSTAFF 98M.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma8.gn} = \htuse{Gamma8.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma8.pub.ACKERSTAFF.98M}
\\
\begin{ensuredisplaymath}
\htuse{Gamma13.gn} = \htuse{Gamma13.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma13.pub.ACKERSTAFF.98M}
\\
\begin{ensuredisplaymath}
\htuse{Gamma17.gn} = \htuse{Gamma17.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma17.pub.ACKERSTAFF.98M}}%
\htdef{ACKERSTAFF 99E.cite}{\cite{Ackerstaff:1998ia}}%
\htdef{ACKERSTAFF 99E.collab}{OPAL}%
\htdef{ACKERSTAFF 99E.ref}{ACKERSTAFF 99E (OPAL) \cite{Ackerstaff:1998ia}}%
\htdef{ACKERSTAFF 99E.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma103.gn} = \htuse{Gamma103.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma103.pub.ACKERSTAFF.99E}
\\
\begin{ensuredisplaymath}
\htuse{Gamma104.gn} = \htuse{Gamma104.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma104.pub.ACKERSTAFF.99E}}%
\htdef{AKERS 94G.cite}{\cite{Akers:1994td}}%
\htdef{AKERS 94G.collab}{OPAL}%
\htdef{AKERS 94G.ref}{AKERS 94G (OPAL) \cite{Akers:1994td}}%
\htdef{AKERS 94G.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma33.gn} = \htuse{Gamma33.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma33.pub.AKERS.94G}}%
\htdef{AKERS 95Y.cite}{\cite{Akers:1995ry}}%
\htdef{AKERS 95Y.collab}{OPAL}%
\htdef{AKERS 95Y.ref}{AKERS 95Y (OPAL) \cite{Akers:1995ry}}%
\htdef{AKERS 95Y.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma55.gn} = \htuse{Gamma55.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma55.pub.AKERS.95Y}
\\
\begin{ensuredisplaymath}
\htuse{Gamma57by55.gn} = \htuse{Gamma57by55.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma57by55.pub.AKERS.95Y}}%
\htdef{ALEXANDER 91D.cite}{\cite{Alexander:1991am}}%
\htdef{ALEXANDER 91D.collab}{OPAL}%
\htdef{ALEXANDER 91D.ref}{ALEXANDER 91D (OPAL) \cite{Alexander:1991am}}%
\htdef{ALEXANDER 91D.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma7.gn} = \htuse{Gamma7.td}
\end{ensuredisplaymath} & \htuse{OPAL.Gamma7.pub.ALEXANDER.91D}}%
\htdef{AIHARA 87B.cite}{\cite{Aihara:1986mw}}%
\htdef{AIHARA 87B.collab}{TPC}%
\htdef{AIHARA 87B.ref}{AIHARA 87B (TPC) \cite{Aihara:1986mw}}%
\htdef{AIHARA 87B.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma54.gn} = \htuse{Gamma54.td}
\end{ensuredisplaymath} & \htuse{TPC.Gamma54.pub.AIHARA.87B}}%
\htdef{BAUER 94.cite}{\cite{Bauer:1993wn}}%
\htdef{BAUER 94.collab}{TPC}%
\htdef{BAUER 94.ref}{BAUER 94 (TPC) \cite{Bauer:1993wn}}%
\htdef{BAUER 94.meas}{%
\begin{ensuredisplaymath}
\htuse{Gamma82.gn} = \htuse{Gamma82.td}
\end{ensuredisplaymath} & \htuse{TPC.Gamma82.pub.BAUER.94}
\\
\begin{ensuredisplaymath}
\htuse{Gamma92.gn} = \htuse{Gamma92.td}
\end{ensuredisplaymath} & \htuse{TPC.Gamma92.pub.BAUER.94}}%
\htdef{MeasPaper}{%
\multicolumn{2}{l}{\htuse{BARATE 98.ref}} \\
\htuse{BARATE 98.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARATE 98E.ref}} \\
\htuse{BARATE 98E.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARATE 99K.ref}} \\
\htuse{BARATE 99K.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARATE 99R.ref}} \\
\htuse{BARATE 99R.meas} \\\hline
\multicolumn{2}{l}{\htuse{BUSKULIC 96.ref}} \\
\htuse{BUSKULIC 96.meas} \\\hline
\multicolumn{2}{l}{\htuse{BUSKULIC 97C.ref}} \\
\htuse{BUSKULIC 97C.meas} \\\hline
\multicolumn{2}{l}{\htuse{SCHAEL 05C.ref}} \\
\htuse{SCHAEL 05C.meas} \\\hline
\multicolumn{2}{l}{\htuse{ALBRECHT 88B.ref}} \\
\htuse{ALBRECHT 88B.meas} \\\hline
\multicolumn{2}{l}{\htuse{ALBRECHT 92D.ref}} \\
\htuse{ALBRECHT 92D.meas} \\\hline
\multicolumn{2}{l}{\htuse{AUBERT 08.ref}} \\
\htuse{AUBERT 08.meas} \\\hline
\multicolumn{2}{l}{\htuse{AUBERT 10F.ref}} \\
\htuse{AUBERT 10F.meas} \\\hline
\multicolumn{2}{l}{\htuse{DEL-AMO-SANCHEZ 11E.ref}} \\
\htuse{DEL-AMO-SANCHEZ 11E.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEES 12X.ref}} \\
\htuse{LEES 12X.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEES 12Y.ref}} \\
\htuse{LEES 12Y.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEES 18B.ref}} \\
\htuse{LEES 18B.meas} \\\hline
\multicolumn{2}{l}{\htuse{BaBar prelim. ICHEP2018.ref}} \\
\htuse{BaBar prelim. ICHEP2018.meas} \\\hline
\multicolumn{2}{l}{\htuse{FUJIKAWA 08.ref}} \\
\htuse{FUJIKAWA 08.meas} \\\hline
\multicolumn{2}{l}{\htuse{INAMI 09.ref}} \\
\htuse{INAMI 09.meas} \\\hline
\multicolumn{2}{l}{\htuse{LEE 10.ref}} \\
\htuse{LEE 10.meas} \\\hline
\multicolumn{2}{l}{\htuse{RYU 14vpc.ref}} \\
\htuse{RYU 14vpc.meas} \\\hline
\multicolumn{2}{l}{\htuse{BEHREND 89B.ref}} \\
\htuse{BEHREND 89B.meas} \\\hline
\multicolumn{2}{l}{\htuse{ANASTASSOV 01.ref}} \\
\htuse{ANASTASSOV 01.meas} \\\hline
\multicolumn{2}{l}{\htuse{ANASTASSOV 97.ref}} \\
\htuse{ANASTASSOV 97.meas} \\\hline
\multicolumn{2}{l}{\htuse{ARTUSO 92.ref}} \\
\htuse{ARTUSO 92.meas} \\\hline
\multicolumn{2}{l}{\htuse{ARTUSO 94.ref}} \\
\htuse{ARTUSO 94.meas} \\\hline
\multicolumn{2}{l}{\htuse{BALEST 95C.ref}} \\
\htuse{BALEST 95C.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARINGER 87.ref}} \\
\htuse{BARINGER 87.meas} \\\hline
\multicolumn{2}{l}{\htuse{BARTELT 96.ref}} \\
\htuse{BARTELT 96.meas} \\\hline
\multicolumn{2}{l}{\htuse{BATTLE 94.ref}} \\
\htuse{BATTLE 94.meas} \\\hline
\multicolumn{2}{l}{\htuse{BISHAI 99.ref}} \\
\htuse{BISHAI 99.meas} \\\hline
\multicolumn{2}{l}{\htuse{BORTOLETTO 93.ref}} \\
\htuse{BORTOLETTO 93.meas} \\\hline
\multicolumn{2}{l}{\htuse{COAN 96.ref}} \\
\htuse{COAN 96.meas} \\\hline
\multicolumn{2}{l}{\htuse{EDWARDS 00A.ref}} \\
\htuse{EDWARDS 00A.meas} \\\hline
\multicolumn{2}{l}{\htuse{GIBAUT 94B.ref}} \\
\htuse{GIBAUT 94B.meas} \\\hline
\multicolumn{2}{l}{\htuse{PROCARIO 93.ref}} \\
\htuse{PROCARIO 93.meas} \\\hline
\multicolumn{2}{l}{\htuse{RICHICHI 99.ref}} \\
\htuse{RICHICHI 99.meas} \\\hline
\multicolumn{2}{l}{\htuse{ARMS 05.ref}} \\
\htuse{ARMS 05.meas} \\\hline
\multicolumn{2}{l}{\htuse{BRIERE 03.ref}} \\
\htuse{BRIERE 03.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABDALLAH 06A.ref}} \\
\htuse{ABDALLAH 06A.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABREU 92N.ref}} \\
\htuse{ABREU 92N.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABREU 94K.ref}} \\
\htuse{ABREU 94K.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABREU 99X.ref}} \\
\htuse{ABREU 99X.meas} \\\hline
\multicolumn{2}{l}{\htuse{BYLSMA 87.ref}} \\
\htuse{BYLSMA 87.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACCIARRI 01F.ref}} \\
\htuse{ACCIARRI 01F.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACCIARRI 95.ref}} \\
\htuse{ACCIARRI 95.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACCIARRI 95F.ref}} \\
\htuse{ACCIARRI 95F.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACHARD 01D.ref}} \\
\htuse{ACHARD 01D.meas} \\\hline
\multicolumn{2}{l}{\htuse{ADEVA 91F.ref}} \\
\htuse{ADEVA 91F.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 00C.ref}} \\
\htuse{ABBIENDI 00C.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 00D.ref}} \\
\htuse{ABBIENDI 00D.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 01J.ref}} \\
\htuse{ABBIENDI 01J.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 03.ref}} \\
\htuse{ABBIENDI 03.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 04J.ref}} \\
\htuse{ABBIENDI 04J.meas} \\\hline
\multicolumn{2}{l}{\htuse{ABBIENDI 99H.ref}} \\
\htuse{ABBIENDI 99H.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACKERSTAFF 98M.ref}} \\
\htuse{ACKERSTAFF 98M.meas} \\\hline
\multicolumn{2}{l}{\htuse{ACKERSTAFF 99E.ref}} \\
\htuse{ACKERSTAFF 99E.meas} \\\hline
\multicolumn{2}{l}{\htuse{AKERS 94G.ref}} \\
\htuse{AKERS 94G.meas} \\\hline
\multicolumn{2}{l}{\htuse{AKERS 95Y.ref}} \\
\htuse{AKERS 95Y.meas} \\\hline
\multicolumn{2}{l}{\htuse{ALEXANDER 91D.ref}} \\
\htuse{ALEXANDER 91D.meas} \\\hline
\multicolumn{2}{l}{\htuse{AIHARA 87B.ref}} \\
\htuse{AIHARA 87B.meas} \\\hline
\multicolumn{2}{l}{\htuse{BAUER 94.ref}} \\
\htuse{BAUER 94.meas}}%
\htdef{BrStrangeVal}{%
\htQuantLine{Gamma10}{0.6986 \pm 0.0085}{-2} 
\htQuantLine{Gamma16}{0.4904 \pm 0.0092}{-2} 
\htQuantLine{Gamma23}{0.0585 \pm 0.0027}{-2} 
\htQuantLine{Gamma28}{0.0113 \pm 0.0026}{-2} 
\htQuantLine{Gamma35}{0.8378 \pm 0.0139}{-2} 
\htQuantLine{Gamma40}{0.3807 \pm 0.0129}{-2} 
\htQuantLine{Gamma44}{0.0235 \pm 0.0231}{-2} 
\htQuantLine{Gamma53}{0.0222 \pm 0.0202}{-2} 
\htQuantLine{Gamma128}{0.0154 \pm 0.0008}{-2} 
\htQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\htQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\htQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\htQuantLine{Gamma168}{0.0022 \pm 0.0008}{-2} 
\htQuantLine{Gamma169}{0.0015 \pm 0.0006}{-2} 
\htQuantLine{Gamma802}{0.2923 \pm 0.0067}{-2} 
\htQuantLine{Gamma803}{0.0410 \pm 0.0143}{-2} 
\htQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\htQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2}}%
\htdef{BrStrangeTotVal}{%
\htQuantLine{Gamma110}{2.9308 \pm 0.0412}{-2}}%
\htdef{UnitarityQuants}{%
\htConstrLine{Gamma3}{17.3915 \pm 0.0395}{1.0000}{-2}{0} 
\htConstrLine{Gamma5}{17.8171 \pm 0.0409}{1.0000}{-2}{0} 
\htConstrLine{Gamma9}{10.8036 \pm 0.0519}{1.0000}{-2}{0} 
\htConstrLine{Gamma10}{0.6986 \pm 0.0085}{1.0000}{-2}{0} 
\htConstrLine{Gamma14}{25.4475 \pm 0.0908}{1.0000}{-2}{0} 
\htConstrLine{Gamma16}{0.4904 \pm 0.0092}{1.0000}{-2}{0} 
\htConstrLine{Gamma20}{9.2114 \pm 0.0921}{1.0000}{-2}{0} 
\htConstrLine{Gamma23}{0.0585 \pm 0.0027}{1.0000}{-2}{0} 
\htConstrLine{Gamma27}{1.1381 \pm 0.0292}{1.0000}{-2}{0} 
\htConstrLine{Gamma28}{0.0113 \pm 0.0026}{1.0000}{-2}{0} 
\htConstrLine{Gamma30}{0.0864 \pm 0.0067}{1.0000}{-2}{0} 
\htConstrLine{Gamma35}{0.8378 \pm 0.0139}{1.0000}{-2}{0} 
\htConstrLine{Gamma37}{0.1483 \pm 0.0034}{1.0000}{-2}{0} 
\htConstrLine{Gamma40}{0.3807 \pm 0.0129}{1.0000}{-2}{0} 
\htConstrLine{Gamma42}{0.1494 \pm 0.0070}{1.0000}{-2}{0} 
\htConstrLine{Gamma44}{0.0235 \pm 0.0231}{1.0000}{-2}{0} 
\htConstrLine{Gamma47}{0.0234 \pm 0.0006}{2.0000}{-2}{0} 
\htConstrLine{Gamma48}{0.1048 \pm 0.0247}{1.0000}{-2}{0} 
\htConstrLine{Gamma50}{0.0018 \pm 0.0002}{2.0000}{-2}{0} 
\htConstrLine{Gamma51}{0.0318 \pm 0.0119}{1.0000}{-2}{0} 
\htConstrLine{Gamma53}{0.0222 \pm 0.0202}{1.0000}{-2}{0} 
\htConstrLine{Gamma62}{8.9596 \pm 0.0511}{1.0000}{-2}{0} 
\htConstrLine{Gamma70}{2.7703 \pm 0.0710}{1.0000}{-2}{0} 
\htConstrLine{Gamma77}{0.0981 \pm 0.0356}{1.0000}{-2}{0} 
\htConstrLine{Gamma93}{0.1431 \pm 0.0027}{1.0000}{-2}{0} 
\htConstrLine{Gamma94}{0.0061 \pm 0.0018}{1.0000}{-2}{0} 
\htConstrLine{Gamma126}{0.1386 \pm 0.0072}{1.0000}{-2}{0} 
\htConstrLine{Gamma128}{0.0154 \pm 0.0008}{1.0000}{-2}{0} 
\htConstrLine{Gamma130}{0.0048 \pm 0.0012}{1.0000}{-2}{0} 
\htConstrLine{Gamma132}{0.0094 \pm 0.0015}{1.0000}{-2}{0} 
\htConstrLine{Gamma136}{0.0220 \pm 0.0013}{1.0000}{-2}{0} 
\htConstrLine{Gamma151}{0.0410 \pm 0.0092}{1.0000}{-2}{0} 
\htConstrLine{Gamma152}{0.4066 \pm 0.0419}{1.0000}{-2}{0} 
\htConstrLine{Gamma167}{0.0044 \pm 0.0016}{0.8320}{-2}{0} 
\htConstrLine{Gamma800}{1.9546 \pm 0.0647}{1.0000}{-2}{0} 
\htConstrLine{Gamma802}{0.2923 \pm 0.0067}{1.0000}{-2}{0} 
\htConstrLine{Gamma803}{0.0410 \pm 0.0143}{1.0000}{-2}{0} 
\htConstrLine{Gamma805}{0.0400 \pm 0.0200}{1.0000}{-2}{0} 
\htConstrLine{Gamma811}{0.0071 \pm 0.0016}{1.0000}{-2}{0} 
\htConstrLine{Gamma812}{0.0013 \pm 0.0027}{1.0000}{-2}{0} 
\htConstrLine{Gamma821}{0.0772 \pm 0.0030}{1.0000}{-2}{0} 
\htConstrLine{Gamma822}{0.0001 \pm 0.0001}{1.0000}{-2}{0} 
\htConstrLine{Gamma831}{0.0084 \pm 0.0006}{1.0000}{-2}{0} 
\htConstrLine{Gamma832}{0.0038 \pm 0.0009}{1.0000}{-2}{0} 
\htConstrLine{Gamma833}{0.0001 \pm 0.0001}{1.0000}{-2}{0} 
\htConstrLine{Gamma920}{0.0052 \pm 0.0004}{1.0000}{-2}{0} 
\htConstrLine{Gamma945}{0.0194 \pm 0.0038}{1.0000}{-2}{0} 
\htConstrLine{Gamma998}{0.0274 \pm 0.1026}{1.0000}{-2}{0}}%
\htdef{BaseQuants}{%
\htQuantLine{Gamma3}{17.3915 \pm 0.0395}{-2} 
\htQuantLine{Gamma5}{17.8171 \pm 0.0409}{-2} 
\htQuantLine{Gamma9}{10.8036 \pm 0.0519}{-2} 
\htQuantLine{Gamma10}{0.6986 \pm 0.0085}{-2} 
\htQuantLine{Gamma14}{25.4475 \pm 0.0908}{-2} 
\htQuantLine{Gamma16}{0.4904 \pm 0.0092}{-2} 
\htQuantLine{Gamma20}{9.2114 \pm 0.0921}{-2} 
\htQuantLine{Gamma23}{0.0585 \pm 0.0027}{-2} 
\htQuantLine{Gamma27}{1.1381 \pm 0.0292}{-2} 
\htQuantLine{Gamma28}{0.0113 \pm 0.0026}{-2} 
\htQuantLine{Gamma30}{0.0864 \pm 0.0067}{-2} 
\htQuantLine{Gamma35}{0.8378 \pm 0.0139}{-2} 
\htQuantLine{Gamma37}{0.1483 \pm 0.0034}{-2} 
\htQuantLine{Gamma40}{0.3807 \pm 0.0129}{-2} 
\htQuantLine{Gamma42}{0.1494 \pm 0.0070}{-2} 
\htQuantLine{Gamma44}{0.0235 \pm 0.0231}{-2} 
\htQuantLine{Gamma47}{0.0234 \pm 0.0006}{-2} 
\htQuantLine{Gamma48}{0.1048 \pm 0.0247}{-2} 
\htQuantLine{Gamma50}{0.0018 \pm 0.0002}{-2} 
\htQuantLine{Gamma51}{0.0318 \pm 0.0119}{-2} 
\htQuantLine{Gamma53}{0.0222 \pm 0.0202}{-2} 
\htQuantLine{Gamma62}{8.9596 \pm 0.0511}{-2} 
\htQuantLine{Gamma70}{2.7703 \pm 0.0710}{-2} 
\htQuantLine{Gamma77}{0.0981 \pm 0.0356}{-2} 
\htQuantLine{Gamma93}{0.1431 \pm 0.0027}{-2} 
\htQuantLine{Gamma94}{0.0061 \pm 0.0018}{-2} 
\htQuantLine{Gamma126}{0.1386 \pm 0.0072}{-2} 
\htQuantLine{Gamma128}{0.0154 \pm 0.0008}{-2} 
\htQuantLine{Gamma130}{0.0048 \pm 0.0012}{-2} 
\htQuantLine{Gamma132}{0.0094 \pm 0.0015}{-2} 
\htQuantLine{Gamma136}{0.0220 \pm 0.0013}{-2} 
\htQuantLine{Gamma151}{0.0410 \pm 0.0092}{-2} 
\htQuantLine{Gamma152}{0.4066 \pm 0.0419}{-2} 
\htQuantLine{Gamma167}{0.0044 \pm 0.0016}{-2} 
\htQuantLine{Gamma800}{1.9546 \pm 0.0647}{-2} 
\htQuantLine{Gamma802}{0.2923 \pm 0.0067}{-2} 
\htQuantLine{Gamma803}{0.0410 \pm 0.0143}{-2} 
\htQuantLine{Gamma805}{0.0400 \pm 0.0200}{-2} 
\htQuantLine{Gamma811}{0.0071 \pm 0.0016}{-2} 
\htQuantLine{Gamma812}{0.0013 \pm 0.0027}{-2} 
\htQuantLine{Gamma821}{0.0772 \pm 0.0030}{-2} 
\htQuantLine{Gamma822}{0.0001 \pm 0.0001}{-2} 
\htQuantLine{Gamma831}{0.0084 \pm 0.0006}{-2} 
\htQuantLine{Gamma832}{0.0038 \pm 0.0009}{-2} 
\htQuantLine{Gamma833}{0.0001 \pm 0.0001}{-2} 
\htQuantLine{Gamma920}{0.0052 \pm 0.0004}{-2} 
\htQuantLine{Gamma945}{0.0194 \pm 0.0038}{-2}}%
\htdef{BrCorr}{%
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 1.\label{tab:tau:br-fit-corr1}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 1.}\label{tab:tau:br-fit-corr1}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{5} \) &   22 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{9} \) &    6 &    4 &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{10} \) &    2 &    4 &    2 &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{14} \) &  -13 &  -14 &  -13 &   -7 &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{16} \) &   -2 &   -1 &   -3 &   35 &  -13 &  &  &  &  &  &  &  &  &  \\
\( \BR_{20} \) &   -7 &   -7 &  -12 &   -4 &  -42 &  -16 &  &  &  &  &  &  &  &  \\
\( \BR_{23} \) &   -3 &   -2 &   -5 &   14 &   -9 &   66 &  -18 &  &  &  &  &  &  &  \\
\( \BR_{27} \) &   -4 &   -4 &   -7 &    3 &   -9 &   61 &  -23 &   72 &  &  &  &  &  &  \\
\( \BR_{28} \) &   -2 &   -1 &   -3 &    2 &   -4 &   32 &  -10 &   28 &   37 &  &  &  &  &  \\
\( \BR_{30} \) &   -3 &   -3 &   -6 &   -1 &   -6 &   34 &  -14 &   41 &   52 &   23 &  &  &  &  \\
\( \BR_{35} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  \\
\( \BR_{37} \) &    0 &   -1 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &  -15 &  &  \\
\( \BR_{40} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &  -12 &    2 &  \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 2.\label{tab:tau:br-fit-corr2}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 2.}\label{tab:tau:br-fit-corr2}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{42} \) &    0 &    0 &    0 &   -2 &    1 &   -5 &    1 &   -4 &   -4 &   -2 &   -2 &   -1 &  -15 &  -20 \\
\( \BR_{44} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -4 \\
\( \BR_{47} \) &    0 &   -1 &    2 &    1 &   -1 &    2 &   -1 &    1 &    1 &    0 &    0 &   -1 &    2 &   -4 \\
\( \BR_{48} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -3 &    0 &   -2 \\
\( \BR_{50} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    5 &    0 \\
\( \BR_{51} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &   -1 \\
\( \BR_{53} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{62} \) &   -4 &   -5 &    6 &    2 &   -4 &    1 &  -11 &   -1 &   -2 &   -2 &   -3 &   -1 &    3 &    0 \\
\( \BR_{70} \) &   -5 &   -6 &   -7 &   -2 &   -8 &   -1 &   -1 &   -1 &   -1 &    0 &    0 &    0 &   -1 &    0 \\
\( \BR_{77} \) &    0 &    0 &   -2 &    0 &   -2 &    1 &    0 &    1 &    2 &    1 &    1 &    0 &    0 &    0 \\
\( \BR_{93} \) &   -1 &   -1 &    2 &    1 &   -1 &    1 &   -2 &    0 &    0 &    0 &    0 &    0 &    1 &    0 \\
\( \BR_{94} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{126} \) &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{128} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 3.\label{tab:tau:br-fit-corr3}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 3.}\label{tab:tau:br-fit-corr3}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{130} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{132} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{136} \) &    0 &    0 &    1 &    1 &    0 &    1 &   -1 &    0 &    0 &    0 &    0 &    0 &    1 &    0 \\
\( \BR_{151} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{152} \) &    0 &    0 &   -3 &    0 &   -2 &    1 &    0 &    1 &    2 &    1 &    2 &    0 &    0 &    0 \\
\( \BR_{167} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{800} \) &   -1 &   -1 &   -2 &    0 &   -3 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{802} \) &   -1 &   -1 &    0 &    0 &   -1 &   -1 &   -3 &   -1 &   -2 &   -1 &   -1 &    0 &    0 &    0 \\
\( \BR_{803} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{805} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{811} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{812} \) &    1 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{821} \) &    0 &    0 &    2 &    1 &    0 &    1 &   -2 &    0 &    0 &    0 &    0 &    0 &    1 &    0 \\
\( \BR_{822} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 4.\label{tab:tau:br-fit-corr4}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 4.}\label{tab:tau:br-fit-corr4}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{831} \) &    0 &    0 &    1 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    1 &    0 \\
\( \BR_{832} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{833} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{920} \) &    0 &    0 &    1 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{945} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{3} \) & \( \BR_{5} \) & \( \BR_{9} \) & \( \BR_{10} \) & \( \BR_{14} \) & \( \BR_{16} \) & \( \BR_{20} \) & \( \BR_{23} \) & \( \BR_{27} \) & \( \BR_{28} \) & \( \BR_{30} \) & \( \BR_{35} \) & \( \BR_{37} \) & \( \BR_{40} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 5.\label{tab:tau:br-fit-corr5}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 5.}\label{tab:tau:br-fit-corr5}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{44} \) &    0 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{47} \) &    1 &    0 &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{48} \) &   -1 &   -6 &    0 &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{50} \) &    6 &    0 &   -7 &    0 &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{51} \) &    0 &   -3 &    0 &   -6 &    0 &  &  &  &  &  &  &  &  &  \\
\( \BR_{53} \) &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  &  &  &  &  &  \\
\( \BR_{62} \) &   -1 &    0 &    5 &    0 &    1 &    0 &    0 &  &  &  &  &  &  &  \\
\( \BR_{70} \) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &  -19 &  &  &  &  &  &  \\
\( \BR_{77} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &   -7 &  &  &  &  &  \\
\( \BR_{93} \) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &   14 &   -4 &    0 &  &  &  &  \\
\( \BR_{94} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -2 &    0 &    0 &  &  &  \\
\( \BR_{126} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -5 &    0 &    0 &  &  \\
\( \BR_{128} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &    0 &    0 &    1 &    0 &    4 &  \\
 & \( \BR_{42} \) & \( \BR_{44} \) & \( \BR_{47} \) & \( \BR_{48} \) & \( \BR_{50} \) & \( \BR_{51} \) & \( \BR_{53} \) & \( \BR_{62} \) & \( \BR_{70} \) & \( \BR_{77} \) & \( \BR_{93} \) & \( \BR_{94} \) & \( \BR_{126} \) & \( \BR_{128} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 6.\label{tab:tau:br-fit-corr6}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 6.}\label{tab:tau:br-fit-corr6}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{130} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    1 \\
\( \BR_{132} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    1 \\
\( \BR_{136} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    2 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{151} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   12 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{152} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  -11 &  -64 &    0 &    0 &    0 &    0 \\
\( \BR_{167} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{800} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -8 &  -69 &   -2 &   -1 &    0 &    0 &    0 \\
\( \BR_{802} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   16 &   -6 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{803} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  -19 &    0 &    0 &   -2 &    0 &   -1 \\
\( \BR_{805} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{811} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{812} \) &    0 &    0 &    0 &    0 &   -1 &    0 &    0 &   -1 &   -1 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{821} \) &    0 &    0 &    2 &    0 &    0 &    0 &    0 &    3 &   -1 &    0 &    1 &    0 &    0 &    1 \\
\( \BR_{822} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{42} \) & \( \BR_{44} \) & \( \BR_{47} \) & \( \BR_{48} \) & \( \BR_{50} \) & \( \BR_{51} \) & \( \BR_{53} \) & \( \BR_{62} \) & \( \BR_{70} \) & \( \BR_{77} \) & \( \BR_{93} \) & \( \BR_{94} \) & \( \BR_{126} \) & \( \BR_{128} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 7.\label{tab:tau:br-fit-corr7}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 7.}\label{tab:tau:br-fit-corr7}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{831} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{832} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{833} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
\( \BR_{920} \) &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    1 &   -1 &    0 &    1 &    0 &    0 &    0 \\
\( \BR_{945} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\
 & \( \BR_{42} \) & \( \BR_{44} \) & \( \BR_{47} \) & \( \BR_{48} \) & \( \BR_{50} \) & \( \BR_{51} \) & \( \BR_{53} \) & \( \BR_{62} \) & \( \BR_{70} \) & \( \BR_{77} \) & \( \BR_{93} \) & \( \BR_{94} \) & \( \BR_{126} \) & \( \BR_{128} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 8.\label{tab:tau:br-fit-corr8}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 8.}\label{tab:tau:br-fit-corr8}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{132} \) &    0 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{136} \) &    0 &    0 &  &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{151} \) &    0 &    0 &    0 &  &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{152} \) &    0 &    0 &    0 &    0 &  &  &  &  &  &  &  &  &  &  \\
\( \BR_{167} \) &    0 &    0 &    0 &    0 &    0 &  &  &  &  &  &  &  &  &  \\
\( \BR_{800} \) &    0 &    0 &    0 &  -14 &   -3 &    0 &  &  &  &  &  &  &  &  \\
\( \BR_{802} \) &    0 &    0 &    0 &   -2 &    0 &    1 &   -1 &  &  &  &  &  &  &  \\
\( \BR_{803} \) &    0 &    0 &    0 &  -58 &    0 &    0 &    9 &    1 &  &  &  &  &  &  \\
\( \BR_{805} \) &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  &  &  \\
\( \BR_{811} \) &    0 &   -1 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  &  &  &  \\
\( \BR_{812} \) &    0 &   -2 &   -8 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  -16 &  &  &  \\
\( \BR_{821} \) &    0 &    0 &   46 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    8 &   -4 &  &  \\
\( \BR_{822} \) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &  \\
 & \( \BR_{130} \) & \( \BR_{132} \) & \( \BR_{136} \) & \( \BR_{151} \) & \( \BR_{152} \) & \( \BR_{167} \) & \( \BR_{800} \) & \( \BR_{802} \) & \( \BR_{803} \) & \( \BR_{805} \) & \( \BR_{811} \) & \( \BR_{812} \) & \( \BR_{821} \) & \( \BR_{822} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 9.\label{tab:tau:br-fit-corr9}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 9.}\label{tab:tau:br-fit-corr9}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrrrrrrrrrrr}
\hline
\( \BR_{831} \) &    0 &    0 &   38 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   14 &   -4 &   39 &   -1 \\
\( \BR_{832} \) &    0 &    0 &    3 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    3 &    0 \\
\( \BR_{833} \) &    0 &    0 &   -1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   -1 &    0 \\
\( \BR_{920} \) &    0 &    0 &   20 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    3 &   -2 &   34 &   -1 \\
\( \BR_{945} \) &    0 &   -1 &   25 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   10 &  -11 &   10 &    0 \\
 & \( \BR_{130} \) & \( \BR_{132} \) & \( \BR_{136} \) & \( \BR_{151} \) & \( \BR_{152} \) & \( \BR_{167} \) & \( \BR_{800} \) & \( \BR_{802} \) & \( \BR_{803} \) & \( \BR_{805} \) & \( \BR_{811} \) & \( \BR_{812} \) & \( \BR_{821} \) & \( \BR_{822} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
%
%
%
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Basis quantities correlation coefficients in percent, subtable 10.\label{tab:tau:br-fit-corr10}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Basis quantities correlation coefficients in percent, subtable 10.}\label{tab:tau:br-fit-corr10}%
\fi
\begin{envsmall}
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{rrrrrr}
\hline
\( \BR_{832} \) &   -2 &  &  &  &  \\
\( \BR_{833} \) &   -1 &   -1 &  &  &  \\
\( \BR_{920} \) &   17 &    1 &    0 &  &  \\
\( \BR_{945} \) &   17 &    2 &    0 &    4 &  \\
 & \( \BR_{831} \) & \( \BR_{832} \) & \( \BR_{833} \) & \( \BR_{920} \) & \( \BR_{945} \)
\\\hline
\end{tabular}
\end{center}
\end{envsmall}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi}%
\htconstrdef{Gamma1.c}{\BR_{1}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} + \BR_{40} + \BR_{44} + \BR_{37} + \BR_{42} + \BR_{47} + \BR_{48} + \BR_{804} + \BR_{50} + \BR_{51} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16}  \\ 
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}  \\ 
  {}& + \BR_{40} + \BR_{44} + \BR_{37} + \BR_{42} + \BR_{47} + \BR_{48}  \\ 
  {}& + \BR_{804} + \BR_{50} + \BR_{51} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma}  \\ 
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}%
\htconstrdef{Gamma2.c}{\BR_{2}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{40}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{44}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{37}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{42}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^0\pi^0} + \BR_{804} + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^0\pi^0} + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}(\BR_{\eta\to\text{neutral}}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>})) + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16}  \\ 
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\ 
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{40}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{44}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\ 
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{37}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{42}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0} \\ 
  {}& +\BR_{<\bar{K}^0|K_L>}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^0\pi^0}  \\ 
  {}& + \BR_{804} + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^0\pi^0}  \\ 
  {}& + \BR_{806} + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{132}\cdot{}(\BR_{\eta\to\text{neutral}}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>})) + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}  \\ 
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma3by5.c}{\frac{\BR_{3}}{\BR_{5}}}{\frac{\BR_{3}}{\BR_{5}}}{\frac{\BR_{3}}{\BR_{5}}}%
\htconstrdef{Gamma7.c}{\BR_{7}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_L>} + \BR_{9} + \BR_{804} + \BR_{37}\cdot{}\BR_{<K^0|K_L>} + \BR_{10}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_L>} + \BR_{9} + \BR_{804} + \BR_{37}\cdot{}\BR_{<K^0|K_L>}  \\ 
  {}& + \BR_{10}}%
\htconstrdef{Gamma8.c}{\BR_{8}}{\BR_{9} + \BR_{10}}{\BR_{9} + \BR_{10}}%
\htconstrdef{Gamma8by5.c}{\frac{\BR_{8}}{\BR_{5}}}{\frac{\BR_{8}}{\BR_{5}}}{\frac{\BR_{8}}{\BR_{5}}}%
\htconstrdef{Gamma9by5.c}{\frac{\BR_{9}}{\BR_{5}}}{\frac{\BR_{9}}{\BR_{5}}}{\frac{\BR_{9}}{\BR_{5}}}%
\htconstrdef{Gamma10by5.c}{\frac{\BR_{10}}{\BR_{5}}}{\frac{\BR_{10}}{\BR_{5}}}{\frac{\BR_{10}}{\BR_{5}}}%
\htconstrdef{Gamma10by9.c}{\frac{\BR_{10}}{\BR_{9}}}{\frac{\BR_{10}}{\BR_{9}}}{\frac{\BR_{10}}{\BR_{9}}}%
\htconstrdef{Gamma11.c}{\BR_{11}}{\BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}}{\BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28}  \\ 
  {}& + \BR_{30} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{126}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^0\gamma}  \\ 
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^0\gamma} + \BR_{800}\cdot{}\BR_{\omega\to\pi^0\gamma}}%
\htconstrdef{Gamma12.c}{\BR_{12}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{14}  \\ 
  {}& + \BR_{16} + \BR_{20} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma13.c}{\BR_{13}}{\BR_{14} + \BR_{16}}{\BR_{14} + \BR_{16}}%
\htconstrdef{Gamma17.c}{\BR_{17}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{27} + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{23} + \BR_{28} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{20} + \BR_{27} + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma18.c}{\BR_{18}}{\BR_{23} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{23} + \BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{20} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma19.c}{\BR_{19}}{\BR_{23} + \BR_{20}}{\BR_{23} + \BR_{20}}%
\htconstrdef{Gamma19by13.c}{\frac{\BR_{19}}{\BR_{13}}}{\frac{\BR_{19}}{\BR_{13}}}{\frac{\BR_{19}}{\BR_{13}}}%
\htconstrdef{Gamma24.c}{\BR_{24}}{\BR_{27} + \BR_{28} + \BR_{30} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to3\pi^0})}{\BR_{27} + \BR_{28} + \BR_{30} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{47}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{50}\cdot{}(\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to3\pi^0}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{132}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to3\pi^0})}%
\htconstrdef{Gamma25.c}{\BR_{25}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{28} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{30} + \BR_{28} + \BR_{27} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma26.c}{\BR_{26}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{28} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{27}}{\BR_{128}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{28} + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{27}}%
\htconstrdef{Gamma26by13.c}{\frac{\BR_{26}}{\BR_{13}}}{\frac{\BR_{26}}{\BR_{13}}}{\frac{\BR_{26}}{\BR_{13}}}%
\htconstrdef{Gamma29.c}{\BR_{29}}{\BR_{30} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{30} + \BR_{126}\cdot{}\BR_{\eta\to3\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma31.c}{\BR_{31}}{\BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{23} + \BR_{28} + \BR_{42} + \BR_{16} + \BR_{37} + \BR_{10} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{23} + \BR_{28} + \BR_{42} + \BR_{16}  \\ 
  {}& + \BR_{37} + \BR_{10} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma32.c}{\BR_{32}}{\BR_{16} + \BR_{23} + \BR_{28} + \BR_{37} + \BR_{42} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}{\BR_{16} + \BR_{23} + \BR_{28} + \BR_{37} + \BR_{42} + \BR_{128}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{167}\cdot{}(\BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^0\pi^0})}%
\htconstrdef{Gamma33.c}{\BR_{33}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{40}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{42}\cdot{}\BR_{<K^0|K_S>} + \BR_{47} + \BR_{48} + \BR_{50} + \BR_{51} + \BR_{37}\cdot{}\BR_{<K^0|K_S>} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}{\BR_{35}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{40}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{42}\cdot{}\BR_{<K^0|K_S>}  \\ 
  {}& + \BR_{47} + \BR_{48} + \BR_{50} + \BR_{51} + \BR_{37}\cdot{}\BR_{<K^0|K_S>}  \\ 
  {}& + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{\eta\to\text{neutral}}) + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}%
\htconstrdef{Gamma34.c}{\BR_{34}}{\BR_{35} + \BR_{37}}{\BR_{35} + \BR_{37}}%
\htconstrdef{Gamma38.c}{\BR_{38}}{\BR_{42} + \BR_{37}}{\BR_{42} + \BR_{37}}%
\htconstrdef{Gamma39.c}{\BR_{39}}{\BR_{40} + \BR_{42}}{\BR_{40} + \BR_{42}}%
\htconstrdef{Gamma43.c}{\BR_{43}}{\BR_{40} + \BR_{44}}{\BR_{40} + \BR_{44}}%
\htconstrdef{Gamma46.c}{\BR_{46}}{\BR_{48} + \BR_{47} + \BR_{804}}{\BR_{48} + \BR_{47} + \BR_{804}}%
\htconstrdef{Gamma49.c}{\BR_{49}}{\BR_{50} + \BR_{51} + \BR_{806}}{\BR_{50} + \BR_{51} + \BR_{806}}%
\htconstrdef{Gamma54.c}{\BR_{54}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^+\pi^-} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^+\pi^-} + \BR_{53}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{93} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_L>}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-} + \BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{48}\cdot{}\BR_{K_S\to\pi^+\pi^-}  \\ 
  {}& + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{51}\cdot{}\BR_{K_S\to\pi^+\pi^-}  \\ 
  {}& + \BR_{53}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}+\BR_{<\bar{K}^0|K_L>}) + \BR_{62} + \BR_{70}  \\ 
  {}& + \BR_{77} + \BR_{78} + \BR_{93} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_L>}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})  \\ 
  {}& + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})  \\ 
  {}& + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-} + \BR_{\phi\to K_S K_L}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803}  \\ 
  {}& + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}%
\htconstrdef{Gamma55.c}{\BR_{55}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{78} + \BR_{77} + \BR_{94} + \BR_{62} + \BR_{70} + \BR_{93} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{168}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{78}  \\ 
  {}& + \BR_{77} + \BR_{94} + \BR_{62} + \BR_{70} + \BR_{93} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}}  \\ 
  {}& + \BR_{802} + \BR_{803} + \BR_{800}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{168}}%
\htconstrdef{Gamma56.c}{\BR_{56}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{93} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{168}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{93} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{168}}%
\htconstrdef{Gamma57.c}{\BR_{57}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}  \\ 
  {}& + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma57by55.c}{\frac{\BR_{57}}{\BR_{55}}}{\frac{\BR_{57}}{\BR_{55}}}{\frac{\BR_{57}}{\BR_{55}}}%
\htconstrdef{Gamma58.c}{\BR_{58}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{62} + \BR_{93} + \BR_{802} + \BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma59.c}{\BR_{59}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{35}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma60.c}{\BR_{60}}{\BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{62} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma63.c}{\BR_{63}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to\text{neutral}} + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{charged}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{70} + \BR_{77} + \BR_{78} + \BR_{94} + \BR_{126}\cdot{}\BR_{\eta\to\text{charged}}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{130}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to\text{neutral}}  \\ 
  {}& + \BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^0\pi^0}\cdot{}\BR_{\eta\to\text{charged}}) + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma64.c}{\BR_{64}}{\BR_{78} + \BR_{77} + \BR_{94} + \BR_{70} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{803}}{\BR_{78} + \BR_{77} + \BR_{94} + \BR_{70} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{803}}%
\htconstrdef{Gamma65.c}{\BR_{65}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma66.c}{\BR_{66}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma67.c}{\BR_{67}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{70} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803}}%
\htconstrdef{Gamma68.c}{\BR_{68}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{40}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{70} + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-}  \\ 
  {}& + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma69.c}{\BR_{69}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{70} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{70} + \BR_{800}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma74.c}{\BR_{74}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{78} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{78} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma75.c}{\BR_{75}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{47}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0})  \\ 
  {}& + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma76.c}{\BR_{76}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{77} + \BR_{126}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{130}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma76by54.c}{\frac{\BR_{76}}{\BR_{54}}}{\frac{\BR_{76}}{\BR_{54}}}{\frac{\BR_{76}}{\BR_{54}}}%
\htconstrdef{Gamma78.c}{\BR_{78}}{\BR_{810} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})}{\BR_{810} + \BR_{50}\cdot{}(2\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{K_S\to\pi^0\pi^0}) + \BR_{132}\cdot{}(\BR_{<\bar{K}^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}\cdot{}\BR_{\eta\to3\pi^0})}%
\htconstrdef{Gamma79.c}{\BR_{79}}{\BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{93} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{168} + \BR_{802} + \BR_{803}}{\BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})  \\ 
  {}& + \BR_{93} + \BR_{94} + \BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-}) + \BR_{168} + \BR_{802} + \BR_{803}}%
\htconstrdef{Gamma80.c}{\BR_{80}}{\BR_{93} + \BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{93} + \BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma80by60.c}{\frac{\BR_{80}}{\BR_{60}}}{\frac{\BR_{80}}{\BR_{60}}}{\frac{\BR_{80}}{\BR_{60}}}%
\htconstrdef{Gamma81.c}{\BR_{81}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{94} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{94} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma81by69.c}{\frac{\BR_{81}}{\BR_{69}}}{\frac{\BR_{81}}{\BR_{69}}}{\frac{\BR_{81}}{\BR_{69}}}%
\htconstrdef{Gamma82.c}{\BR_{82}}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}{\BR_{128}\cdot{}\BR_{\eta\to\text{charged}} + \BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{802}  \\ 
  {}& + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-}) + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}%
\htconstrdef{Gamma83.c}{\BR_{83}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0}+\BR_{\omega\to\pi^+\pi^-})}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{802} + \BR_{803} + \BR_{151}\cdot{}(\BR_{\omega\to\pi^+\pi^-\pi^0} \\ 
  {}& +\BR_{\omega\to\pi^+\pi^-})}%
\htconstrdef{Gamma84.c}{\BR_{84}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-} + \BR_{37}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-})}%
\htconstrdef{Gamma85.c}{\BR_{85}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{802} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma85by60.c}{\frac{\BR_{85}}{\BR_{60}}}{\frac{\BR_{85}}{\BR_{60}}}{\frac{\BR_{85}}{\BR_{60}}}%
\htconstrdef{Gamma87.c}{\BR_{87}}{\BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{803}}{\BR_{42}\cdot{}(\BR_{<K^0|K_S>}\cdot{}\BR_{K_S\to\pi^+\pi^-}) + \BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}  \\ 
  {}& + \BR_{803}}%
\htconstrdef{Gamma88.c}{\BR_{88}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{128}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0} + \BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma89.c}{\BR_{89}}{\BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{803} + \BR_{151}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma92.c}{\BR_{92}}{\BR_{94} + \BR_{93}}{\BR_{94} + \BR_{93}}%
\htconstrdef{Gamma93by60.c}{\frac{\BR_{93}}{\BR_{60}}}{\frac{\BR_{93}}{\BR_{60}}}{\frac{\BR_{93}}{\BR_{60}}}%
\htconstrdef{Gamma94by69.c}{\frac{\BR_{94}}{\BR_{69}}}{\frac{\BR_{94}}{\BR_{69}}}{\frac{\BR_{94}}{\BR_{69}}}%
\htconstrdef{Gamma96.c}{\BR_{96}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma102.c}{\BR_{102}}{\BR_{103} + \BR_{104}}{\BR_{103} + \BR_{104}}%
\htconstrdef{Gamma103.c}{\BR_{103}}{\BR_{820} + \BR_{822} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-}}{\BR_{820} + \BR_{822} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-}}%
\htconstrdef{Gamma104.c}{\BR_{104}}{\BR_{830} + \BR_{833}}{\BR_{830} + \BR_{833}}%
\htconstrdef{Gamma106.c}{\BR_{106}}{\BR_{30} + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{47} + \BR_{53}\cdot{}\BR_{<K^0|K_S>} + \BR_{77} + \BR_{103} + \BR_{126}\cdot{}(\BR_{\eta\to3\pi^0}+\BR_{\eta\to\pi^+\pi^-\pi^0}) + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}{\BR_{30} + \BR_{44}\cdot{}\BR_{<\bar{K}^0|K_S>} + \BR_{47} + \BR_{53}\cdot{}\BR_{<K^0|K_S>}  \\ 
  {}& + \BR_{77} + \BR_{103} + \BR_{126}\cdot{}(\BR_{\eta\to3\pi^0}+\BR_{\eta\to\pi^+\pi^-\pi^0}) + \BR_{152}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma110.c}{\BR_{110}}{\BR_{10} + \BR_{16} + \BR_{23} + \BR_{28} + \BR_{35} + \BR_{40} + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{151} + \BR_{130} + \BR_{132} + \BR_{44} + \BR_{53} + \BR_{168} + \BR_{169} + \BR_{822} + \BR_{833}}{\BR_{10} + \BR_{16} + \BR_{23} + \BR_{28} + \BR_{35} + \BR_{40}  \\ 
  {}& + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{151} + \BR_{130} + \BR_{132}  \\ 
  {}& + \BR_{44} + \BR_{53} + \BR_{168} + \BR_{169} + \BR_{822} + \BR_{833}}%
\htconstrdef{Gamma149.c}{\BR_{149}}{\BR_{152} + \BR_{800} + \BR_{151}}{\BR_{152} + \BR_{800} + \BR_{151}}%
\htconstrdef{Gamma150.c}{\BR_{150}}{\BR_{800} + \BR_{151}}{\BR_{800} + \BR_{151}}%
\htconstrdef{Gamma150by66.c}{\frac{\BR_{150}}{\BR_{66}}}{\frac{\BR_{150}}{\BR_{66}}}{\frac{\BR_{150}}{\BR_{66}}}%
\htconstrdef{Gamma152by54.c}{\frac{\BR_{152}}{\BR_{54}}}{\frac{\BR_{152}}{\BR_{54}}}{\frac{\BR_{152}}{\BR_{54}}}%
\htconstrdef{Gamma152by76.c}{\frac{\BR_{152}}{\BR_{76}}}{\frac{\BR_{152}}{\BR_{76}}}{\frac{\BR_{152}}{\BR_{76}}}%
\htconstrdef{Gamma168.c}{\BR_{168}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}{\BR_{167}\cdot{}\BR_{\phi\to K^+K^-}}%
\htconstrdef{Gamma169.c}{\BR_{169}}{\BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}{\BR_{167}\cdot{}\BR_{\phi\to K_S K_L}}%
\htconstrdef{Gamma804.c}{\BR_{804}}{\BR_{47} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}{\BR_{47} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}%
\htconstrdef{Gamma806.c}{\BR_{806}}{\BR_{50} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}{\BR_{50} \cdot{} ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))}%
\htconstrdef{Gamma809.c}{\BR_{809}}{\BR_{30}}{\BR_{30}}%
\htconstrdef{Gamma810.c}{\BR_{810}}{\BR_{910} + \BR_{911} + \BR_{811}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{812}}{\BR_{910} + \BR_{911} + \BR_{811}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{812}}%
\htconstrdef{Gamma820.c}{\BR_{820}}{\BR_{920} + \BR_{821}}{\BR_{920} + \BR_{821}}%
\htconstrdef{Gamma830.c}{\BR_{830}}{\BR_{930} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{832}}{\BR_{930} + \BR_{831}\cdot{}\BR_{\omega\to\pi^+\pi^-\pi^0} + \BR_{832}}%
\htconstrdef{Gamma910.c}{\BR_{910}}{\BR_{136}\cdot{}\BR_{\eta\to3\pi^0}}{\BR_{136}\cdot{}\BR_{\eta\to3\pi^0}}%
\htconstrdef{Gamma911.c}{\BR_{911}}{\BR_{945}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{945}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma930.c}{\BR_{930}}{\BR_{136}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}{\BR_{136}\cdot{}\BR_{\eta\to\pi^+\pi^-\pi^0}}%
\htconstrdef{Gamma944.c}{\BR_{944}}{\BR_{136}\cdot{}\BR_{\eta\to\gamma\gamma}}{\BR_{136}\cdot{}\BR_{\eta\to\gamma\gamma}}%
\htconstrdef{GammaAll.c}{\BR_{\text{All}}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16} + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35} + \BR_{37} + \BR_{40} + \BR_{42} + \BR_{47}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) + \BR_{48} + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{811} + \BR_{812} + \BR_{93} + \BR_{94} + \BR_{832} + \BR_{833} + \BR_{126} + \BR_{128} + \BR_{802} + \BR_{803} + \BR_{800} + \BR_{151} + \BR_{130} + \BR_{132} + \BR_{44} + \BR_{53} + \BR_{50}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>}))) + \BR_{51} + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-}+\BR_{\phi\to K_S K_L}) + \BR_{152} + \BR_{920} + \BR_{821} + \BR_{822} + \BR_{831} + \BR_{136} + \BR_{945} + \BR_{805}}{\BR_{3} + \BR_{5} + \BR_{9} + \BR_{10} + \BR_{14} + \BR_{16}  \\ 
  {}& + \BR_{20} + \BR_{23} + \BR_{27} + \BR_{28} + \BR_{30} + \BR_{35}  \\ 
  {}& + \BR_{37} + \BR_{40} + \BR_{42} + \BR_{47}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>})))  \\ 
  {}& + \BR_{48} + \BR_{62} + \BR_{70} + \BR_{77} + \BR_{811} + \BR_{812}  \\ 
  {}& + \BR_{93} + \BR_{94} + \BR_{832} + \BR_{833} + \BR_{126} + \BR_{128}  \\ 
  {}& + \BR_{802} + \BR_{803} + \BR_{800} + \BR_{151} + \BR_{130} + \BR_{132}  \\ 
  {}& + \BR_{44} + \BR_{53} + \BR_{50}\cdot{}(1 + ((\BR_{<K^0|K_L>}\cdot{}\BR_{<\bar{K}^0|K_L>}) / (\BR_{<K^0|K_S>}\cdot{}\BR_{<\bar{K}^0|K_S>})))  \\ 
  {}& + \BR_{51} + \BR_{167}\cdot{}(\BR_{\phi\to K^+K^-}+\BR_{\phi\to K_S K_L}) + \BR_{152} + \BR_{920}  \\ 
  {}& + \BR_{821} + \BR_{822} + \BR_{831} + \BR_{136} + \BR_{945} + \BR_{805}}%
\htconstrdef{Unitarity}{1}{\BR_{\text{All}} + \BR_{998}}{\BR_{\text{All}} + \BR_{998}}%
\htdef{ConstrEqs}{%
\begin{align*}
\htuse{Gamma1.c.left} ={}& \htuse{Gamma1.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma2.c.left} ={}& \htuse{Gamma2.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma3by5.c.left} ={}& \htuse{Gamma3by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma7.c.left} ={}& \htuse{Gamma7.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma8.c.left} ={}& \htuse{Gamma8.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma8by5.c.left} ={}& \htuse{Gamma8by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma9by5.c.left} ={}& \htuse{Gamma9by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma10by5.c.left} ={}& \htuse{Gamma10by5.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma10by9.c.left} ={}& \htuse{Gamma10by9.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma11.c.left} ={}& \htuse{Gamma11.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma12.c.left} ={}& \htuse{Gamma12.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma13.c.left} ={}& \htuse{Gamma13.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma17.c.left} ={}& \htuse{Gamma17.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma18.c.left} ={}& \htuse{Gamma18.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma19.c.left} ={}& \htuse{Gamma19.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma19by13.c.left} ={}& \htuse{Gamma19by13.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma24.c.left} ={}& \htuse{Gamma24.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma25.c.left} ={}& \htuse{Gamma25.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma26.c.left} ={}& \htuse{Gamma26.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma26by13.c.left} ={}& \htuse{Gamma26by13.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma29.c.left} ={}& \htuse{Gamma29.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma31.c.left} ={}& \htuse{Gamma31.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma32.c.left} ={}& \htuse{Gamma32.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma33.c.left} ={}& \htuse{Gamma33.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma34.c.left} ={}& \htuse{Gamma34.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma38.c.left} ={}& \htuse{Gamma38.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma39.c.left} ={}& \htuse{Gamma39.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma43.c.left} ={}& \htuse{Gamma43.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma46.c.left} ={}& \htuse{Gamma46.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma49.c.left} ={}& \htuse{Gamma49.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma54.c.left} ={}& \htuse{Gamma54.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma55.c.left} ={}& \htuse{Gamma55.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma56.c.left} ={}& \htuse{Gamma56.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma57.c.left} ={}& \htuse{Gamma57.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma57by55.c.left} ={}& \htuse{Gamma57by55.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma58.c.left} ={}& \htuse{Gamma58.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma59.c.left} ={}& \htuse{Gamma59.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma60.c.left} ={}& \htuse{Gamma60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma63.c.left} ={}& \htuse{Gamma63.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma64.c.left} ={}& \htuse{Gamma64.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma65.c.left} ={}& \htuse{Gamma65.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma66.c.left} ={}& \htuse{Gamma66.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma67.c.left} ={}& \htuse{Gamma67.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma68.c.left} ={}& \htuse{Gamma68.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma69.c.left} ={}& \htuse{Gamma69.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma74.c.left} ={}& \htuse{Gamma74.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma75.c.left} ={}& \htuse{Gamma75.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma76.c.left} ={}& \htuse{Gamma76.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma76by54.c.left} ={}& \htuse{Gamma76by54.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma78.c.left} ={}& \htuse{Gamma78.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma79.c.left} ={}& \htuse{Gamma79.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma80.c.left} ={}& \htuse{Gamma80.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma80by60.c.left} ={}& \htuse{Gamma80by60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma81.c.left} ={}& \htuse{Gamma81.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma81by69.c.left} ={}& \htuse{Gamma81by69.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma82.c.left} ={}& \htuse{Gamma82.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma83.c.left} ={}& \htuse{Gamma83.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma84.c.left} ={}& \htuse{Gamma84.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma85.c.left} ={}& \htuse{Gamma85.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma85by60.c.left} ={}& \htuse{Gamma85by60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma87.c.left} ={}& \htuse{Gamma87.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma88.c.left} ={}& \htuse{Gamma88.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma89.c.left} ={}& \htuse{Gamma89.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma92.c.left} ={}& \htuse{Gamma92.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma93by60.c.left} ={}& \htuse{Gamma93by60.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma94by69.c.left} ={}& \htuse{Gamma94by69.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma96.c.left} ={}& \htuse{Gamma96.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma102.c.left} ={}& \htuse{Gamma102.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma103.c.left} ={}& \htuse{Gamma103.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma104.c.left} ={}& \htuse{Gamma104.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma106.c.left} ={}& \htuse{Gamma106.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma110.c.left} ={}& \htuse{Gamma110.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma149.c.left} ={}& \htuse{Gamma149.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma150.c.left} ={}& \htuse{Gamma150.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma150by66.c.left} ={}& \htuse{Gamma150by66.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma152by54.c.left} ={}& \htuse{Gamma152by54.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma152by76.c.left} ={}& \htuse{Gamma152by76.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma168.c.left} ={}& \htuse{Gamma168.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma169.c.left} ={}& \htuse{Gamma169.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma804.c.left} ={}& \htuse{Gamma804.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma806.c.left} ={}& \htuse{Gamma806.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma809.c.left} ={}& \htuse{Gamma809.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma810.c.left} ={}& \htuse{Gamma810.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma820.c.left} ={}& \htuse{Gamma820.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma830.c.left} ={}& \htuse{Gamma830.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma910.c.left} ={}& \htuse{Gamma910.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma911.c.left} ={}& \htuse{Gamma911.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma930.c.left} ={}& \htuse{Gamma930.c.right.split}
\end{align*}
\begin{align*}
\htuse{Gamma944.c.left} ={}& \htuse{Gamma944.c.right.split}
\end{align*}
\begin{align*}
\htuse{GammaAll.c.left} ={}& \htuse{GammaAll.c.right.split}
\end{align*}}%
\htdef{NumMeasALEPH}{39}%
\htdef{NumMeasARGUS}{2}%
\htdef{NumMeasBaBar}{29}%
\htdef{NumMeasBelle}{15}%
\htdef{NumMeasCELLO}{1}%
\htdef{NumMeasCLEO}{35}%
\htdef{NumMeasCLEO3}{6}%
\htdef{NumMeasDELPHI}{14}%
\htdef{NumMeasHRS}{2}%
\htdef{NumMeasL3}{11}%
\htdef{NumMeasOPAL}{19}%
\htdef{NumMeasTPC}{3}%


==> tau/tau-br-fit-meas-byref.tex <==
%
%
\subsection{Branching fractions fit measurement list by reference}
\cutname{br-fit-meas-byref.html}

Table~\ref{tab:tau:measPerPaper} reports the measurements used for the
\hfagtau branching fraction fit grouped by their bibliographic reference.

%
%
%
\begin{center}
\begin{envsmall}
\renewcommand*{\arraystretch}{1.3}%
\ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
\begin{longtable}{ll}
\caption{By-reference measurements list.\label{tab:tau:measPerPaper}}%
\\
\hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endfirsthead
\multicolumn{2}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \hline
\multicolumn{1}{l}{\bfseries Reference / Branching Fraction} & \multicolumn{1}{l}{\bfseries Value} \\
\hline
\endhead
\htuse{MeasPaper} \\
\hline
\end{longtable}
\end{envsmall}
\end{center}


==> tau/tau-defs.tex <==
\newcommand{\BRF}[2]{#2}
%
%
%
%

%
\newcommand{\lepth}{\lambda}
\newcommand{\leptl}{\rho}

%
\newcommand{\radRatio}{R}
%
\newcommand{\radDelta}{\delta R}

%
\newcommand{\Rhad}{\ensuremath{R_{\text{had}}}\xspace}
\newcommand{\BRhad}{\ensuremath{\BR_{\text{had}}}\xspace}
\newcommand{\Gammahad}{\ensuremath{\Gamma_{\text{had}}}\xspace}
%
\newcommand{\Rstrange}{\ensuremath{R_s}\xspace}
\newcommand{\BRstrange}{\ensuremath{\BR_s}\xspace}
\newcommand{\Gammastrange}{\ensuremath{\Gamma_s}\xspace}
\newcommand{\Rnonstrange}{\ensuremath{R_{\text{VA}}}\xspace}
\newcommand{\BRnonstrange}{\ensuremath{\BR_{\text{VA}}}\xspace}
\newcommand{\Gammanonstrange}{\ensuremath{\Gamma_{\text{VA}}}\xspace}
\newcommand{\tauknu}{\ensuremath{\tau^{-} \to K^{-} \nut}\xspace}
\newcommand{\taupinu}{\ensuremath{\tau^{-} \to \pi^{-} \nut}\xspace}
\newcommand{\BFtautoknu}{\ensuremath{\BR(\tauknu)}\xspace}
\newcommand{\BFtautopinu}{\ensuremath{\BR(\taupinu)}\xspace}
\newcommand{\VusUni}{\ensuremath{\Vus_{\text{uni}}}\xspace}
\newcommand{\VusTauIncl}{\ensuremath{\Vus_{\tau s}}\xspace}
\newcommand{\VusTauKpi}{\ensuremath{\Vus_{\tau K/\pi}}\xspace}
\newcommand{\VusTauKnu}{\ensuremath{\Vus_{\tau K}}\xspace}
\newcommand{\VusTauKPinu}{\ensuremath{\Vus_{\tau K\pi}}\xspace}
%
\newcommand{\hfagtau}{HFLAV-Tau\xspace}
%
\newcommand{\dRradTauhHmu}{\ensuremath{\radDelta_{\tau/h}}\xspace}
\newcommand{\dRradTaupiPimu}{\ensuremath{\radDelta_{\tau/\pi}}\xspace}
\newcommand{\dRradTaukKmu}{\ensuremath{\radDelta_{\tau/K}}\xspace}
\newcommand{\RradKmuPimu}{\ensuremath{\radRatio_{K/\pi}}\xspace}
%
\providecommand{\slashLikeH}{%
  \raisebox{.9ex}{%
    \scalebox{.7}{%
      \rotatebox[origin=c]{18}{$-$}%
    }%
  }%
}
\providecommand{\hslash}{%
  {%
   \vphantom{h}%
   \ooalign{\kern.05em\smash{\slashLikeH}\hidewidth\cr$h$\cr}%
   \kern.05em
  }%
}


==> tau/tau-header.tex <==
%
%
%
%
\newcommand{\hfagTauTag}{2018\xspace}
\newcommand{\hfagFitLabel}{HFLAV \hfagTauTag fit}

%
%
%
%
\newif\ifhevea\heveafalse
%

%
\makeatletter
\newenvironment*{fleqn}[1][\leftmargini minus\leftmargini]{\@fleqntrue
  \setlength\@mathmargin{#1}\ignorespaces
}{%
  \ignorespacesafterend
}
\makeatother

\ifhevea
\renewcommand{\babar}{BaBar\xspace}
\else
\makeatletter
\providecommand{\cutname}[1]{}

%
\newenvironment{envsmall}%
  {\small}%
  {}

%
\newenvironment{ceqn}{\@fleqnfalse
  \@mathmargin\@centering \ignorespaces
}{%
  \ignorespacesafterend
}

%
\newenvironment{citenoleadsp}{\@fleqnfalse
  \let\cite@adjust\@empty
}{%
  \ignorespacesafterend
}

%
\newenvironment{ensuredisplaymath}
  {\(\displaystyle}
  {\)}
\makeatother
\fi

%
%
%
\makeatletter

%
\newcommand{\htdef}[2]{%
  \@namedef{hfagtau@#1}{#2}%
}

%
\ifhevea
\newcommand{\htuse}[1]{%
  \@nameuse{hfagtau@#1}}%
\else
\newcommand{\htuse}[1]{%
  \ifcsname hfagtau@#1\endcsname
  \@nameuse{hfagtau@#1}%
  \else
  \@latex@error{Undefined name hfagtau@#1}\@eha
  \fi}
\fi

%
\ifhevea
\newcommand{\htquantdef}[6]{%
  \@namedef{hfagtau@#1.gn}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1.td}{\ensuremath{#3}}%
  \@namedef{hfagtau@#1}{\ensuremath{#4}}%
  \@namedef{hfagtau@#1.v}{\ensuremath{#5}}%
  \@namedef{hfagtau@#1.e}{\ensuremath{#6}}%
}
\else
\newcommand{\htquantdef}[6]{%
  \ifx&#2&\else
  \@namedef{hfagtau@#1.gn}{\ensuremath{#2}}%
  \fi
  \ifx&#3&\else
  \@namedef{hfagtau@#1.td}{\ensuremath{#3}}%
  \fi
  \ifx&#6&%
    \@namedef{hfagtau@#1}{\ensuremath{#5}}%
  \else
    \ifthenelse{\equal{#6}{0}}{%
      \@namedef{hfagtau@#1}{\ensuremath{#5}}%
    }{%
      \@namedef{hfagtau@#1}{\ensuremath{#4}}%
      \@namedef{hfagtau@#1.v}{\ensuremath{#5}}%
      \@namedef{hfagtau@#1.e}{\ensuremath{#6}}%
    }%
  \fi
}
\fi

%
\newcommand{\htmeasdef}[8]{%
  \@namedef{hfagtau@#1,quant}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1,exp}{#3}%
  \@namedef{hfagtau@#1,ref}{\cite{#4}}%
  \@namedef{hfagtau@#1}{\ensuremath{#5}}%
  \@namedef{hfagtau@#1,val}{\ensuremath{#6}}%
  \@namedef{hfagtau@#1,stat}{\ensuremath{#7}}%
  \@namedef{hfagtau@#1,syst}{\ensuremath{#8}}%
}

%
\newcommand{\htconstrdef}[4]{%
  \@namedef{hfagtau@#1.left}{\ensuremath{#2}}%
  \@namedef{hfagtau@#1.right}{\ensuremath{#3}}%
  \@namedef{hfagtau@#1.right.split}{\ensuremath{#4}}%
  \@namedef{hfagtau@#1.constr.eq}{\htuse{#1.left} ={}& \htuse{#1.right}}%
}

\newcommand{\htQuantLine}[3]{\ensuremath{\htuse{#1.td}}&\ensuremath{#2}\\}

\makeatother

\ifhevea
\input{tau-defs}
\input{hflav-2018}
\input{hflav-2018-elab-vadirect}
\input{tau-lfv-data}
\else
\input{tau/tau-defs}
\input{tau/hflav-2018}
\input{tau/hflav-2018-elab-vadirect}
\input{tau/tau-lfv-data}
\fi


==> tau/tau-lfv-combs-plot.tex <==
%
%
\ifhevea
\subsection{Combination of upper limits on \mtau lepton-flavour-violating branching fractions: summary plot}
\cutname{lfv-combinations-plot.html}
\fi

\begin{figure}[tb]
  \begin{center}
    \ifhevea
    \begin{tabular}{@{}cc@{}}
      \larger\bfseries\ahref{tau-lfv-combs.png}{full size PNG} &
      \larger\bfseries\ahref{tau-lfv-combs.pdf}{PDF format} \\
      \multicolumn{2}{c}{\ahref{tau-lfv-combs.png}{%
          \imgsrc[alt="Tau LFV limits combinations plot" width=720]{tau-lfv-combs.png}}}
    \end{tabular}
    \else
    \includegraphics[angle=90,totalheight=0.82\textheight,clip]{figures/tau/tau-lfv-combs.pdf}
    \fi
    \caption{Tau lepton-flavour-violating branching fraction upper limits
      combinations summary plot. For each channel we report the HFLAV
      combined limit, and the experimental published limits. In some cases,
      the combined limit is weaker than the limit published by a single
      experiment. This arises since the \cls method used in the
      combination can be more conservative compared to other legitimate
      methods, especially when the number of observed events fluctuates below the
      expected background. 
      \label{fig:tau:lfv-limits-plot-average}
    }
  \end{center}
\end{figure}


==> tau/tau-lfv-combs.tex <==
%
\subsection{\texorpdfstring{%
  Combination of upper limits on \mtau lepton-flavour-violating branching fractions}{%
  Combination of upper limits on tau lepton-flavour-violating branching fractions}}
\label{sec:tau:lfv-limits}
%
%
\cutname{lfv-combinations.html}
%
\newcommand{\cls}{\ensuremath{\text{CL}_s}\xspace}
\newcommand{\clsb}{\ensuremath{\text{CL}_{s+b}}\xspace}
\newcommand{\clb}{\ensuremath{\text{CL}_b}\xspace}
%
%
%
\newcommand{\htLimitLine}[5]{%
  #1 & #2 & #3 & #4 & #5 \\
}
\newcommand{\htCombLimitLine}[4]{%
  #1 & #2 & #3 & #4 \\
}
\newcommand{\htCombExtraLine}[7]{%
  #1 & #2 & \cite{#3} & #4 & #5 & #6 & #7 \\
}
%
The Standard Model predicts that the \mtau lepton-flavour-violating
(LFV) branching fractions are
too small to be measured with the available experimental precision.
We report in Table~\ref{tab:tau:lfv-limits-and-combs} and
Figure~\ref{fig:tau:lfv-limits-plot} the experimental upper
limits on these branching fractions that have been published by the
$B$-factories \babar and Belle and later experiments. We omit 
previous weaker upper limits (mainly from CLEO) and all preliminary
results older than a few years. Presently, no preliminary result is included.

\iffalse
\begin{center}

\begin{longtable}{lcclc}
\caption{Experimental upper limits on lepton flavour violating \mtau
  decays. The modes are grouped according to the properties of their final
  states. Modes with baryon number violation are labelled with ``BNV''.
  \label{tab:tau:lfv-limits}}%
\\
\toprule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{l}{\bfseries Category} &
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{c}{\bfseries Reference} \\
\midrule
\endfirsthead
\multicolumn{5}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{l}{\bfseries Category} &
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{c}{\bfseries Reference} \\
\midrule
\endhead
%
\htuse{LimitLines}
%
\bottomrule
\end{longtable}
\end{center}
\fi

Combining upper limits is a delicate issue, since there is no standard and
generally agreed procedure. Furthermore, the \mtau LFV searches
published limits are extracted from the data with a variety of
methods, and cannot be directly combined with a uniform procedure. It
is however possible to use a single and effective
upper limit combination procedure for all modes by re-computing the published upper
limits with just one extraction method, using the published
information that documents the upper limit determination:
number of observed candidates, expected background, signal efficiency and
number of analyzed \mtau decays.

We chose to use the \cls method~\cite{Read:2002hq} to re-compute the
\mtau LFV upper limits, since it is well known and widely used (see the
Statistics review of PDG 2018~\cite{PDG_2018}), and since the
limits computed with the \cls method can be combined in a straightforward
way (see below). The \cls method is based on two hypotheses: signal plus background and
background only. We calculate the observed confidence levels for the two
hypotheses:
\begin{align}
&\clsb = P_{s+b}(Q \leq Q_{obs}) = \int_{- \infty}^{Q_{obs}} \frac{dP_{s+b}}{dQ} dQ,
\label{eq:tau:clspdf1} \\
&\clb = P_{b}(Q \leq Q_{obs}) = \int_{- \infty}^{Q_{obs}} \frac{dP_{b}}{dQ} dQ,
\label{eq:tau:clspdf2}
\end{align}
where \clsb is the confidence level observed for the signal plus background
hypotheses, \clb is the confidence level observed for the background only
hypothesis, $\frac{dP_{s+b}}{dQ}$ and $\frac{dP_{b}}{dQ}$ are the probability
distribution functions (PDFs) for the two corresponding hypothesis and
$Q$ is called the test statistic. The \cls value is defined as the ratio
between the confidence level for the signal plus background hypothesis and
the confidence level for the background hypothesis:
\begin{align}
\cls = \dfrac{\clsb}{\clb}.
\end{align}
When multiple results are combined, the PDFs in
Eqs.~(\ref{eq:tau:clspdf1}) and~(\ref{eq:tau:clspdf2}) are the
product of the individual PDFs,
\begin{align}
\cls = \dfrac{\prod_{i=1}^{N}\sum_{n=0}^{n_i} \dfrac{e^{-(s_i+b_i)} (s_i+b_i)^{n}}{n!} }{\prod_{i=1}^{N}  \sum_{n=0}^{n_i} \dfrac{e^{-b_i} b_i^{n}}{n!}}    \dfrac{\prod_{j=1}^{N} \left[s_iS_i(x_{ij})+b_iB_i(x_{ij})\right]}{\prod_{j=1}^{N}B_i(x_{ij})}~,
\end{align}
where $N$ is the number of results (or channels), and, for each channel $i$,
$n_i$ is the number of observed candidates, $x_{ij}$ are the values of the
discriminating variables (with index $j$), $s_i$ and $b_i$ are the number
of signal and background events and $S_i$, $B_i$ are the probability
distribution functions of the discriminating variables. The
discriminating variables $x_{ij}$ are assumed to be uncorrelated.
The expected signal $s_i$ is related to the \mtau lepton branching
fraction $\BR(\tau \rightarrow f_i)$ into
the searched final state $f_i$ by $s_i = N_i\epsilon_i\BR(\tau \rightarrow
f_i)$, where $N_i$ is the number of produced \mtau leptons and
$\epsilon_i$ is the detection efficiency for observing the decay $\tau\to
f_i$. For $e^+ e^-$ experiments,
$N_i = 2\mathcal{L}_i\sigma_{\tau\tau}$, where $\mathcal{L}_i$ is the
integrated luminosity and $\sigma_{\tau\tau}$ is the
\mtau pair production cross section $\sigma(e^+ e^- \rightarrow \tau^+
\tau^-)$~\cite{Banerjee:2007is}.
In experiments where \mtau leptons are produced in more complex multiple
reactions, the effective $N_i$ is typically estimated with Monte Carlo simulations
calibrated with related data yields.

The extraction of the upper limits is performed using the code provided by
Tom Junk~\cite{junk:2007:cdfnote}. The systematic uncertainties are modeled
in the Monte Carlo toy experiments by convolving the $S_i$ and $B_i$
PDFs with Gaussian distributions corresponding to the nuisance
parameters.

Table~\ref{tab:tau:lfv-limits-and-combs} reports the HFLAV combinations of the
\mtau LFV limits. Since there is negligible gain in combining limits of very
different strength, the combinations do not include the CLEO searches
and do not include results where the single event sensitivity is more
than a factor of 5 lower than the value for the search with the best limit.

Figure~\ref{fig:tau:lfv-limits-plot-average} reports a graphical
representation of the $\mtau$ LFV limits combinations listed in
Table~\ref{tab:tau:lfv-limits-and-combs}.  The published information
that has been used to obtain these limits is reported in
Table~\ref{tab:tau:lfv-extra-info-comb}. In the previous HFLAV reports,
the determination of combined limit {\ensuremath{\BR_{183} = \mu^-
    \mu^+ \mu^-}} erroneously counted twice the systematic uncertainty
of the LHCb limit. That has been fixed now, and the combination of the
upper limits on $\BR_{183} = \htuse{g183.descr}$ 
has changed from $< 1.2 \cdot 10^{-8}$ to $< 1.1 \cdot 10^{-8}$.

\iffalse
\begin{center}
\begin{longtable}{lcrc}
\caption{Combinations of upper limits on lepton flavour violating \mtau decay
  modes. The modes are grouped according to the properties of their final
  states. Modes with baryon number violation are labelled with ``BNV''.
\label{tab:tau:lfv-combs}}%
\\
\toprule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{c}{\bfseries Category} &
\multicolumn{1}{r}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}} &
\multicolumn{1}{c}{\bfseries Refs.} \\
\midrule
\endfirsthead
\multicolumn{3}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\midrule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{c}{\bfseries Category} &
\multicolumn{1}{r}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}} &
\multicolumn{1}{c}{\bfseries Refs.} \\
\midrule
\endhead
\htuse{CombLines}
\bottomrule
\end{longtable}
\end{center}
\fi

\begin{center}
\begin{longtable}{lcclc}
\caption{Experimental upper limits on lepton flavour violating \mtau
  decays. The modes are grouped according to the properties of their final
  states. Modes with baryon number violation are labelled with ``BNV''.
  The experiment ``HFLAV'' denotes the combinations of upper limits
  computed by HFLAV. The references associated with the combination
  list what upper limits have been used.
  \label{tab:tau:lfv-limits-and-combs}}%
\\
\toprule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{l}{\bfseries Category} &
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{c}{\bfseries References} \\
\midrule
\endfirsthead
\multicolumn{5}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{l}{\bfseries Category} &
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}90\% CL\\Limit\end{tabular}} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{c}{\bfseries References} \\
\midrule
\endhead
%
\htuse{LimitCombLines}
%
\bottomrule
\end{longtable}
\end{center}

\begin{center}\smaller
\begin{longtable}{llcrrrrrr}
\caption{
  %
  Published information that has been used to re-compute upper limits
  with the \cls method, \ie\ the number of \mtau leptons produced, the
  signal detection efficiency and its uncertainty, the number of
  expected background events and its uncertainty,
  and the number of observed events. The uncertainty on the efficiency
  includes the minor uncertainty contribution on the number of \mtau leptons
  (typically originating on the uncertainties on the integrated
  luminosity and on the production cross-section).
  The additional limit used in the
  combinations (from \lhcb) has been originally determined with the \cls
  method.
\label{tab:tau:lfv-extra-info-comb}}%
\\
\toprule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{c}{\bfseries Exp.} &
\multicolumn{1}{c}{\bfseries Ref.} &
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}$N_{\tau}$\\(millions)\end{tabular}} &
%
%
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}efficiency\\(\%)\end{tabular}} &
\multicolumn{1}{c}{\bfseries $N_{\text{bkg}}$} &
\multicolumn{1}{c}{\bfseries $N_{\text{obs}}$} \\
\midrule
\endfirsthead
\multicolumn{5}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\midrule
\multicolumn{1}{l}{\bfseries Decay mode} &
\multicolumn{1}{c}{\bfseries Exp.} &
\multicolumn{1}{c}{\bfseries Ref.} &
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}$N_{\tau}$\\(millions)\end{tabular}} &
%
%
\multicolumn{1}{c}{\bfseries \begin{tabular}{@{}c@{}}efficiency\\(\%)\end{tabular}} &
\multicolumn{1}{c}{\bfseries $N_{\text{bkg}}$} &
\multicolumn{1}{c}{\bfseries $N_{\text{obs}}$} \\
\midrule
\endhead
\htuse{CombExtraLines}
\bottomrule
\end{longtable}
\end{center}


==> tau/tau-lfv-data.tex <==
\htdef{g156.descr}{\ensuremath{e^- \gamma}}%
\htdef{g157.descr}{\ensuremath{\mu^- \gamma}}%
\htdef{g158.descr}{\ensuremath{e^- \pi^0}}%
\htdef{g159.descr}{\ensuremath{\mu^- \pi^0}}%
\htdef{g160.descr}{\ensuremath{e^- K^0_S}}%
\htdef{g161.descr}{\ensuremath{\mu^- K^0_S}}%
\htdef{g162.descr}{\ensuremath{e^- \eta}}%
\htdef{g163.descr}{\ensuremath{\mu^- \eta}}%
\htdef{g172.descr}{\ensuremath{e^- \eta^\prime(958)}}%
\htdef{g173.descr}{\ensuremath{\mu^- \eta^\prime(958)}}%
\htdef{g164.descr}{\ensuremath{e^- \rho^0}}%
\htdef{g165.descr}{\ensuremath{\mu^- \rho^0}}%
\htdef{g166.descr}{\ensuremath{e^- \omega}}%
\htdef{g167.descr}{\ensuremath{\mu^- \omega}}%
\htdef{g168.descr}{\ensuremath{e^- K^*(892)}}%
\htdef{g169.descr}{\ensuremath{\mu^- K^*(892)}}%
\htdef{g170.descr}{\ensuremath{e^- \bar{K}^*(892)}}%
\htdef{g171.descr}{\ensuremath{\mu^- \bar{K}^*(892)}}%
\htdef{g176.descr}{\ensuremath{e^- \phi}}%
\htdef{g177.descr}{\ensuremath{\mu^- \phi}}%
\htdef{g174.descr}{\ensuremath{e^- f_0(980)}}%
\htdef{g175.descr}{\ensuremath{\mu^- f_0(980)}}%
\htdef{g178.descr}{\ensuremath{e^- e^+ e^-}}%
\htdef{g179.descr}{\ensuremath{e^- \mu^+ \mu^-}}%
\htdef{g180.descr}{\ensuremath{\mu^- e^+ \mu^-}}%
\htdef{g181.descr}{\ensuremath{\mu^- e^+ e^-}}%
\htdef{g182.descr}{\ensuremath{e^- \mu^+ e^-}}%
\htdef{g183.descr}{\ensuremath{\mu^- \mu^+ \mu^-}}%
\htdef{g184.descr}{\ensuremath{e^- \pi^+ \pi^-}}%
\htdef{g185.descr}{\ensuremath{e^+ \pi^- \pi^-}}%
\htdef{g186.descr}{\ensuremath{\mu^- \pi^+  \pi^-}}%
\htdef{g187.descr}{\ensuremath{\mu^+ \pi^- \pi^-}}%
\htdef{g188.descr}{\ensuremath{e^- \pi^+ K^-}}%
\htdef{g189.descr}{\ensuremath{e^- K^+ \pi^-}}%
\htdef{g190.descr}{\ensuremath{e^+ \pi^- K^-}}%
\htdef{g191.descr}{\ensuremath{e^- K^0_S K^0_S}}%
\htdef{g192.descr}{\ensuremath{e^- K^+ K^-}}%
\htdef{g193.descr}{\ensuremath{e^+ K^- K^-}}%
\htdef{g194.descr}{\ensuremath{\mu^- \pi^+  K^-}}%
\htdef{g195.descr}{\ensuremath{\mu^- K^+  \pi^-}}%
\htdef{g196.descr}{\ensuremath{\mu^+ \pi^- K^-}}%
\htdef{g197.descr}{\ensuremath{\mu^- K^0_S  K^0_S}}%
\htdef{g198.descr}{\ensuremath{\mu^- K^+  K^-}}%
\htdef{g199.descr}{\ensuremath{\mu^+ K^- K^-}}%
\htdef{g211.descr}{\ensuremath{\pi^- \Lambda}}%
\htdef{g212.descr}{\ensuremath{\pi^- \bar{\Lambda}}}%
\htdef{g213.descr}{\ensuremath{K^- \Lambda}}%
\htdef{g214.descr}{\ensuremath{K^- \bar{\Lambda}}}%
\htdef{g215.descr}{\ensuremath{p \mu^- \mu^-}}%
\htdef{g216.descr}{\ensuremath{\bar{p} \mu^+ \mu^-}}%
\htdef{CombExtraLines}{%
\htCombExtraLine%
  {\ensuremath{\BR_{156} = e^- \gamma}}%
  {\babar}%
  {Aubert:2009ag}%
  {963}%
  {\ensuremath{3.90 \pm 0.30}}%
  {\ensuremath{1.60 \pm 0.40}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{156} = e^- \gamma}}%
  {\belle}%
  {Hayasaka:2007vc}%
  {983}%
  {\ensuremath{3.00 \pm 0.10}}%
  {\ensuremath{5.14 \pm 3.30}}%
  {5}%
\htCombExtraLine%
  {\ensuremath{\BR_{157} = \mu^- \gamma}}%
  {\babar}%
  {Aubert:2009ag}%
  {963}%
  {\ensuremath{6.10 \pm 0.50}}%
  {\ensuremath{3.60 \pm 0.70}}%
  {2}%
\htCombExtraLine%
  {\ensuremath{\BR_{157} = \mu^- \gamma}}%
  {\belle}%
  {Hayasaka:2007vc}%
  {983}%
  {\ensuremath{5.07 \pm 0.20}}%
  {\ensuremath{13.90 \pm 5.00}}%
  {10}%
\htCombExtraLine%
  {\ensuremath{\BR_{158} = e^- \pi^0}}%
  {\babar}%
  {Aubert:2006cz}%
  {339}%
  {\ensuremath{2.83 \pm 0.25}}%
  {\ensuremath{0.17 \pm 0.04}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{158} = e^- \pi^0}}%
  {\belle}%
  {Miyazaki:2007jp}%
  {401}%
  {\ensuremath{3.93 \pm 0.18}}%
  {\ensuremath{0.20 \pm 0.20}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{159} = \mu^- \pi^0}}%
  {\babar}%
  {Aubert:2006cz}%
  {339}%
  {\ensuremath{4.75 \pm 0.37}}%
  {\ensuremath{1.33 \pm 0.15}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{159} = \mu^- \pi^0}}%
  {\belle}%
  {Miyazaki:2007jp}%
  {401}%
  {\ensuremath{4.53 \pm 0.20}}%
  {\ensuremath{0.58 \pm 0.34}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{160} = e^- K^0_S}}%
  {\babar}%
  {Aubert:2009ys}%
  {862}%
  {\ensuremath{9.10 \pm 1.73}}%
  {\ensuremath{0.59 \pm 0.25}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{160} = e^- K^0_S}}%
  {\belle}%
  {Miyazaki:2010qb}%
  {1274}%
  {\ensuremath{10.20 \pm 0.67}}%
  {\ensuremath{0.18 \pm 0.18}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{161} = \mu^- K^0_S}}%
  {\babar}%
  {Aubert:2009ys}%
  {862}%
  {\ensuremath{6.14 \pm 0.20}}%
  {\ensuremath{0.30 \pm 0.18}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{161} = \mu^- K^0_S}}%
  {\belle}%
  {Miyazaki:2010qb}%
  {1274}%
  {\ensuremath{10.70 \pm 0.73}}%
  {\ensuremath{0.35 \pm 0.21}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{162} = e^- \eta}}%
  {\babar}%
  {Aubert:2006cz}%
  {339}%
  {\ensuremath{2.12 \pm 0.20}}%
  {\ensuremath{0.22 \pm 0.05}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{162} = e^- \eta}}%
  {\belle}%
  {Miyazaki:2007jp}%
  {401}%
  {\ensuremath{2.87 \pm 0.20}}%
  {\ensuremath{0.78 \pm 0.78}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{163} = \mu^- \eta}}%
  {\babar}%
  {Aubert:2006cz}%
  {339}%
  {\ensuremath{3.59 \pm 0.41}}%
  {\ensuremath{0.75 \pm 0.08}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{163} = \mu^- \eta}}%
  {\belle}%
  {Miyazaki:2007jp}%
  {401}%
  {\ensuremath{4.08 \pm 0.28}}%
  {\ensuremath{0.64 \pm 0.04}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{172} = e^- \eta^\prime(958)}}%
  {\babar}%
  {Aubert:2006cz}%
  {339}%
  {\ensuremath{1.53 \pm 0.16}}%
  {\ensuremath{0.12 \pm 0.03}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{172} = e^- \eta^\prime(958)}}%
  {\belle}%
  {Miyazaki:2007jp}%
  {401}%
  {\ensuremath{1.59 \pm 0.13}}%
  {\ensuremath{0.01 \pm 0.41}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{173} = \mu^- \eta^\prime(958)}}%
  {\babar}%
  {Aubert:2006cz}%
  {339}%
  {\ensuremath{2.18 \pm 0.26}}%
  {\ensuremath{0.49 \pm 0.26}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{173} = \mu^- \eta^\prime(958)}}%
  {\belle}%
  {Miyazaki:2007jp}%
  {401}%
  {\ensuremath{2.47 \pm 0.20}}%
  {\ensuremath{0.23 \pm 0.46}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{164} = e^- \rho^0}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{7.31 \pm 0.20}}%
  {\ensuremath{1.32 \pm 0.17}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{164} = e^- \rho^0}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{7.58 \pm 0.41}}%
  {\ensuremath{0.29 \pm 0.15}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{165} = \mu^- \rho^0}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{4.52 \pm 0.40}}%
  {\ensuremath{2.04 \pm 0.19}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{165} = \mu^- \rho^0}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{7.09 \pm 0.37}}%
  {\ensuremath{1.48 \pm 0.35}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{166} = e^- \omega}}%
  {\babar}%
  {Aubert:2007kx}%
  {829}%
  {\ensuremath{2.96 \pm 0.13}}%
  {\ensuremath{0.35 \pm 0.06}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{166} = e^- \omega}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{2.92 \pm 0.18}}%
  {\ensuremath{0.30 \pm 0.14}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{167} = \mu^- \omega}}%
  {\babar}%
  {Aubert:2007kx}%
  {829}%
  {\ensuremath{2.56 \pm 0.16}}%
  {\ensuremath{0.73 \pm 0.03}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{167} = \mu^- \omega}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{2.38 \pm 0.14}}%
  {\ensuremath{0.72 \pm 0.18}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{168} = e^- K^*(892)}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{8.00 \pm 0.20}}%
  {\ensuremath{1.65 \pm 0.23}}%
  {2}%
\htCombExtraLine%
  {\ensuremath{\BR_{168} = e^- K^*(892)}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{4.37 \pm 0.24}}%
  {\ensuremath{0.29 \pm 0.14}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{169} = \mu^- K^*(892)}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{4.60 \pm 0.40}}%
  {\ensuremath{1.79 \pm 0.21}}%
  {4}%
\htCombExtraLine%
  {\ensuremath{\BR_{169} = \mu^- K^*(892)}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{3.39 \pm 0.19}}%
  {\ensuremath{0.53 \pm 0.20}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{170} = e^- \bar{K}^*(892)}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{7.80 \pm 0.20}}%
  {\ensuremath{2.76 \pm 0.28}}%
  {2}%
\htCombExtraLine%
  {\ensuremath{\BR_{170} = e^- \bar{K}^*(892)}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{4.41 \pm 0.25}}%
  {\ensuremath{0.08 \pm 0.08}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{171} = \mu^- \bar{K}^*(892)}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{4.10 \pm 0.30}}%
  {\ensuremath{1.72 \pm 0.17}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{171} = \mu^- \bar{K}^*(892)}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{3.60 \pm 0.20}}%
  {\ensuremath{0.45 \pm 0.17}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{176} = e^- \phi}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{6.40 \pm 0.20}}%
  {\ensuremath{0.68 \pm 0.12}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{176} = e^- \phi}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{4.18 \pm 0.25}}%
  {\ensuremath{0.47 \pm 0.19}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{177} = \mu^- \phi}}%
  {\babar}%
  {Aubert:2009ap}%
  {829}%
  {\ensuremath{5.20 \pm 0.30}}%
  {\ensuremath{2.76 \pm 0.16}}%
  {6}%
\htCombExtraLine%
  {\ensuremath{\BR_{177} = \mu^- \phi}}%
  {\belle}%
  {Miyazaki:2011xe}%
  {1554}%
  {\ensuremath{3.21 \pm 0.19}}%
  {\ensuremath{0.06 \pm 0.06}}%
  {1}%
\htCombExtraLine%
  {\ensuremath{\BR_{178} = e^- e^+ e^-}}%
  {\babar}%
  {Lees:2010ez}%
  {868}%
  {\ensuremath{8.60 \pm 0.20}}%
  {\ensuremath{0.12 \pm 0.02}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{178} = e^- e^+ e^-}}%
  {\belle}%
  {Hayasaka:2010np}%
  {1437}%
  {\ensuremath{6.00 \pm 0.59}}%
  {\ensuremath{0.21 \pm 0.15}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{179} = e^- \mu^+ \mu^-}}%
  {\babar}%
  {Lees:2010ez}%
  {868}%
  {\ensuremath{6.40 \pm 0.40}}%
  {\ensuremath{0.54 \pm 0.14}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{179} = e^- \mu^+ \mu^-}}%
  {\belle}%
  {Hayasaka:2010np}%
  {1437}%
  {\ensuremath{6.10 \pm 0.58}}%
  {\ensuremath{0.10 \pm 0.04}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{180} = \mu^- e^+ \mu^-}}%
  {\babar}%
  {Lees:2010ez}%
  {868}%
  {\ensuremath{10.20 \pm 0.60}}%
  {\ensuremath{0.03 \pm 0.02}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{180} = \mu^- e^+ \mu^-}}%
  {\belle}%
  {Hayasaka:2010np}%
  {1437}%
  {\ensuremath{10.10 \pm 0.77}}%
  {\ensuremath{0.02 \pm 0.02}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{181} = \mu^- e^+ e^-}}%
  {\babar}%
  {Lees:2010ez}%
  {868}%
  {\ensuremath{8.80 \pm 0.50}}%
  {\ensuremath{0.64 \pm 0.19}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{181} = \mu^- e^+ e^-}}%
  {\belle}%
  {Hayasaka:2010np}%
  {1437}%
  {\ensuremath{9.30 \pm 0.73}}%
  {\ensuremath{0.04 \pm 0.04}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{182} = e^- \mu^+ e^-}}%
  {\babar}%
  {Lees:2010ez}%
  {868}%
  {\ensuremath{12.70 \pm 0.70}}%
  {\ensuremath{0.34 \pm 0.12}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{182} = e^- \mu^+ e^-}}%
  {\belle}%
  {Hayasaka:2010np}%
  {1437}%
  {\ensuremath{11.50 \pm 0.89}}%
  {\ensuremath{0.01 \pm 0.01}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{183} = \mu^- \mu^+ \mu^-}}%
  {\babar}%
  {Lees:2010ez}%
  {868}%
  {\ensuremath{6.60 \pm 0.60}}%
  {\ensuremath{0.44 \pm 0.17}}%
  {0}%
\htCombExtraLine%
  {\ensuremath{\BR_{183} = \mu^- \mu^+ \mu^-}}%
  {\belle}%
  {Hayasaka:2010np}%
  {1437}%
  {\ensuremath{7.60 \pm 0.56}}%
  {\ensuremath{0.13 \pm 0.20}}%
  {0}}%
\htdef{LimitLines}{%
\htLimitLine%
  {\ensuremath{\BR_{156} = e^- \gamma}}%
  {\ensuremath{\ell\gamma}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ag}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.2 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Hayasaka:2007vc}}%
\htLimitLine%
  {\ensuremath{\BR_{157} = \mu^- \gamma}}%
  {\ensuremath{}}%
  {\ensuremath{4.4 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ag}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2007vc}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{158} = e^- \pi^0}}%
  {\ensuremath{\ell P^0}}%
  {\ensuremath{1.3 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{\BR_{159} = \mu^- \pi^0}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.2 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{\BR_{160} = e^- K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ys}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{\BR_{161} = \mu^- K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{4.0 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ys}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.3 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{\BR_{162} = e^- \eta}}%
  {\ensuremath{}}%
  {\ensuremath{1.6 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{9.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{\BR_{163} = \mu^- \eta}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{6.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{\BR_{172} = e^- \eta^\prime(958)}}%
  {\ensuremath{}}%
  {\ensuremath{2.4 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.6 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{\BR_{173} = \mu^- \eta^\prime(958)}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.3 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{164} = e^- \rho^0}}%
  {\ensuremath{\ell V^0}}%
  {\ensuremath{4.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{165} = \mu^- \rho^0}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{166} = e^- \omega}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2007kx}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{167} = \mu^- \omega}}%
  {\ensuremath{}}%
  {\ensuremath{1.0 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2007kx}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{168} = e^- K^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{5.9 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{169} = \mu^- K^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{1.7 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{7.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{170} = e^- \bar{K}^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{4.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{171} = \mu^- \bar{K}^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{7.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{7.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{176} = e^- \phi}}%
  {\ensuremath{}}%
  {\ensuremath{3.1 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{\BR_{177} = \mu^- \phi}}%
  {\ensuremath{}}%
  {\ensuremath{1.9 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{174} = e^- f_0(980)}}%
  {\ensuremath{\ell S^0}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2008mw}}%
\htLimitLine%
  {\ensuremath{\BR_{175} = \mu^- f_0(980)}}%
  {\ensuremath{}}%
  {\ensuremath{3.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2008mw}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{178} = e^- e^+ e^-}}%
  {\ensuremath{\ell\ell\ell}}%
  {\ensuremath{2.9 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{\BR_{179} = e^- \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{\BR_{180} = \mu^- e^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{\BR_{181} = \mu^- e^+ e^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.2 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{\BR_{182} = e^- \mu^+ e^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{\BR_{183} = \mu^- \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.8 \cdot 10^{-7}}}%
  {ATLAS}%
  {\cite{Aad:2016wce}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.6 \cdot 10^{-8}}}%
  {LHCb}%
  {\cite{Aaij:2014azz}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{184} = e^- \pi^+ \pi^-}}%
  {\ensuremath{\ell hh}}%
  {\ensuremath{1.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.3 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{185} = e^+ \pi^- \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.7 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{186} = \mu^- \pi^+  \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.9 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{187} = \mu^+ \pi^- \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{7.0 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.9 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{188} = e^- \pi^+ K^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{189} = e^- K^+ \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.7 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{190} = e^+ \pi^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{191} = e^- K^0_S K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{7.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{\BR_{192} = e^- K^+ K^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{193} = e^+ K^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{194} = \mu^- \pi^+  K^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.6 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{195} = \mu^- K^+  \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{196} = \mu^+ \pi^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{197} = \mu^- K^0_S  K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{8.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{\BR_{198} = \mu^- K^+  K^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.5 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{199} = \mu^+ K^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{4.8 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{211} = \pi^- \Lambda}}%
  {\ensuremath{\text{BNV}}}%
  {\ensuremath{7.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2005ng}}%
\htLimitLine%
  {\ensuremath{\BR_{212} = \pi^- \bar{\Lambda}}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2005ng}}%
\htLimitLine%
  {\ensuremath{\BR_{215} = p \mu^- \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{4.4 \cdot 10^{-7}}}%
  {LHCb}%
  {\cite{Aaij:2013fia}}%
\htLimitLine%
  {\ensuremath{\BR_{216} = \bar{p} \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-7}}}%
  {LHCb}%
  {\cite{Aaij:2013fia}}}%
\htdef{CombLines}{%
\htCombLimitLine%
  {\ensuremath{\BR_{156} = e^- \gamma}}%
  {\ensuremath{\ell\gamma}}%
  {\ensuremath{5.4 \cdot 10^{-8}}}%
  {\cite{Hayasaka:2007vc,Aubert:2009ag}}%
\htCombLimitLine%
  {\ensuremath{\BR_{157} = \mu^- \gamma}}%
  {\ensuremath{}}%
  {\ensuremath{5.0 \cdot 10^{-8}}}%
  {\cite{Hayasaka:2007vc,Aubert:2009ag}}%
\midrule%
\htCombLimitLine%
  {\ensuremath{\BR_{158} = e^- \pi^0}}%
  {\ensuremath{\ell P^0}}%
  {\ensuremath{4.9 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htCombLimitLine%
  {\ensuremath{\BR_{159} = \mu^- \pi^0}}%
  {\ensuremath{}}%
  {\ensuremath{3.6 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htCombLimitLine%
  {\ensuremath{\BR_{160} = e^- K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2010qb,Aubert:2009ys}}%
\htCombLimitLine%
  {\ensuremath{\BR_{161} = \mu^- K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2010qb,Aubert:2009ys}}%
\htCombLimitLine%
  {\ensuremath{\BR_{162} = e^- \eta}}%
  {\ensuremath{}}%
  {\ensuremath{5.5 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htCombLimitLine%
  {\ensuremath{\BR_{163} = \mu^- \eta}}%
  {\ensuremath{}}%
  {\ensuremath{3.8 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htCombLimitLine%
  {\ensuremath{\BR_{172} = e^- \eta^\prime(958)}}%
  {\ensuremath{}}%
  {\ensuremath{9.9 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htCombLimitLine%
  {\ensuremath{\BR_{173} = \mu^- \eta^\prime(958)}}%
  {\ensuremath{}}%
  {\ensuremath{6.3 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\midrule%
\htCombLimitLine%
  {\ensuremath{\BR_{164} = e^- \rho^0}}%
  {\ensuremath{\ell V^0}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{165} = \mu^- \rho^0}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{166} = e^- \omega}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2007kx}}%
\htCombLimitLine%
  {\ensuremath{\BR_{167} = \mu^- \omega}}%
  {\ensuremath{}}%
  {\ensuremath{4.0 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2007kx}}%
\htCombLimitLine%
  {\ensuremath{\BR_{168} = e^- K^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{2.3 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{169} = \mu^- K^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{6.0 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{170} = e^- \bar{K}^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{2.2 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{171} = \mu^- \bar{K}^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{4.2 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{176} = e^- \phi}}%
  {\ensuremath{}}%
  {\ensuremath{2.0 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htCombLimitLine%
  {\ensuremath{\BR_{177} = \mu^- \phi}}%
  {\ensuremath{}}%
  {\ensuremath{6.8 \cdot 10^{-8}}}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\midrule%
\htCombLimitLine%
  {\ensuremath{\BR_{178} = e^- e^+ e^-}}%
  {\ensuremath{\ell\ell\ell}}%
  {\ensuremath{1.4 \cdot 10^{-8}}}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htCombLimitLine%
  {\ensuremath{\BR_{179} = e^- \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.6 \cdot 10^{-8}}}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htCombLimitLine%
  {\ensuremath{\BR_{180} = \mu^- e^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{9.8 \cdot 10^{-9}}}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htCombLimitLine%
  {\ensuremath{\BR_{181} = \mu^- e^+ e^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-8}}}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htCombLimitLine%
  {\ensuremath{\BR_{182} = e^- \mu^+ e^-}}%
  {\ensuremath{}}%
  {\ensuremath{8.4 \cdot 10^{-9}}}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htCombLimitLine%
  {\ensuremath{\BR_{183} = \mu^- \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-8}}}%
  {\cite{Hayasaka:2010np,Lees:2010ez,Aaij:2014azz}}}%
\htdef{LimitCombLines}{%
\htLimitLine%
  {\ensuremath{\BR_{156} = e^- \gamma}}%
  {\ensuremath{\ell\gamma}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ag}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.2 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Hayasaka:2007vc}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{5.4 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Hayasaka:2007vc,Aubert:2009ag}}%
\htLimitLine%
  {\ensuremath{\BR_{157} = \mu^- \gamma}}%
  {\ensuremath{}}%
  {\ensuremath{4.4 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ag}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2007vc}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{5.0 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Hayasaka:2007vc,Aubert:2009ag}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{158} = e^- \pi^0}}%
  {\ensuremath{\ell P^0}}%
  {\ensuremath{1.3 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.9 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{\BR_{159} = \mu^- \pi^0}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.2 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.6 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{\BR_{160} = e^- K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ys}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2010qb,Aubert:2009ys}}%
\htLimitLine%
  {\ensuremath{\BR_{161} = \mu^- K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{4.0 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ys}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.3 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2010qb,Aubert:2009ys}}%
\htLimitLine%
  {\ensuremath{\BR_{162} = e^- \eta}}%
  {\ensuremath{}}%
  {\ensuremath{1.6 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{9.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{5.5 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{\BR_{163} = \mu^- \eta}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{6.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.8 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{\BR_{172} = e^- \eta^\prime(958)}}%
  {\ensuremath{}}%
  {\ensuremath{2.4 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.6 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{9.9 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{\BR_{173} = \mu^- \eta^\prime(958)}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2006cz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.3 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2007jp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{6.3 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2007jp,Aubert:2006cz}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{164} = e^- \rho^0}}%
  {\ensuremath{\ell V^0}}%
  {\ensuremath{4.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{165} = \mu^- \rho^0}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{166} = e^- \omega}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2007kx}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2007kx}}%
\htLimitLine%
  {\ensuremath{\BR_{167} = \mu^- \omega}}%
  {\ensuremath{}}%
  {\ensuremath{1.0 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2007kx}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.0 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2007kx}}%
\htLimitLine%
  {\ensuremath{\BR_{168} = e^- K^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{5.9 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.3 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{169} = \mu^- K^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{1.7 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{7.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{6.0 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{170} = e^- \bar{K}^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{4.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.2 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{171} = \mu^- \bar{K}^*(892)}}%
  {\ensuremath{}}%
  {\ensuremath{7.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{7.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.2 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{176} = e^- \phi}}%
  {\ensuremath{}}%
  {\ensuremath{3.1 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.0 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{\BR_{177} = \mu^- \phi}}%
  {\ensuremath{}}%
  {\ensuremath{1.9 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2009ap}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2011xe}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{6.8 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Miyazaki:2011xe,Aubert:2009ap}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{174} = e^- f_0(980)}}%
  {\ensuremath{\ell S^0}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2008mw}}%
\htLimitLine%
  {\ensuremath{\BR_{175} = \mu^- f_0(980)}}%
  {\ensuremath{}}%
  {\ensuremath{3.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2008mw}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{178} = e^- e^+ e^-}}%
  {\ensuremath{\ell\ell\ell}}%
  {\ensuremath{2.9 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{\BR_{179} = e^- \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.6 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{\BR_{180} = \mu^- e^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{9.8 \cdot 10^{-9}}}%
  {HFLAV}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{\BR_{181} = \mu^- e^+ e^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.2 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{\BR_{182} = e^- \mu^+ e^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.4 \cdot 10^{-9}}}%
  {HFLAV}%
  {\cite{Hayasaka:2010np,Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{\BR_{183} = \mu^- \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.8 \cdot 10^{-7}}}%
  {ATLAS}%
  {\cite{Aad:2016wce}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Lees:2010ez}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Hayasaka:2010np}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.6 \cdot 10^{-8}}}%
  {LHCb}%
  {\cite{Aaij:2014azz}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{1.1 \cdot 10^{-8}}}%
  {HFLAV}%
  {\cite{Hayasaka:2010np,Lees:2010ez,Aaij:2014azz}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{184} = e^- \pi^+ \pi^-}}%
  {\ensuremath{\ell hh}}%
  {\ensuremath{1.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.3 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{185} = e^+ \pi^- \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.7 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{186} = \mu^- \pi^+  \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.9 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{2.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{187} = \mu^+ \pi^- \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{7.0 \cdot 10^{-8}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.9 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{188} = e^- \pi^+ K^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{189} = e^- K^+ \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.7 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{190} = e^+ \pi^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.8 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{191} = e^- K^0_S K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{7.1 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{\BR_{192} = e^- K^+ K^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{193} = e^+ K^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{1.5 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{194} = \mu^- \pi^+  K^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.6 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{8.6 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{195} = \mu^- K^+  \pi^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.5 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{196} = \mu^+ \pi^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.2 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.8 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{197} = \mu^- K^0_S  K^0_S}}%
  {\ensuremath{}}%
  {\ensuremath{8.0 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2010qb}}%
\htLimitLine%
  {\ensuremath{\BR_{198} = \mu^- K^+  K^-}}%
  {\ensuremath{}}%
  {\ensuremath{2.5 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.4 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\htLimitLine%
  {\ensuremath{\BR_{199} = \mu^+ K^- K^-}}%
  {\ensuremath{}}%
  {\ensuremath{4.8 \cdot 10^{-7}}}%
  {\babar}%
  {\cite{Aubert:2005tp}}%
\htLimitLine%
  {\ensuremath{}}%
  {\ensuremath{}}%
  {\ensuremath{4.7 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2012mx}}%
\midrule%
\htLimitLine%
  {\ensuremath{\BR_{211} = \pi^- \Lambda}}%
  {\ensuremath{\text{BNV}}}%
  {\ensuremath{7.2 \cdot 10^{-8}}}%
  {\belle}%
  {\cite{Miyazaki:2005ng}}%
\htLimitLine%
  {\ensuremath{\BR_{212} = \pi^- \bar{\Lambda}}}%
  {\ensuremath{}}%
  {\ensuremath{1.4 \cdot 10^{-7}}}%
  {\belle}%
  {\cite{Miyazaki:2005ng}}%
\htLimitLine%
  {\ensuremath{\BR_{215} = p \mu^- \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{4.4 \cdot 10^{-7}}}%
  {LHCb}%
  {\cite{Aaij:2013fia}}%
\htLimitLine%
  {\ensuremath{\BR_{216} = \bar{p} \mu^+ \mu^-}}%
  {\ensuremath{}}%
  {\ensuremath{3.3 \cdot 10^{-7}}}%
  {LHCb}%
  {\cite{Aaij:2013fia}}}%


==> tau/tau-lfv-limits-plot.tex <==
%
%
\ifhevea
\subsection{Upper limits on \mtau lepton-flavour-violating branching fractions: summary plot}
\cutname{lfv-limits-plot.html}
\fi

\begin{figure}[tb]
  \begin{center}
    \ifhevea
    \begin{tabular}{@{}cc@{}}
      \larger\bfseries\ahref{tau-lfv-limits.png}{full size PNG} &
      \larger\bfseries\ahref{tau-lfv-limits.pdf}{PDF format} \\
      \multicolumn{2}{c}{\ahref{tau-lfv-limits.png}{%
          \imgsrc[alt="Tau LFV limits combinations plot" width=720]{tau-lfv-limits.png}}}
    \end{tabular}
    \else
    \includegraphics[angle=90,totalheight=0.9\textheight,clip]{figures/tau/tau-lfv-limits.pdf}
    \fi
    \caption{Tau lepton-flavour-violating branching fraction upper
      limits summary plot. In order to appreciate the physics reach
      improvement over time, the plot includes also the CLEO upper
      limits reported by PDG 2018~\cite{PDG_2018}.
      \label{fig:tau:lfv-limits-plot}
    }
  \end{center}
\end{figure}


==> tau/tau-sections.tex <==
This section reports averages and elaborations of \mtau branching
fractions, and combinations of upper limits on \mtau branching fractions
to lepton-flavour-violating \mtau decay modes.

Branching fractions averages are obtained with a fit of \mtau branching fractions
measurements aimed at optimally exploiting the available experimental
information and described in Section~\ref{sec:tau:br-fit}. The fit
results are used in  
Section~\ref{sec:tau:leptonuniv} to test the lepton-flavour
universality of the charged-current weak interaction. The
``universality-improved''~\cite{Davier:2005xq}  branching fraction
$\BR_e=\BR(\tau \to e \nu \bar{\nu})$ and the ratio between the hadronic
branching fraction and $\BR_e$, are obtained in
Section~\ref{sec:tau:be-univ-rtau}.
The  value of the Cabibbo-Kobayashi-Maskawa
(CKM) matrix element \Vus from \mtau decays
is given in Section~\ref{sec:tau:vus}.
Combinations of upper limits on lepton-flavour-violating \mtau branching
fractions are computed in Section~\ref{sec:tau:lfv-limits}.
All results are obtained from inputs available through the end of 2018.

\iffalse
Since the 2016 edition,
the HFLAV-Tau group has collaborated to the determination of the
$\tau$-lepton branching fractions based on a global fit and to the
related mini-review that are included in the ``Review of particle
physics''~\cite{PDG_2018}.
\fi

%
\subsection{Branching fraction fit}
\cutname{br-fit.html}
\label{sec:tau:br-fit}

A fit of the available experimental measurements is used to
determine the \mtau branching fractions, together with their
uncertainties and correlations.
\iffalse
The \mtau branching fractions provide a test for theory predictions based
on the Standard Model (SM) EW and QCD interactions and can be further
elaborated to test the EW charged-current universality for leptons, and to
determine the CKM matrix coefficient \Vus and the QCD coupling constant
$\alpha_s$ at the \mtau mass. 
\fi

All relevant published statistical and systematic correlations among the
measurements are used. In addition, for a selection of measurements,
particularly the most precise and the most recent ones, the documented
systematic uncertainty contributions are examined to consider systematic
dependencies from external parameters.
\ifx\tauStandalone\undefined
We follow the procedures detailed in Section~\ref{sec:method:corrSysts} to
\else We use the standard HFLAV procedures to
\fi
account for the updated values and uncertainties of the external
parameters and for the correlations induced on different measurements
with a systematic dependence from the same external parameter.

Both the measurements and the fitted quantities consist of either \mtau
decay branching fractions, labelled as $\BR_{i}$, or ratios of two \mtau
decay branching fractions, labelled as $\BR_{i}/\BR_{j}$. Some branching
fractions are sums of other branching fractions, for instance
$\htuse{Gamma8.gn} = \BR(\tau\to\htuse{Gamma8.td})$ is the sum of
$\htuse{Gamma9.gn} = \BR(\tau\to\htuse{Gamma9.td})$ and
$\htuse{Gamma10.gn} = \BR(\tau\to\htuse{Gamma10.td})$. The symbol $h$ is
used to mean either a $\pi$ or a $K$.  The fit \chisq is minimized while
respecting a list of constraints on the fitted quantities:
\begin{itemize}

\item quantities corresponding to ratios like $\BR_{i}/\BR_{j}$ must
  be equal to the ratio of the respective quantities $\BR_{i}$ and
  $\BR_{j}$;

\item quantities corresponding to branching fractions that are sum of
  other branching fractions must be equal to the sum of the quantities
  corresponding to the summed branching fractions.

\end{itemize}
In some cases, constraints describe approximate relations that
nevertheless hold within the present experimental precision. For
instance, the constraint $\BR(\tau\to\htuse{Gamma96.td}) =
\BR(\tau\to\htuse{Gamma167.td}) \times \BR(\phi\to K^+K^-)$
is justified within the current experimental evidence.
Section~\ref{sec:tau:constraints} lists all equations
relating one quantity to other quantities.

\subsubsection{Technical implementation of the fit procedure}
\label{sec:tau:fit-techn}%
\newcommand{\htvarE}{V}%
\newcommand{\htvarm}{x}%

The fit computes the quantities $q_i$ by minimizing a $\chi^2$
while respecting a series of equality constraints on the $q_i$.
The $\chi^2$ is computed using the measurements $\htvarm_i$ and their
covariance matrix $\htvarE_{ij}$ as
\begin{align}
\chi^2 = (\htvarm_i - A_{ik}q_k)^t \htvarE_{ij}^{-1} (\htvarm_j - A_{jl}q_l)~,\label{eq:tau:chisq}
\end{align}
where the model matrix $A_{ij}$ is used to get the
vector of the predicted measurements $\htvarm_i^\prime$ from the vector of the
fit parameters $q_j$ as $\htvarm_i^\prime = A_{ij}q_j$. In this
particular implementation, the measurements are grouped according to
the measured quantity, and all quantities with at least one measurement
correspond to a fit parameter. Therefore, the
matrix $A_{ij}$ has one row per
measurement $\htvarm_i$ and one column per fitted
quantity $q_j$, with unity coefficients for the rows and column that
identify a measurement $\htvarm_i$ of the quantity $q_j$.
In summary, the \chisq given in Eq.~(\ref{eq:tau:chisq}) is minimized subject 
to the constraints
\begin{align}
  f_r(q_s) - c_r = 0~, \label{eq1;b}
\end{align}
where Eq.~(\ref{eq1;b}) corresponds to the constraint equations, written
as a set of ``constraint expressions'' that are equated to zero.
Using the method of Lagrange multipliers, a set of equations is obtained by
taking the derivatives with respect to the fitted quantities $q_k$ and the
Lagrange multipliers $\lambda_r$ of the sum of the $\chi^2$ and the
constraint expressions multiplied by the
Lagrange multipliers $\lambda_r$, one for each constraint:
\begin{align}
&\text{min} \left[h = (A_{ik}q_k {-} \htvarm_i)^t \htvarE_{ij}^{-1} (A_{jl}q_l {-} \htvarm_j) +
2\lambda_r(f_r(q_s) - c_r) \right] \label{eq2;a}
\\
&(\partial/\partial q_k, \partial/\partial \lambda_r) \, h = 0~. \label{eq2;b}
\end{align}
%
%
Equation~(\ref{eq2;b}) defines a set of equations for the vector of the unknowns $(q_k,
\lambda_r)$, some of which may be non-linear, in case of non-linear
constraints. An iterative minimization procedure approximates at
each step the non-linear constraint expressions by their first order
Taylor expansion around the current values of the fitted quantities,
$\bar{q}_s$:
\begin{align}
f_r(q_s) - c_r \simeq
f_r(\bar{q}_s) + \left.\frac{\partial f_r(q_s)}{\partial q_s}\right|_{\bar{q}_s} (q_s - \bar{q}_s) - c_r~, \label{eq3;a}
\end{align}
which can be written as
\begin{align}
B_{rs} q_s - c^\prime_r~, \label{eq3;b}
\end{align}
where $c^\prime_r$ are the resulting constant known terms, independent
of $q_s$ at first order. After linearization, the differentiation by
$q_k$ and $\lambda_r$ is trivial and leads to a set of linear equations
\begin{align}
&A_{ki}^t \htvarE_{ij}^{-1} A_{jl} q_l + B^t_{kr} \lambda_r =  A_{ki}^t \htvarE_{ij}^{-1} \htvarm_j \label{eq4;a}
\\
&B_{rs} q_s = c^\prime_r~, \label{eq4;b}
\end{align}
which can be expressed as:
\begin{align}
F_{ij} u_j = v_i~, \label{eq5}
\end{align}
where $u_j = (q_k, \lambda_r)$ and $v_i$ is the vector of the known
constant terms running over the index $k$ and then $r$ in the right
terms of Eq.~(\ref{eq4;a}) and Eq.~(\ref{eq4;b}). Solving the equation
set in Eq.~(\ref{eq5}) gives the fitted quantities and
their covariance matrix, using the measurements and their
covariance matrix.
%
%
%
%
%
%
The fit procedure starts by computing the linear
approximation of the non-linear constraint
expressions around the quantities seed values. With an
iterative procedure, the unknowns are updated at each step by solving
the equations and the equations are then linearized around the updated
values, until the RMS average of relative variation of the
fitted unknowns is reduced below $10^{-12}$.

\subsubsection{Fit results}
\label{sec:tau:fit}

Although the fit treats all quantities in the same way, for the
purpose of describing the results we select a set
of \htuse{BaseQuantNum} ``basis quantities'' from which all remaining
quantities can be calculated using the definitions listed in
Section~\ref{sec:tau:constraints}.

The fit output consists of \htuse{QuantNum} fitted quantities that correspond to
either branching fractions or ratios of branching
fractions. The fitted quantities values and uncertainties are listed in
Table~\ref{tab:tau:br-fit}. The off-diagonal correlation terms
between the basis quantities are listed
in Section~\ref{sec:tau:fitcorr}.

Furthermore we define (see Section~\ref{sec:tau:constraints}) $\BR_{110}
= \BR(\tau^- \to X_s^- \nu_\tau)$, the total branching fraction of the \mtau
decays to final states with the strangeness quantum number equal to one, and
$\BR_{\text{All}}$, the branching fraction of the \mtau into any
measured final state, which should be equal to $1$ within the
experimental uncertainty. We define the unitarity residual as $\BR_{998}
= 1 -\BR_{\text{All}}$.

The fit has $\chi^2/\text{d.o.f.} = \htuse{Chisq}/\htuse{Dof}$,
corresponding to a confidence level $\text{CL} = \htuse{ChisqProb}$. We use a total of
\htuse{MeasNum} measurements to fit the above mentioned
\htuse{QuantNum} quantities subjected to \htuse{ConstrNum} constraints.
Although the unitarity constraint is not applied, the fit is statistically
consistent with unitarity, where the residual is
\htuse{Gamma998.gn} =  \htuse{Gamma998.td} = \htuse{Gamma998}.

\label{ref:tau:kkk-error-scale-factor}%
%
A scale factor of 5.44 has been applied
to the published uncertainties of the two severely inconsistent
measurements of \(\BR_{96} = \tau \to KKK\nu\) by \babar and
Belle. The scale factor has been determined using the PDG procedure,
\ie, to the proper size in order to obtain a reduced \chisq equal to $1$
when fitting just the two \(\BR_{96}\) measurements.

%
\subsubsection{Changes with respect to the previous report}

The following changes have been introduced with respect to the previous
HFLAV report~\cite{Amhis:2016xyh}.

We added the \babar 2018 result~\htuse{LEES 18B.cite} for the \mtau branching fraction
{\setlength{\LTleft}{\parindent}%
\begin{longtable}{@{}ll@{}}
\htuse{LEES 18B.meas}~,
\end{longtable}}
\noindent
and the 2018 \babar preliminary results~\htuse{BaBar prelim. ICHEP2018.cite}
for the \mtau branching fractions
{\setlength{\LTleft}{\parindent}%
\begin{longtable}{@{}ll@{}}
\htuse{BaBar prelim. ICHEP2018.meas}~.
\end{longtable}}
\noindent The above \htuse{Gamma16.gn} result supersedes the previous
\babar result in Ref.~\cite{Aubert:2007jh}.

\iffalse
The ALEPH measurement on \htuse{Gamma49.gn} ($\tau^- \to
\htuse{Gamma49.td}$)~\cite{Barate:1999hj} has been added. It is
computed by ALEPH as the sum of $\htuse{Gamma51.gn} =
\htuse{Gamma51.td}$, also measured by ALEPH~\cite{Barate:1999hj}, 
$\htuse{Gamma50.gn} = \htuse{Gamma50.td}$, which was measured by ALEPH
as not being significant above zero~\cite{Barate:1999hj}, and
$\htuse{Gamma806.gn} = \htuse{Gamma806.td}$. It is assumed that
\htuse{Gamma806.gn} and \htuse{Gamma50.gn} are equal.
By using in the fit the measurements of \htuse{Gamma49.gn} and
\htuse{Gamma51.gn} by ALEPH, with a proper statistical correlation
coefficient to account for the determination of \htuse{Gamma49.gn},
the two measurements contribute to determine also \htuse{Gamma50.gn}
and \htuse{Gamma806.gn}.
\fi

\iffalse
%
%
%
%
%
%
%
%
The total \mtau branching fraction \htuse{GammaAll.gn} definition
includes two modes that have overlapping final states, to a minor
extent, which we consider negligible:
\begin{align*}
  &\htuse{Gamma50.gn} =  \htuse{Gamma50.td} \\
  &\htuse{Gamma132.gn} =  \htuse{Gamma132.td}~.
\end{align*}
\fi

The parameters used to update the measurements' systematic biases and
the parameters appearing in the constraint
equations in Section~\ref{sec:tau:constraints} have been updated to the
PDG 2018 averages~\cite{PDG_2018}.

%
\subsubsection{Differences between the HFLAV 2018 fit and the PDG 2018
  fit}
\label{sec:tau:diffpdg}

As is standard for the PDG branching fraction fits, the PDG 2018 \mtau branching
fraction fit is unitarity constrained, while the HFLAV 2018 fit is
unconstrained.

The HFLAV-Tau fit uses an elaboration of the measurements
reported on the main ALEPH paper on \mtau branching fractions~\cite{Schael:2005am} to
obtain branching fractions to inclusive final states with ``hadrons''
(where a hadron is either a pion or a kaon), since
this set of results is closer to the actual experimental measurements
and facilitates a more appropriate and
comprehensive treatment of the experimental results correlations.
The PDG 2018 fit on the other hand
continues to use -- as in the past editions -- the published ALEPH measurements
of branching fractions to esclusive final states with pions~\cite{Schael:2005am}.

\iffalse
The HFLAV Spring 2017 fit includes two preliminary results that are not
included in the PDG 2016 fit:
\begin{align*}
  \begin{tabular}{@{}lll}
    \htuse{BaBar prelim. ICHEP08.meas} & \htuse{BaBar prelim. ICHEP08.cite}~, \\
    \htuse{BaBar prelim. DPF09.meas} & \htuse{BaBar prelim. DPF09.cite}~.
  \end{tabular}
\end{align*}
\fi

As in 2016, HFLAV uses the ALEPH estimate for
$\htuse{Gamma805.gn} =  \BR(\tau\to\htuse{Gamma805.td})$, which is not a direct
measurement, and the PDG 2018 fit uses the PDG average of
$\BR(a_1\to\pi\gamma)$ as a parameter and defines $\htuse{Gamma805.gn}
= \BR(a_1\to\pi\gamma)\times\BR(\tau \to 3\pi \nu)$. As a consequence, the PDG fit
procedure does not take into account the large uncertainty on $\BR(a_1\to\pi\gamma)$,
resulting in an underestimated fit uncertainty on \htuse{Gamma805.gn}.
Therefore, in this case an appropriate correction has been applied after the fit.

Finally, the HFLAV 2018 \mtau branching fraction fit includes measurements that appeared after the
deadline for inclusion in the PDG, and preliminary measurements that are
not included in the PDG.

\iffalse
Unlike this edition of the HFLAV-Tau fit, the PDG 2016 fit does not
include the  \htuse{Gamma49.gn} ($\tau^- \to
\htuse{Gamma49.td}$)~\cite{Barate:1999hj} measurement. Its inclusion
would have required adding a proper correlation term in the PDG tables,
which has been postponed.
\fi

%
\subsubsection{Branching ratio fit results and experimental inputs}
\label{sec:tau:br-fit-results}

Table~\ref{tab:tau:br-fit} reports the \mtau branching ratio fit results
and experimental inputs.

%
%
%
\begin{center}
\begin{envsmall}
\setlength{\LTcapwidth}{0.85\linewidth}
\renewcommand*{\arraystretch}{1.3}%
\ifhevea
\renewcommand{\bar}[1]{\textoverline{#1}}
\else
\begin{citenoleadsp}
\fi
\begin{longtable}{llll}
\caption{HFLAV \hfagTauTag branching fractions fit results.\label{tab:tau:br-fit}}%
\\
\toprule
\multicolumn{1}{l}{\bfseries \mtau lepton branching fraction} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{l}{\bfseries Reference} \\
\midrule
\endfirsthead
\multicolumn{4}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
\multicolumn{1}{l}{\bfseries \mtau lepton branching fraction} &
\multicolumn{1}{l}{\bfseries Experiment} &
\multicolumn{1}{l}{\bfseries Reference} \\
\midrule
\endhead
\endfoot
\endlastfoot
\htuse{BrVal} \\
\bottomrule
\end{longtable}
\ifhevea\else
\end{citenoleadsp}
\fi
\end{envsmall}
\end{center}

\subsubsection{Correlation terms between basis branching fractions uncertainties}
\label{sec:tau:fitcorr}

The following tables report the correlation coefficients between basis
quantities that were obtained from the \mtau branching fractions fit,
in percent.

%
%
%
\htuse{BrCorr}

\subsubsection{Equality constraints}
\label{sec:tau:constraints}

The constraints on the \mtau branching fractions fitted quantities are
listed in the following.
The constraint equations include as coefficients the
values of some non-tau branching fractions, denoted \eg, with the
self-describing notation $\BR_{K_S \to \pi^0\pi^0}$. Some coefficients
are probabilities corresponding to the modulus square of amplitudes
describing quantum
mixtures of states such as $K^0$, $\bar{K}^0$, $K_S$, $K_L$, denoted with
\eg, $\BR_{<K^0|K_S>} = |{<}K^0|K_S{>}|^2$.
All non-tau quantities are taken from the PDG 2018~\cite{PDG_2018}
averages. The fit procedure does not account for their
uncertainties, which are generally small with respect
to the uncertainties on the \mtau branching fractions.
Please note that, in the following table, when a quantity like
$\BR_3/\BR_5$ appears on the left side of the equation, it represents a
fitted quantity, and when it appears on the right side it represents the
ratio of two separate fitted quantities.

\begin{envsmall}
  \setlength\abovedisplayskip{0pt}
  \setlength\belowdisplayshortskip{0pt}
  \ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
  %
  %
  %
  \htuse{ConstrEqs}
\end{envsmall}

\iffalse
%
%
%
The \mtau branching fractions are listed in Table~\ref{tab:tau:br-fit}.
The equations in the following permit the computation of the values and
uncertainties for branching fractions that are not listed in
Table~\ref{tab:tau:br-fit}, once they are expressed as function of the
quantities that are listed there. 
\fi

%
\subsection{Tests of lepton universality}
\cutname{lepton-univ.html}
\label{sec:tau:leptonuniv}

Lepton universality tests probe the Standard Model prediction that the
charged weak current interaction has the same coupling for all lepton generations.
The precision of such tests has been significantly improved since the
2014 edition by the
addition of the Belle \mtau lifetime
measurement~\cite{Belous:2013dba}, while improvements from the \mtau
branching fraction fit are negligible.
We compute the universality tests by using
ratios of the partial widths of a heavier lepton $\lepth$
decaying to a lighter lepton $\leptl$~\cite{Marciano:1988vm},
\begin{align*}
  \Gamma(\lepth \to \nu_{\lepth} \leptl \nub_{\leptl} (\gamma)) =
  \frac{\BR(\lepth \to \nu_{\lepth} \leptl \nub_{\leptl})}{\tau_{\lepth}} =
  \frac {G_{\lepth} G_{\leptl} m^5_{\lepth}}{192 \pi^3}\, f\left(\frac {m^2_{\leptl}}{m^2_{\lepth}}\right)
  \radRatio^{\lepth}_W \radRatio^{\lepth}_\gamma~,
\end{align*}
where
\begin{alignat*}{3}
 G_{\leptl} &= \frac {g^2_{\leptl}}{4 \sqrt{2} M^2_W}~, &\quad&&
 f(x) &= 1 -8x +8x^3 -x^4 -12x^2 \text{ln}x~, \\
 \radRatio^{\lepth}_W &= 1 + \frac {3}{5} \frac {m^2_{\lepth}}{M^2_W} + \frac {9}{5} \frac {m^2_{\leptl}}{M^2_W}~
\cite{Pich:2013lsa, Ferroglia:2013dga, Fael:2013pja}, &\quad\quad&&
 \radRatio^{\lepth}_\gamma &= 1+\frac {\alpha(m_{\lepth})}{2\pi} \left(\frac {25}{4}-\pi^2\right)~.
\end{alignat*}
We use $\radRatio^\tau_\gamma=1-43.2\cdot 10^{-4}$ and
$\radRatio^\mu_\gamma=1-42.4\cdot 10^{-4}$~\cite{Marciano:1988vm} and $M_W$
from PDG 2018~\cite{PDG_2018}.
We use HFLAV 2018 averages and PDG 2018 for the other quantities.
Using pure leptonic processes we obtain
\begin{align*}
  \left( \frac{g_\tau}{g_\mu} \right) = \htuse{gtaubygmu_tau}~,
  && \left( \frac{g_\tau}{g_e} \right) = \htuse{gtaubyge_tau}~,
  && \left( \frac{g_\mu}{g_e} \right) = \htuse{gmubyge_tau}~.
\end{align*}
Using the expressions for the \mtau semi-hadronic partial
widths, we obtain
\begin{align*}
  \left( \frac{g_\tau}{g_\mu} \right)^2 =
  \frac{\BR({\tau \to h \nu_\tau})}{\BR({h \to \mu \bar{\nu}_\mu})}
  \frac{2m_h m^2_{\mu}\tau_h}{(1 + \dRradTauhHmu)m^3_{\tau}\tau_{\tau}}
  \left( \frac{1-m^2_{\mu}/m^2_h}{1-m^2_h/m^2_{\tau}} \right)^2~,
\end{align*}
where $h$ = $\pi$ or $K$ and the radiative corrections are
$\dRradTaupiPimu = (\htuse{dRrad_taupi_by_pimu})\%$ and
$\dRradTaukKmu = (\htuse{dRrad_tauK_by_Kmu})\%$~\cite{Marciano:1993sh,Decker:1994dd,Decker:1994ea,Decker:1994kw}.
We measure:
\begin{align*}
  \left( \frac{g_\tau}{g_\mu} \right)_\pi &= \htuse{gtaubygmu_pi}~,
  & \left( \frac{g_\tau}{g_\mu} \right)_K = \htuse{gtaubygmu_K}~.
\end{align*}
Similar tests could be performed with decays to electrons, however they are
less precise because the hadron two body decays to electrons are
helicity-suppressed.
Averaging the three \(g_\tau/g_\mu\) ratios we obtain
\begin{align*}
  \left( \frac{g_\tau}{g_\mu} \right)_{\tau{+}\pi{+}K} &= \htuse{gtaubygmu_fit}~,
\end{align*}
accounting for correlations.
Table~\ref{tab:tau:univ-fit-corr} reports the correlation coefficients for the fitted coupling ratios.
\ifhevea\begin{table}\fi%
\begin{center}
\ifhevea
\caption{Universality coupling ratios correlation coefficients (\%).\label{tab:tau:univ-fit-corr}}%
\else
\begin{minipage}{\linewidth}
\begin{center}
\captionof{table}{Universality coupling ratios correlation coefficients (\%).}\label{tab:tau:univ-fit-corr}%
\fi
\begin{center}
\renewcommand*{\arraystretch}{1.1}%
\begin{tabular}{lcccc}
\toprule
\htuse{couplingsCorr}
\\\bottomrule
\end{tabular}
\end{center}
\ifhevea\else
\end{center}
\end{minipage}
\fi
\end{center}
\ifhevea\end{table}\fi
\noindent Since there is 100\% correlation between $g_\tau/g_\mu$,
$g_\tau/g_e$ and $g_\mu/g_e$, the correlation matrix is expected to be
positive semi-definite, with one eigenvalue equal to zero. Due to
numerical inaccuracies, one eigenvalue is expected to be close to zero
rather than exactly zero.

%
\subsection{\texorpdfstring{%
  Universality-improved $\BR(\tau \to e \nu \bar{\nu})$ and $\Rhad$}{%
  Universality-improved B(tau -> e nu nu\_bar) and Rhad}}
\cutname{Be_univ_and_Rtau.html}
\label{sec:tau:be-univ-rtau}

We compute two quantities that are used in this report and that have been
traditionally used for further elaborations and
tests involving the \mtau branching fractions:
\begin{itemize}
  
\item the ``universality-improved'' experimental
  determination of $\BR_e = \BR(\tau \to e \nu \bar{\nu})$, which relies on the assumption
  that the Standard Model and lepton universality hold;

\item the ratio \Rhad between the
total branching fraction of the \mtau to hadrons, $\BR_{\text{had}}$ and the universality-improved $\BR_e$, which is the same as the ratio of the two respective
partial widths, $\Gamma(\tau \to \text{had})$ and $\Gamma(\tau\to e\nu\bar{\nu})$.
\end{itemize}

Following Ref.~\cite{Davier:2005xq}, we obtain a more precise experimental
determination of $\BR_e$ using the
\mtau branching fraction to $\mu \nu \bar{\nu}$, $\BR_\mu$, and the \mtau lifetime. We average:
\begin{itemize}

\item the $\BR_e$ fit value \htuse{Gamma5.gn},

\item
  the $\BR_e$ determination from the $\BR_\mu = \BR(\tau \to \mu \nu
  \bar{\nu})$ fit value \htuse{Gamma3.gn} assuming that $g_\mu/g_e = 1$,
  hence (see also Section~\ref{sec:tau:leptonuniv})
  $$
  \BR_e = \BR_\mu \cdot f(m^2_e/m^2_\tau)/f(m^2_\mu/m^2_\tau)~,
  $$

\item
  the $\BR_e$ determination from the \mtau lifetime assuming that
  $g_\tau/g_\mu =1$, hence
  $$
  \BR_e = \BR(\mu \to e \bar{\nu}_e
  \nu_\mu)\cdot (\tau_\tau / \tau_\mu) \cdot (m_\tau/m_\mu)^5 \cdot
  f(m^2_e/m^2_\tau)/f(m^2_e/m^2_\mu) \cdot (\radRatio_\gamma^\tau
  \radRatio_W^\tau)/(\radRatio_\gamma^\mu \radRatio_W^\mu)~,
  $$
  where $\BR(\mu \to e
  \bar{\nu}_e \nu_\mu) = 1$.

\end{itemize}
Accounting for correlations, we obtain
\begin{align*}
  \BR_e^{\text{uni}} = (\htuse{Be_univ})\%.
\end{align*}
%
We use $\BR_e^{\text{uni}}$ to obtain the ratio
\begin{align*}
  \Rhad = \frac{\Gamma(\tau \to \text{hadrons})}{\Gamma(\tau\to
    e\nu\bar{\nu})} = \frac{\BR_{\text{had}}}{\BR_e^{\text{uni}}} =
  \htuse{R_tau}~.
\end{align*}
We define $\BR_{\text{had}}$ as the sum of all {\em measured}
branching fractions to hadrons, which corresponds to the sum of all
branching fractions minus the leptonic branching fractions,
$\BR_{\text{had}} = \htuse{GammaAll.gn} - \BR_e - \BR_\mu =
(\htuse{B_tau_had_fit})\%$ (see
Section~\ref{sec:tau:br-fit} and Table~\ref{tab:tau:br-fit} for more details on the
definition of \htuse{GammaAll.gn}).
An alternative definition of $\BR_{\text{had}}$ uses the unitarity of
the sum of all branching fractions,
$\BR_{\text{had}}^{\text{uni}} = 1 - \BR_e - \BR_\mu =
(\htuse{B_tau_had_uni})\%$, and results in:
\begin{align*}
  \Rhad^{\text{uni}} = \frac{1 - \BR_e - \BR_\mu}{\BR_e^{\text{uni}}} =
  \htuse{R_tau_uni}~.
\end{align*}
A third definition of $\BR_{\text{had}}$ uses the unitarity of
the sum of all branching fractions, the Standard Model prediction
$\BR_\mu = \BR_e \cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau)$ and $ \BR_e^{\text{uni}}$ to define
$\BR_{\text{had}}^{\text{uni, SM}} = 1 -  \BR_e^{\text{uni}} -
\BR_e^{\text{uni}} \cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau) =
(\htuse{B_tau_had_uni_SM})\%$, and to compute
\begin{align*}
  \Rhad^{\text{uni, SM}} = \frac{1 - \BR_e^{\text{uni}} -
    \BR_e^{\text{uni}}\cdot f(m^2_\mu/m^2_\tau)/f(m^2_e/m^2_\tau)}{\BR_e^{\text{uni}}} =
  \htuse{R_tau_uni_SM}~.
\end{align*}
Although $\BR_{\text{had}}^{\text{uni}}$ and
$\BR_{\text{had}}^{\text{uni, SM}}$ are more precise than
$\BR_{\text{had}}$, the precision of $\Rhad^{\text{uni}}$ and
$\Rhad^{\text{uni, SM}}$ is just slightly better than the one of \Rhad
because there are larger correlations between
$\BR_{\text{had}}^{\text{uni}}$, $\BR_{\text{had}}^{\text{uni, SM}}$ and
$\BR_e^{\text{uni}}$ than between $\BR_{\text{had}}$ and $\BR_e^{\text{uni}}$.

%
\subsection{\texorpdfstring{$\Vus$ measurement}{Vus measurement}}
\cutname{vus.html}
\label{sec:tau:vus}

The CKM matrix element magnitude \Vus is most precisely determined from kaon
decays~\cite{Antonelli:2010yf} (see Figure~\ref{fig:tau:vus-summary}),
and its precision is limited by the
uncertainties of the lattice QCD estimates of the meson decay constants $f_+^{K\pi}(0)$
and $f_{K\pm}/f_{\pi\pm}$.
Using the \mtau branching fractions, it is possible to determine \Vus in an
alternative way~\cite{Gamiz:2002nu,Gamiz:2004ar} that does not depend on lattice QCD and
has small theory uncertainties (as discussed in Section~\ref{sec:tau:vus:incl}).
Moreover, \Vus can be determined using the \mtau branching fractions
similarly to the kaon case, using the same meson decay constants from lattice QCD.

%
\subsubsection{\texorpdfstring{\Vus from $\BR(\tau \to X_s\nu)$}{Vus from B(tau -> X\_s nu)}}
\label{sec:tau:vus:incl}

The \mtau hadronic partial width is the sum of the \mtau partial widths to
strange and to non-strange hadronic final states, $\Gammahad =
\Gammastrange + \Gammanonstrange$.  The suffix ``VA'' traditionally denotes
the sum of the \mtau partial widths to non-strange final states, which proceed
through either vector or axial-vector currents.

Dividing any partial width $\Gamma_x$
by the electronic partial width, $\Gamma_e$, we obtain partial width ratios
$R_x$ (which are equal to the respective branching fraction ratios
$\BR_x/\BR_e$) for which $\Rhad = \Rstrange + \Rnonstrange$. In terms of
such ratios, \Vus can be measured as~\cite{Gamiz:2002nu,Gamiz:2004ar}
\begin{align*}
  \VusTauIncl &= \sqrt{\Rstrange/\left[\frac{\Rnonstrange}{\Vud^2} -  \delta R_{\text{theory}}\right]}~,
\end{align*}
where $\delta R_{\text{theory}}$ can be determined in the context of low
energy QCD theory, partly relying on experimental low energy scattering
data. The literature reports several
calculations~\cite{Gamiz:2006xx,Gamiz:2007qs,Maltman:2010hb}. In this
report we use Ref.~\cite{Gamiz:2006xx}, whose estimated uncertainty size is
intermediate between the two other ones. We use the information in that paper and the
PDG 2018 value for the $s$-quark mass $m_s = \htuse{m_s}\,\text{MeV}$~\cite{PDG_2018}
to calculate $\delta R_{\text{theory}} = \htuse{deltaR_su3break}$.

We proceed following the same procedure of the 2012 HFLAV
report~\cite{Amhis:2012bh}. We sum the relevant \mtau branching
fractions to compute $\BRnonstrange$ and $\BRstrange$ and we use the
universality-improved $\BR_e^{\text{uni}}$ (see
Section~\ref{sec:tau:be-univ-rtau}) to compute the $\Rnonstrange$ and $\Rstrange$  ratios.
In past determinations of \Vus, for example in the 2009 HFLAV
report~\cite{Asner:2010qj}, the total hadronic branching fraction
has been computed using unitarity as $\BRhad^{\text{uni}} = 1 - \BR_e
-\BR_\mu$, obtaining then $\BRstrange$ from the sum of the strange
branching fractions and $\BRnonstrange$ from $\BRhad^{\text{uni}} -
\BRstrange$. We prefer to use the more direct experimental determination
of $\BRnonstrange$ for two reasons.
First, both methods result in comparable uncertainties on \Vus,
since the better precision on  $\BRhad^{\text{uni}} = 1 - \BR_e
-\BR_\mu$ is counterbalanced by increased correlations in the
expressions $(1-\BR_e -\BR_\mu)/\BR_e^{\text{univ}}$ and
$\BRstrange/(\BRhad-\BRstrange)$ in the \Vus calculation. Second, if
there are unobserved \mtau hadronic decay modes, they would affect
\BRnonstrange and \BRstrange in a more asymmetric way when using
unitarity.

Using the \mtau branching fraction fit results with their uncertainties
and correlations (Section~\ref{sec:tau:br-fit}), we compute $\BRstrange =
(\htuse{B_tau_s_fit})\%$ (see also Table~\ref{tab:tau:vus}) and
$\BRnonstrange = \BR_{\text{had}} - \BRstrange=
(\htuse{B_tau_VA_fit})\%$, where $\BR_{\text{had}}$ has been defined in
section~\ref{sec:tau:be-univ-rtau}. PDG 2018 averages
are used for non-\mtau quantities; $\Vud =
\htuse{Vud}$~\cite{Hardy:2014qxa,Hardy:2016vhg}.

We obtain $\VusTauIncl = \htuse{Vus}$, which
is $\htuse{Vus_mism_sigma_abs}\sigma$ lower than the unitarity CKM
prediction $\VusUni = \htuse{Vus_uni}$, from $(\VusUni)^2 = 1 -
\Vud^2 - \Vub^2$. The \VusTauIncl uncertainty includes a systematic error
contribution of \htuse{Vus_err_th} from the theory uncertainty on
$\delta R_{\text{theory}}$. The 2018 \babar preliminary results improved
the \Vus precision by about 10\% and reduced the discrepancy by about
6.5\%.

%
%
%
\begin{table}
\begin{center}
\renewcommand*{\arraystretch}{1.3}%
\caption{HFLAV \hfagTauTag \mtau branching fractions to strange final states.\label{tab:tau:vus}}%
\ifhevea\renewcommand{\bar}[1]{\textoverline{#1}}\fi
\begin{envsmall}
\begin{center}
\begin{tabular}{lc}
\toprule
\multicolumn{1}{l}{\bfseries Branching fraction} &
\multicolumn{1}{c}{\bfseries HFLAV \hfagTauTag fit (\%)} \\
\midrule
\htuse{BrStrangeVal}
\midrule
\htuse{BrStrangeTotVal}
\bottomrule
\end{tabular}
\end{center}
\end{envsmall}
\end{center}
\end{table}

%
%
\subsubsection{\texorpdfstring{%
  \Vus from $\BR(\tau \to K\nu) / \BR(\tau \to \pi\nu)$}{%
  Vus from B(tau -> K nu) / B(tau -> pi nu)}}
\label{sec:tau:vus:taukpi}
%
%

We compute \Vus from
the ratio of branching fractions $\BR(\tau \to \htuse{Gamma10.td}) / \BR(\tau \to \htuse{Gamma9.td}) =
\htuse{Gamma10by9}$
from the equation~\cite{Banerjee:2008hg}:
\begin{align*}
\frac{\BR(\tau \to \htuse{Gamma10.td})}{\BR(\tau \to \htuse{Gamma9.td})} &=
\frac{f_{K\pm}^2 \Vus^2}{f_{\pi\pm}^2 \Vud^2} \frac{\left( m_\tau^2 - m_K^2 \right)^2}{\left( m_\tau^2 -  m_\pi^2 \right)^2}
\frac{1+\delta R_{\tau/K}}{1+\delta R_{\tau/\pi}}(1+\delta R_{K/\pi})
\end{align*}
We use $f_{K\pm}/f_{\pi\pm} = \htuse{f_Kpm_by_f_pipm}$ from the
FLAG 2019 lattice QCD averages with
$N_f=2+1+1$~\cite{Aoki:2019cca,Dowdall:2013rya,Carrasco:2014poa,Bazavov:2017lyh},
\begin{align*}
  &\frac{1+\delta R_{\tau/K}}{1+\delta R_{\tau/\pi}} =
  \frac{1+(\htuse{dRrad_tauK_by_Kmu})\%}{1+(\htuse{dRrad_taupi_by_pimu})\%}%
  ~\cite{Marciano:1993sh,Decker:1994dd,Decker:1994ea,Decker:1994kw}~,\\
  &1+\delta R_{K/\pi} = 1 + (\htuse{dRrad_kmunu_by_pimunu})\%~\cite{Pich:2013lsa,Cirigliano:2011tm,Marciano:2004uf}~.
\end{align*}
The value of $\delta R_{K/\pi}$ in the Spring 2017 HFLAV-Tau report~\cite{Amhis:2016xyh}
incorrectly included a strong isospin-breaking correction that is not
needed when using $f_{K\pm}/f_{\pi\pm}$ rather than its isospin-limit variant.
We compute $\VusTauKpi = \htuse{Vus_tauKpi}$,
$\htuse{Vus_tauKpi_mism_sigma_abs}\sigma$ below the CKM unitarity prediction.

%
%
%
\subsubsection{\texorpdfstring{%
    \Vus from $\BR(\tau \to K\nu)$}{%
    Vus from B(tau -> K nu)}}
\label{sec:tau:vus:tauk}
%
%

We determine \Vus from the branching fraction
$\BFtautoknu$ using
\begin{align*}
  \BR(\tau^- \to K^-\nu_\tau) =
  \frac{G^2_F}{16\pi\hslash} f^2_{K\pm} \Vus^2 \tau_{\tau}  m_{\tau}^3 \left(1 - \frac{m_K^2}{m_\tau^2}\right)^2
  \iffalse S_{EW} \fi
  (1+\delta R_{\tau/K}) (1+\delta R_{K\mu2})~.
\end{align*}
We use $f_{K\pm} = \htuse{f_Kpm}\,\mev$ from the FLAG 2019 lattice QCD averages with
$N_f=2+1+1$~\cite{Aoki:2019cca,Dowdall:2013rya,Bazavov:2014wgs,Carrasco:2014poa},
\iffalse $S_{EW} = \htuse{Rrad_SEW_tau_Knu}$~\cite{Erler:2002mv}, \fi
$\delta R_{\tau/K} =
(\htuse{dRrad_tauK_by_Kmu})\%$~\cite{Marciano:1993sh,Decker:1994dd,Decker:1994ea,Decker:1994kw}
and $\delta R_{K\mu2} =
(\htuse{dRrad_K_munu})\%$~\cite{Cirigliano:2011tm, PDG_2018, Rosner:2015wva}, which includes short
and long-distance radiative corrections.
We obtain $\VusTauKnu = \htuse{Vus_tauKnu}$,
which is $\htuse{Vus_tauKnu_mism_sigma_abs}\sigma$ below
the CKM unitarity prediction. The physical constants have been taken
from PDG 2018 (which uses CODATA 2014~\cite{Mohr:2015ccw}).

%
%
%
\subsubsection{\texorpdfstring{\Vus from \mtau summary}{Vus from tau summary}}

\begin{figure}[tb]
  \begin{center}
   \ifhevea
    \begin{tabular}{@{}cc@{}}
      \larger\bfseries\ahref{vus-tau-hflav18.png}{PNG format} &
      \larger\bfseries\ahref{vus-tau-hflav18.pdf}{PDF format} \\
      \multicolumn{2}{c}{\ahref{vus-tau-hflav18.png}{%
          \imgsrc[alt="Vus summary plot"]{vus-tau-hflav18.png}}}
    \end{tabular}
    \else
    {\fboxsep=2pt\fbox{%
        \includegraphics[width=0.75\linewidth,clip]{figures/tau/vus-tau-hflav18.pdf}}}
    \fi
    \caption{\Vus averages.
      \iffalse
      The ``Maltman 2017'' \Vus
      determination~\cite{Hudspith:2017vew} reports the experimental
      uncertainty followed by the theoretical uncertainty.
      \fi
      \label{fig:tau:vus-summary}%
    }
  \end{center}
\end{figure}

We summarize the \Vus results reporting the values, the discrepancy with
respect to the \Vus determination from CKM unitarity, and an illustration
of the measurement method:
\begin{alignat*}{6}
  &\VusUni &&= \htuse{Vus_uni.v} &&\pm \htuse{Vus_uni.e} & \quad & & \quad
  & [\text{from } \sqrt{1 - \Vud^2 - \Vub^2} \quad\text{(CKM unitarity)}]~, \\
  %
  &\VusTauIncl &&= \htuse{Vus.v} &&\pm \htuse{Vus.e} & \quad & \htuse{Vus_mism_sigma}\sigma &
  & [\text{from } \BR(\tau^- \to X_s^- \nut)]~, \\
  %
  &\VusTauKpi &&= \htuse{Vus_tauKpi.v} &&\pm \htuse{Vus_tauKpi.e} & \quad & \htuse{Vus_tauKpi_mism_sigma}\sigma &
  & [\text{from } \BR(\tauknu)/\BR(\taupinu)]~, \\
  &\VusTauKnu &&= \htuse{Vus_tauKnu.v} &&\pm \htuse{Vus_tauKnu.e} & \quad & \htuse{Vus_tauKnu_mism_sigma}\sigma &
  & [\text{from } \BR(\tauknu)]~.
\end{alignat*}

Averaging the three above \Vus determinations that rely on the \mtau branching fractions (taking into account all
correlations due to the \mtau HFLAV and other mentioned inputs) we obtain, for \Vus and its discrepancy:
\begin{alignat*}{6}
  & \Vus_\tau &&= \htuse{Vus_tau} &\quad &\htuse{Vus_tau_mism_sigma}\sigma \quad
  & [\text{average of 3 \Vus \mtau measurements}]~.
\end{alignat*}
The correlation between $f_{K\pm}$ and $f_{K\pm}/f_{\pi\pm}$ has been
assumed to be zero. Even assuming $\pm 100\%$ correlation, the \Vus uncertainty varies by less than 10\%.
\iffalse
We could not find a published estimate of the correlation of the
uncertainties on $f_{K\pm}$ and $f_{K\pm}/f_{\pi\pm}$, but even if we assume $\pm
100\%$ correlation, the uncertainty on $\Vus_\tau$ does not change by
more than $6\%$.
\fi

All \Vus determinations based on measured $\tau$ branching fractions are
lower than both the kaon and the CKM-unitarity determinations. This is
correlated with the fact that the direct measurements of the
three major $\tau$ branching fractions to kaons
[$\BR(\tau\to\htuse{Gamma10.td})$, $\BR(\tau\to\htuse{Gamma16.td})$ and
$\BR(\tau\to\htuse{Gamma35.td})$] are lower than their determinations
from the kaon branching fractions into final states with leptons within
the SM~\cite{Pich:2013lsa, Jamin:2008qg, Antonelli:2013usa}.

Alternative deterrminations of \Vus from $\BR(\tau \to
X_s\nu)$~\cite{Hudspith:2017vew,Boyle:2018dwv}, based on partially
different sets of experimental inputs, report \Vus values consistent
with the unitarity determination.

Figure~\ref{fig:tau:vus-summary} reports the HFLAV \Vus determinations
that use the \mtau branching fractions, compared to two \Vus
determinations based on kaon data~\cite{PDG_2018} and to \Vus obtained
from \Vud and the CKM matrix unitarity~\cite{PDG_2018}.


==> tau/tau_all_common.tex <==
%

%
%
%

%
%
%

\ifhevea\else
\makeatletter
\let\citeSaveTau\cite
\let\bfseriesSaveTau\bfseries
\let\LT@makecaptionSaveTau\LT@makecaption
\makeatother

%
\renewcommand{\cite}[1]{\ifmmode\text{\citeSaveTau{#1}}\else\citeSaveTau{#1}\fi}

%
\makeatletter
\DeclareRobustCommand\bfseries{%
  \not@math@alphabet\bfseries\mathbf
  \fontseries\bfdefault\selectfont\boldmath}
\DeclareRobustCommand*{\bm}[1]{%
    \mathchoice{\bmbox{\displaystyle}{#1}}%
               {\bmbox{\textstyle}{#1}}%
               {\bmbox{\scriptstyle}{#1}}%
               {\bmbox{\scriptscriptstyle}{#1}}}
\DeclareRobustCommand*{\bmbox}[2]{\mbox{\bfseries$#1 #2$}}
\makeatother

%
\makeatletter
\def\LT@makecaption#1#2#3{%
  \LT@mcol\LT@cols c{\hbox to\z@{\hss\parbox[t]\LTcapwidth{%
    \sbox\@tempboxa{\normalsize#1{#2: }#3}%
    \ifdim\wd\@tempboxa>\hsize
      \normalsize#1{#2: }#3%
    \else
      \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
    \fi
    \endgraf\vskip\baselineskip}%
  \hss}}}
\makeatother

\begin{fleqn}
\fi
%
%
%
\ifhevea
\input{tau-sections}
\input{tau-lfv-combs}
\input{tau-lfv-limits-plot}
\input{tau-lfv-combs-plot}
\else
\input{tau/tau-sections}
\input{tau/tau-lfv-combs}
\input{tau/tau-lfv-limits-plot}
\input{tau/tau-lfv-combs-plot}
\fi
%
%
%
\ifhevea\else
\end{fleqn}

\makeatletter
\let\cite\citeSaveTau
\let\bfseries\bfseriesSaveTau
\let\LT@makecaption\LT@makecaptionSaveTau
\makeatother
\fi

